Orthogonal Trace-Sum Maximization: Tightness of the Semidefinite Relaxation and Guarantee of Locally Optimal Solutions

This paper studies an optimization problem on the sum of traces of matrix quadratic forms in $m$ semi-orthogonal matrices, which can be considered as a generalization of the synchronization of rotations. While the problem is nonconvex, the paper shows that its semidefinite programming relaxation solves the original nonconvex problems exactly with high probability, under an additive noise model with small noise in the order of $O(m^{1/4})$. In addition, it shows that the solution of a nonconvex algorithm considered in Won, Zhou, and Lange [SIAM J. Matrix Anal. Appl., 2 (2021), pp. 859-882] is also its global solution with high probability under similar conditions. These results can be considered as a generalization of existing results on phase synchronization.

==> rrp-macro-file.tex <==
%&LaTeX

%%% This document contains macros that will be used throughout
%%% It is very neatly organized.
\usepackage{amsfonts,amsmath,amssymb,amsthm}
\usepackage{url}
\usepackage{natbib}
%\usepackage[natbib,authordate,backend=biber,isbn=false,doi=false,noibid]{biblatex-chicago}
\usepackage{flexisym}


\newtheorem{assumption}{Assumption}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newcommand{\qed}{\hfill\rule{2mm}{2mm}}
\newcommand{\svskip}{\vspace{1.75mm}}
\newcommand{\mvskip}{\vspace{.25in}}
\newcommand{\lvskip}{\vspace{.5in}}

%%%%% Packages

%\usepackage[notcite]{showkeys}

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage[dvips]{graphicx}

\usepackage{algorithmic}
\usepackage{algorithm}


\usepackage{color}

\usepackage{url}
%\usepackage{citesort}

\usepackage{supertabular}

%\usepackage{enumitem}


%%% Theorem setup

%\theoremstyle{plain}

\newtheorem{bigthm}{Theorem}
\renewcommand{\thebigthm}{\Alph{bigthm}}	% Number with A, B, C, etc.

\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}

%\newtheorem{algorithm}[thm]{Algorithm}

\theoremstyle{remark}

\newtheorem{fact}[thm]{Fact}
\newtheorem{claim}[thm]{Claim}

\newtheorem{rem}[thm]{Remark}
%\newtheorem{example}[thm]{Example}


%\newtheorem*{notation}{Notation}

%\numberwithin{equation}%{section}

\numberwithin{thm}{section}

%\numberwithin{figure}{chapter}
%\numberwithin{table}{chapter}


%%% Typesetting

\DeclareMathAlphabet{\mathsfsl}{OT1}{cmss}{m}{sl}


%%% Other font changes

\newcommand{\lang}{\textit}
\newcommand{\titl}{\textsl}
\newcommand{\term}{\emph}

%\newcommand{\algname}{\textsc}

\newcommand{\notate}[1]{\textcolor{red}{\textbf{[#1]}}}
\newcommand{\marginnote}[1]{\marginpar{\tiny{\notate{#1}}}}
\newcommand{\cnst}[1]{\mathrm{#1}}


%%% Old symbols with new names

\newcommand{\oldphi}{\phi}
\renewcommand{\phi}{\varphi}

\newcommand{\eps}{\varepsilon}


%%% New symbols

\newcommand{\defby}{\overset{\mathrm{\scriptscriptstyle{def}}}{=}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}

\newcommand{\sumnl}{\sum\nolimits}
\newcommand{\defeq}{\mathrel{\mathop{:}}=}

%%% Constants

\newcommand{\econst}{\mathrm{e}}
\newcommand{\iunit}{\mathrm{i}}

\newcommand{\onevct}{\mathbf{e}}
\newcommand{\zerovct}{\vct{0}}

%\newcommand{\Id}{\mathsf{I}}
%\newcommand{\onemtx}{\mathsf{1}}
%\newcommand{\zeromtx}{\mathsf{0}}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\onemtx}{\bm{1}}
\newcommand{\zeromtx}{\bm{0}}


%%% Sets

\newcommand{\coll}[1]{\mathscr{#1}}

\newcommand{\Sspace}[1]{\mathbb{S}^{#1}}

\newcommand{\Rplus}{\mathbb{R}_{+}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

\newcommand{\M}{\mathbb{M}}


%%% Real and complex analysis

\newcommand{\abs}[1]{\left\vert {#1} \right\vert}
\newcommand{\abssq}[1]{{\abs{#1}}^2}

\newcommand{\sgn}[1]{\operatorname{sgn}{#1}}
\newcommand{\real}{\operatorname{Re}}
\newcommand{\imag}{\operatorname{Im}}

\newcommand{\diff}[1]{\mathrm{d}{#1}}
\newcommand{\idiff}[1]{\, \diff{#1}}

\newcommand{\grad}{\nabla}
\newcommand{\subdiff}{\partial}

\newcommand{\argmin}{\operatorname*{arg\; min}}
\newcommand{\argmax}{\operatorname*{arg\; max}}


%%% Probability

\newcommand{\Probe}[1]{\mathbb{P}\left({#1}\right)}
\newcommand{\Prob}[1]{\mathbb{P}\left\{ {#1} \right\}}
\newcommand{\Expect}{\operatorname{\mathbb{E}}}

\newcommand{\normal}{\textsc{normal}}
\newcommand{\erf}{\operatorname{erf}}



%%% Vector and matrix operators

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\tvct}[1]{\tilde{\vct{#1}}} % Add tilde to vector
%\newcommand{\mtx}[1]{\mathsfsl{#1}}

%\newcommand{\transp}{\mathrm{T}}
\newcommand{\transp}{*}
\newcommand{\adj}{*}
\newcommand{\psinv}{\dagger}

\newcommand{\lspan}[1]{\operatorname{span}{#1}}

\newcommand{\range}{\operatorname{range}}
\newcommand{\colspan}{\operatorname{colspan}}

\newcommand{\rank}{\operatorname{rank}}

\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{tr}}

\newcommand{\supp}[1]{\operatorname{supp}(#1)}

\newcommand{\smax}{\sigma_{\max}}
\newcommand{\smin}{\sigma_{\min}}

% Projection operator
\newcommand{\Proj}{\ensuremath{\mtx{\Pi}}}

%%% Semidefinite orders

\newcommand{\psdle}{\preccurlyeq}
\newcommand{\psdge}{\succcurlyeq}

\newcommand{\psdlt}{\prec}
\newcommand{\psdgt}{\succ}

%%% Mensuration: inner products and norms

\newcommand{\ip}[2]{\left\langle {#1},\ {#2} \right\rangle}
\newcommand{\absip}[2]{\abs{\ip{#1}{#2}}}
\newcommand{\abssqip}[2]{\abssq{\ip{#1}{#2}}}
\newcommand{\tworealip}[2]{2 \, \real{\ip{#1}{#2}}}

\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\normsq}[1]{\norm{#1}^2}

% Fixed-size inner products and norms are useful sometimes

\newcommand{\smip}[2]{\bigl\langle {#1}, \ {#2} \bigr\rangle}
\newcommand{\smabsip}[2]{\bigl\vert \smip{#1}{#2} \bigr\vert}
\newcommand{\smnorm}[2]{{\bigl\Vert {#2} \bigr\Vert}_{#1}}

% Specific norms that are used frequently

\newcommand{\enorm}[1]{\norm{#1}}
\newcommand{\enormsq}[1]{\enorm{#1}^2}

\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\fnormsq}[1]{\fnorm{#1}^2}

\newcommand{\pnorm}[2]{\norm{#2}_{#1}}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}

\newcommand{\iinorm}[1]{\pnorm{\infty,\infty}{#1}}

\newcommand{\dist}{\operatorname{dist}}

\newcommand{\triplenorm}[1]{\left\vert\!\left\vert\!\left\vert {#1} \right\vert\!\right\vert\!\right\vert}

\newcommand{\opnorm}[1]{\ensuremath{\triplenorm{#1}}}

%%% Optimization

% Minimization program
\newcommand{\minprog}[3]{
  \left.
  \begin{array}{ll}
    \text{minimize}_{#1} & {#2}  \\[5pt]
    \text{subject to} & #3
  \end{array}
  \right.
}

%%% Landau notation
\newcommand{\bigOh}{\mathcal{O}}

%%% Special definitions for inliers/outliers
\newcommand{\In}{\ensuremath{\mathrm{In}}}
\newcommand{\Out}{\ensuremath{\mathrm{Out}}}
\newcommand{\Xin}{\ensuremath{\mathcal{X}_{\mathrm{In}}}}
\newcommand{\Xout}{\ensuremath{\mathcal{X}_{\mathrm{Out}}}}
\newcommand{\Xall}{\ensuremath{\mathcal{X}}}

\newcommand{\Expr}{\ensuremath{\mathcal{E}}}
\newcommand{\sExpr}{\ensuremath{\tilde{\mathcal{E}}}}
\newcommand{\Strct}{\ensuremath{\mathcal{S}}}
\newcommand{\sStrct}{\ensuremath{\tilde{\mathcal{S}}}}
%%% Special definitions for inliers/outliers

%\newcommand{\Xin}{\ensuremath{\mathcal{X}_{\mathrm{In}}}}
%\newcommand{\Xout}{\ensuremath{\mathcal{X}_{\mathrm{Out}}}}
\newcommand{\sI}{\mathcal{I}}

\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bc}{\boldsymbol{c}}
%\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bT}{\boldsymbol{T}}

\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\bSigma}{\boldsymbol\Sigma}
\newcommand{\bDelta}{\boldsymbol\Delta}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\def\bbC{\mathbb{C}}

\def\reals{\mathbb{R}}
\def\bx{\boldsymbol{x}}
\def\be{\boldsymbol{e}}
\def\bu{\boldsymbol{u}}
\def\bb{\boldsymbol{b}}
\def\bS{\boldsymbol{S}}
\def\b0{\mathbf{0}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
%\def\bC{\boldsymbol{C}}
\def\bSigma{\boldsymbol\Sigma}
\def\bGamma{\boldsymbol\Gamma}
\def\bDelta{\boldsymbol\Delta}
\def\bU{\boldsymbol{U}}
\def\bR{\boldsymbol{R}}
\def\bC{\boldsymbol{C}}
\def\bv{\boldsymbol{v}}
\def\bA{\boldsymbol{A}}
\def\bY{\boldsymbol{Y}}
\def\bB{\boldsymbol{B}}
\def\bG{\boldsymbol{G}}

\def\bg{\boldsymbol{g}}
\def\ba{\boldsymbol{a}}
\def\bw{\boldsymbol{w}}
\def\bd{\boldsymbol{d}}
\def\bt{\boldsymbol{t}}
\def\beps{\boldsymbol{\epsilon}}



\def\bH{\boldsymbol{H}}
\def\bn{\boldsymbol{n}}
\def\calD{\mathcal{D}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}

\def\bI{\mathbf{I}}
\def\TV{\mathrm{TV}}
\def\im{\mathrm{im}}
\def\tr{\mathrm{tr}}
\def\rmL{\mathrm{L}}
\def\rmV{\mathrm{V}}
\def\Nin{N_{\text{in}}}
\def\Nout{N_{\text{out}}}
\def\SPSD{\mathrm{S_+}}
\def\CTF{\mathrm{CTF}}
\def\corr{\mathrm{corr}}
\def\orth{\mathrm{orth}}
\def\PSD{\mathrm{S_{++}}}
\def\Sp{\mathrm{Sp}}
\def\HPSD{\mathbb{H}}
\def\bbH{\mathbb{H}}
\usepackage{algorithmic}
\usepackage{algorithm}
\newcommand{\di}{{\,\mathrm{d}}}


\def\E{\mathop{\rm E\,\!}\nolimits}
\def\Pr{\mathop{\rm Pr\,\!}\nolimits}
\def\Var{\mathop{\rm Var}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\den{\mathop{\rm den}\nolimits}
\def\midd{\mathop{\,|\,}\nolimits}
\def\sgn{\mathop{\rm sgn}\nolimits}
\def\vec{\mathop{\rm vec}\nolimits}
\def\sinc{\mathop{\rm sinc}\nolimits}
\def\curl{\mathop{\rm curl}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\tr{\mathop{\rm tr}\nolimits}
\def\len{\mathop{\rm len}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\dist{\mathop{\rm dist}\nolimits}
\def\prox{\mathop{\rm prox}\nolimits}
\def\argmin{\mathop{\rm argmin}\nolimits}
\def\amp{\mathop{\;\:}\nolimits}
\def\dom{\mathop{\rm dom}\nolimits}

\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bzero}{\mathbf{0}}



==> sections/00-abstract.tex <==
This paper studies an optimization problem on the sum of traces of matrix quadratic forms in $m$  {semi-}orthogonal matrices, which can be considered as a generalization of the synchronization of rotations. While the problem is nonconvex, the paper shows that its semidefinite programming relaxation solves the original nonconvex problems exactly  {with high probability}, under an additive noise model with small noise in the order of $O(m^{1/4})$. In addition, it shows that a local solution of the nonconvex problem is also its global solution  {with high probability under similar conditions}. These results can be considered as a generalization of existing results on phase synchronization.


==> sections/01-intro.tex <==
\section{Introduction}
This paper considers the orthogonal trace-sum maximization (OTSM) problem \citep{won2018orthogonal} of estimating $m$ orthogonal matrices $\bO_1, \cdots, \bO_m$ with $\bO_i\in\reals^{d_i\times r}$ from the optimization problem:
\begin{equation}\tag{OTSM}\label{eqn:tracemax}
	\text{maximize} ~~ \sum_{1\leq i, j\leq m} \tr(\bO_i^T \bS_{ij} \bO_j) ~~
	\text{subject~to} ~~ \bO_i \in \mathcal{O}_{d_i,r},~ i=1,\dotsc,m
	,
\end{equation}
where $\bS_{ij}=\bS_{ji}^T \in \mathbb{R}^{d_i\times d_j}$ for $i,j = 1,\dotsc,m$, and $r\le\min_{i=1,\dotsc,m} d_i$, 
and
$\mathcal{O}_{d,r} = \{O \in \mathbb{R}^{d\times r}: \bO^T\bO=\bI_r\}$ is the Stiefel manifold of semi-orthogonal matrices; $\bI_r$ denotes the identity matrix of order $r$. 
%
%This paper considers the problem of estimating $m$ orthogonal matrices $\bO_1, \cdots, \bO_m$ with $\bO_i\in\reals^{d_i\times r}$ from the optimization problem:
%\begin{equation}\label{eqn:tracemax}
%    \{\hat{\bO}_i\}_{i=1}^m=\max_{\bO_i\in\reals^{d_i\times r}, i=1,\cdots,m} \sum_{i,j=1, i\neq j}^m\tr(\bO_i^T\bS_{ij}\bO_j),\,\,\,\text{subject to $\bO_i^T\bO_i=\bI$ for all $1\leq i\leq m$}.
%\end{equation}
%

The OTSM problem
has applications in generalized canonical correlation analysis \citep{hanafi2006analysis} and Procrustes analysis \citep{gower1975generalized,TenBerge1977orthogonal}. Furthermore, if $d_1=\cdots=d_m=r$, then \eqref{eqn:tracemax} reduces to the problem of synchronization of rotations  \cite{Bandeira20164}, which have wide applications such as multi-reference alignment \cite{Bandeira2017},  {cryogenic electron microscopy (cryo-EM)} \cite{doi:10.1137/090767777,ZHANG2017159}, 2D/3D point set registration~\cite{7430328,Cucuringu2012, doi:10.1137/130935458}, and multiview structure from motion \cite{6374980,7785130,7789623}.
\subsection{Related Works}
While the OTSM problem is proposed recently in \citep{won2018orthogonal}, it is closely related to many well-studied problems. In particular, its special cases have been studied in the name of angular synchronization, $\mathbb{Z}_2$ synchronization, and synchronization of rotations, and the OTSM problem itself can also be considered as a special case of the group synchronization problem. We first review these related problems and their recent developments.

%
\textbf{Angular synchronization} The complex-valued OTSM problem with $d_1=\cdots=d_m=1$ is equivalent to a problem called angular synchronization or phase synchronization, which estimates angles $\theta_1, \cdots, \theta_m \in[0,2\pi)$ from the observation of relative offsets $(\theta_i-\theta_j)$ mod $2\pi$. The problem has applications in %cryogenic electron microscopy
 {cryo-EM}
\cite{Singer2009AngularSB}, comparative biology~\cite{Gao2019}, and many others. To address this problem, Singer~\cite{Singer2009AngularSB} formulates the problem as an optimization problem as follows: let $x_k=e^{i\theta_k}$ for all $1\leq k\leq m$, it attempts to solve the nonconvex problem \begin{equation}\label{eq:angular}
\max_{\bx\in\mathbb{C}^m}\bx^*\bC\bx,\,\,\text{s.t. $|x_1|=\cdots=|x_m|=1$}.
\end{equation}
In fact, \eqref{eq:angular} can be considered as the special case of \eqref{eqn:tracemax} when $d_1=\cdots=d_m=r=2$. 

 

The angular synchronization problem \eqref{eq:angular} has been studied extensively. For example, Singer \cite{Singer2009AngularSB} proposes two methods, by eigenvectors and semidefinite programming respectively. The performance of the method is analyzed using random matrix theory and information
theory. In \cite{Bandeira2017}, Bandeira et al. assume the model $\bC=\bz\bz^*+\sigma\bW$, where $\bz\in\mathbb{C}^m$ satisfies $|z_1|=\cdots=|z_m|=1$ and $\bW\in\mathbb{C}^{m\times m}$ is a Hermitian Gaussian Wigner matrix, and show that if $\sigma\leq \frac{1}{18}m^{\frac{1}{4}}$, then the solution of semidefinite programming approach is also the solution to \eqref{eq:angular}  {with high probability}. 
 {Using a more involved argument and a modified power method, Zhong and Boumal \cite{ZhongBoumal18PhaseSynchNearOptimalBounds} improve the bound in \cite{Bandeira2017} to $\sigma=O(\sqrt{\frac{m}{\log m}})$}.

There is another line of works that solve \eqref{eq:angular} using power methods. In particular, Boumal \cite{Boumal16NonconvexPhaseSynch} investigates a modified power method and shows that the method converges to solution of \eqref{eq:angular} when $\sigma=O(m^{\frac{1}{6}})$, Liu et al.  \cite{LiuYueSo27PowerPhaseSynch} investigate another generalized power method and prove the convergence for $\sigma=O(m^{\frac{1}{4}})$, and Zhong and Boumal \cite{ZhongBoumal18PhaseSynchNearOptimalBounds} improve the rate to $\sigma=O(\sqrt{\frac{m}{\log m}})$. 


There are some other interesting works for the angular synchronization problem that are not based on semidefinite programming or power method. \cite{doi:10.1137/18M1217644} assumes that the pairwise difference are only observed over a graph, studies the landscape of a proposed objective function, and shows that the global minimizer is unique when the associated graph is incomplete and follows the Erd\"{o}s-R\'{e}nyi random graphs. \cite{doi:10.1002/cpa.21750} proposes an approximate message passing (AMP) algorithm, and analyzes its behavior by identifying phases where the problem is easy, computationally hard, and statistically impossible. 


\textbf{$\mathbb{Z}_2$ synchronization}  The real-valued OTSM problem with $d_1=\cdots=d_m=1$ is called $\mathbb{Z}_2$-synchronization problem~\cite{10.1093/comnet/cnu050} for   $\mathbb{Z}_2=\{1,-1\}$. For this problem, \cite{Fei2019AchievingTB} shows that the solution of the semidefinite programming method matches the minimax lower bound on the optimal Bayes error rate for original problem \eqref{eq:angular}.  


\textbf{Synchronization of rotations} The OTSM problem with $d_1=\cdots=d_m=r>2$ is called ``synchronization of rotations'' in some literature. This special case has wide applications in  graph realization and point cloud registration, multiview Structure from Motion (SfM)  \cite{6374980,7785130,7789623},  common lines in Cryo-EM \cite{doi:10.1137/090767777},  orthogonal least squares~\cite{ZHANG2017159}, and 2D/3D point set registration~\cite{7430328}. \cite{10.1093/imaiai/iat006} studies the problem from the perspective of manifold optimization and derive the Cram\'{e}r-Rao bounds, which is the lower bounds of the variance of any unbiased estimator. %\cite{DBLP:journals/corr/BoumalC13} shows that a lower bound concentrates on its expectation. 
\cite{THUNBERG2017243} proposes a distributed algorithm with theoretical guarantees on convergence. 
 %\cite{pmlr-v97-gao19f} generalized  \eqref{eqn:tracemax} by assuming multi-frequency information, and develop a two-stage algorithm that leverages the additional information.  
 \cite{10.1093/imaiai/iat005} discusses a method to make the estimator in \eqref{eqn:tracemax}  more robust to outlying observations. Another robust algorithm based on maximum likelihood estimator is proposed in \cite{6760038}. As for the theoretical properties, \cite{Bandeira20164} analyzes a semidefinite program approach that solves the problem approximately, and studies its approximation ratio. \cite{liu2020unified} investigates a generalized power method for this problem. A recent manuscript \cite{ling2021improved} follows the line of \cite{Bandeira2017,Boumal16NonconvexPhaseSynch,LiuYueSo27PowerPhaseSynch,ZhongBoumal18PhaseSynchNearOptimalBounds} and proves that the original problem and the relaxed problem   have the same solution when $\sigma\leq O(\frac{\sqrt{m}}{d+\sqrt{d}\log m})$. %However, we are not aware of works in the spirit of  \cite{Bandeira2017,doi:10.1137/16M105808X,doi:10.1137/16M110109X,doi:10.1137/17M1122025} that studies the effectiveness of algorithm in an additive noise model.
%We remark that the problem \eqref{eq:tracesum_relaxed} also has applications in the multi-reference alignment model in \cite{Bandeira2017} and can be solved using the synchronization approach as discussed in~\cite[Section 1.2]{Bandeira2017}, but the underlying model would not be the additive noise model. 

\textbf{Group synchronization} The OTSM problem can also be considered as a special case of the group synchronization problem, which recovers a vector of
 elements in a group, given noisy pairwise measurements of the relative elements $g_ug_v^{-1}$. The OTSM problem is the special case when the group is $\mathcal{O}_{d,r}$, the set of orthogonal matrices. \cite{abbe2017group} studies the properties of weak recovery when the elements are from a generic compact group and the underlying graph of pairwise observations is the $d$-dimensional grid.   \cite{doi:10.1002/cpa.21750} proposes an approximate message passing (AMP) algorithm for solving synchronization problems over a class of compact groups. \cite{doi:10.1137/16M1106055} generates the estimation from compact groups to the class of Cartan motion groups, which includes the important special case of rigid motions by applying the compactification process. %\cite{doi:10.1002/cpa.21760} discusses the performance of a projected power method to the problem where the elements are scalars and the observations are the modulo differences $x_i - x_j$ mod $m$, and establishes its theoretical properties.
 \cite{6875186}  assumes that measurement graph is sparse and there are corrupted observations, and show that minimax recovery rate depends almost exclusively on the edge sparsity of the measurement graph irrespective of other graphical metrics. 
 

\subsection{Our Contribution}
The main contribution of this work is the study of the OTSM problem under an additive model of Gaussian noise. The main results are two-folds: First, we propose a semidefinite programming approach for solving \eqref{eqn:tracemax} and show that it solves \eqref{eqn:tracemax} exactly when the size of noise is bounded. Second, we show that any local minimizer of \eqref{eqn:tracemax} is the global minimizer, when the noise size is bounded and a technical assumption is satisfied. %The 
 {These} results can be considered as a generalization of \cite{Bandeira2017} from angular synchronization to the OTSM problem. %Since the OTSM problem is a generalization of the synchronization-of-rotations problem, our result has have a wide range of applications. 


\section{The OTSM problem}
\subsection{Model Assumption}
In this work, we assume the MAXBET model of generating $\bS_{ij}$, which %assumes that there exists $\{\bTheta_i\}_{1\leq i\leq m}, \{\bW_{ij}\}_{1\leq i\neq j\leq m}$ 
 {postulates the existence of $\{\bTheta_i\}_{1\leq i\leq m}$ and $\{\bW_{ij}\}_{1\leq i\neq j\leq m}$} 
such that %$\bTheta_i\in\reals^{d_i\times r}$, $\bTheta_i^T\bTheta_i=\bI$ for all $1\leq i\leq m$,
$\bTheta_i\in\mathcal{O}_{d_i,r}$ for all $1\leq i\leq m$, and
\begin{equation}
	\text{$\bS_{ij}=\bTheta_i\bTheta_j^T+\bW_{ij}$, where $\bW_{ij}=\bW_{ji}^T$ for all $1\leq i,j\leq m$.}\label{eq:model}\tag{MAXBET}
\end{equation} 
In this model, $\bTheta_i\bTheta_j^T$ is considered as the ``clean measurement of relative elements'' and $\bW_{ij}$ is considered as an additive noise. This is a natural model for the generalized canonical correlation analysis in \citep{won2018orthogonal}, and it is also the standard problem for synchronization problems, such as synchronization of rotations \cite{10.1093/imaiai/iat005,10.1093/imaiai/iat006} and group synchronization \cite{abbe2017group,doi:10.1002/cpa.21750}.
%
%We remark that in some applications, 


In some applications \cite{TenBerge1977orthogonal,hanafi2006analysis}, it is also natural to assume the MAXDIFF model that differs from the MAXBET model only in the diagonal terms:%that
\begin{equation}\label{eq:model2}\tag{MAXDIFF}
\bS_{ii}=\bzero
\quad\text{and}\quad
\bS_{ij}=\bTheta_i\bTheta_j^T+\bW_{ij},
~i \neq j
.
\end{equation}
In this work, we will present our main results based on the MAXBET model, and discuss the MAXDIFF model in the remarks.

%\subsection{Noiseless case}
When there is no noise in either MAXBET or MAXDIFF model, setting $\bO_i=\bTheta_i$, $i=1, \dotsc, m$, solves problem \eqref{eqn:tracemax}. This observation is summarized as Proposition~\ref{prop:noiseless} and the proof is deferred to Section~\ref{sec:proof_prop:noiseless}.  
\begin{proposition}\label{prop:noiseless} In the noiseless case ($\bW_{ij}=\bzero$ for all $i, j=1,\dotsc,m$), $(\bO_1, \dotsc, \bO_m) = (\bTheta_1, \dotsc, \bTheta_m)$ globally solves \eqref{eqn:tracemax}
under the model \eqref{eq:model} or \eqref{eq:model2}.
\end{proposition}

However, in the presence of noise, Proposition~\ref{prop:noiseless} does not hold and problem \eqref{eqn:tracemax} is difficult to solve. To establish theoretical guarantees for the noisy setting, we investigate two approaches, one is based on semidefinite programming and the other one is based on finding local optimal solutions of \eqref{eqn:tracemax}.

\subsection{Approach 1: Semidefinite programming relaxation}

While the problem \eqref{eqn:tracemax} is nonconvex and difficult to solve,
we can relax it to a convex optimization problem based on semidefinite programming that can be solved efficiently. In fact, semidefinite programming-based approaches have been proposed and analyzed for the problem of angular synchronization \cite{Singer2009AngularSB,Bandeira2017,ZhongBoumal18PhaseSynchNearOptimalBounds} and synchronization of rotations \cite{Bandeira20164}, and our proposed method can be considered as a generalization of these existing methods.

The argument of the relaxation is as follows. Let $D=\sum_{i=1}^md_i$, 
\begin{equation}\label{eqn:blockS}
\bS=\begin{bmatrix}
    \bS_{11} & \bS_{12} & \dots  & \bS_{1m} \\
    \bS_{21} & \bS_{22} &  & \bS_{2m} \\
    \vdots &  & \ddots& \vdots \\
   \bS_{m1} & \bS_{m2} &\cdots  &\bS_{mm}
\end{bmatrix}\in\reals^{D\times D},  \,\,\,\text{and} \,\,\,{\bO}=\left[ \begin{array}{c}
{\bO}_1\\
\vdots\\
{\bO}_m\\
 \end{array} \right]\in\reals^{D\times r},
\end{equation}
then by setting $\bU=\bO\bO^T$, 
the problem
\eqref{eqn:tracemax} 
 {%
is equivalent to finding
\begin{equation}\label{eq:tracesum_problem1}
\tilde{\bU}= {\arg}\max_{\bU\in\reals^{D\times D}, \bU=\bU^T}\tr(\bS\bU),~\text{subject to $\bU\psdge \mathbf{0},~\bU_{ii}\psdle\bI,~\tr(\bU_{ii})=r,~ \rank(\bU)=r$,}
\end{equation}
which%
}
can be relaxed to solving
\begin{equation}\label{eq:tracesum_relaxed}
%\hat{\bU}=
\max_{\bU\in\reals^{D\times D}, \bU=\bU^T}\langle\bS, \bU\rangle ~~ \text{subject to $\bU\psdge \mathbf{0}, \bU_{ii}\psdle\bI, \tr(\bU_{ii})=r$,}
\end{equation}
where $\bM \psdge \bzero$ (resp. $\bM \psdle \bzero$) means that a matrix $\bM$ is positive (resp. negative) semidefinite.
% If a solution $\hat{\bU}$ to problem \eqref{eq:tracesum_relaxed} has rank $r$, then it can be decomposed to $\hat{\bU}=\hat{\bO}\hat{\bO}^T$ where $\hat{\bO}\in\mathbb{R}^{D\times r}$. Write $\hat{\bO}=[\hat{\bO}_1^T, \dotsc, \hat{\bO}_m^T]^T$, then $\hat{\bO}_i\in\mathcal{O}_{d_i,r}$ for all $1\leq i\leq m$ and $(\hat{\bO}_1, \dotsc, \hat{\bO}_m)$ \emph{globally} solves problem \eqref{eqn:tracemax}.
 {%
If a solution $\hat{\bU}$ to problem \eqref{eq:tracesum_relaxed} has rank $r$, then we can set $\tilde{\bU}=\hat{\bU}$, which can be decomposed to $\hat{\bU}=\tilde{\bV}\tilde{\bV}^T$ where $\tilde{\bV}\in\mathbb{R}^{D\times r}$. Write $\tilde{\bV}=[\tilde{\bV}_1^T, \dotsc, \tilde{\bV}_m^T]^T$, then $\tilde{\bV}_i\in\mathcal{O}_{d_i,r}$ for all $1\leq i\leq m$ and $(\tilde{\bV}_1, \dotsc, \tilde{\bV}_m)$ \emph{globally} solves problem \eqref{eqn:tracemax}.%
}


This work shows that if the noises $\bW_{ij}$ are ``small'', then the solutions of problems \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed} are equivalent in the sense that
%$\hat{\bU}=\hat{\bO}\hat{\bO}^T$ with $\hat{\bO}$ rank-$r$, 
 {$\hat{\bU}=\tilde{\bV}\tilde{\bV}^T$ with $\tilde{\bV}$ rank-$r$,} 
hence the convex relaxation is tight.



\subsection{Approach 2: finding local optimal solutions of \eqref{eqn:tracemax}}
While the semidefinite progamming approach is convex and can be solved efficiently, it has a large computational cost when $m$ is large, and solving the original nonconvex problem \eqref{eqn:tracemax} 
 {without lifting the variable (from $\bO$ to $\bU$)}
is more efficient. A natural question is, is there any guarantee on the goodness of local minimizers of \eqref{eqn:tracemax} and when is a critical point of problem \eqref{eqn:tracemax} globally optimal? 

Using the optimality conditions for the convex relaxation \eqref{eq:tracesum_relaxed}, Won et al. \citep{won2018orthogonal} study  conditions for a first-order critical point of problem \eqref{eqn:tracemax} to be globally optimal. 
Specifically, 
the first-order necessary condition for local optimality of \eqref{eqn:tracemax} is
\begin{equation}\label{eqn:firstorder}
	\bO_i\bLambda_i = \sum_{j\neq i}\bS_{ij}\bO_j, \quad i=1,\dotsc,m,
\end{equation}
for some symmetric matrix $\bLambda_i$. The latter matrix is the Lagrange multiplier associated with the constraint $\bO_i \in \mathcal{O}_{d_i,r}$, and has a representation $\bLambda_i = \sum_{j\neq i}\bO_i^T\bS_{ij}\bO_j$.
If $\tau_i$ is the smallest eigenvalue of $\bLambda_i$,
then a first-order critical point $(\bO_1,\dotsc,\bO_m)$ is a global optimum of \eqref{eqn:tracemax} if
\begin{equation}\label{eqn:certificate}
	\bL =
	\begin{bmatrix} 
	\bO_1\bLambda_1\bO_1^T+\tau_1(\bI_{d_1}-\bO_1\bO_1^T)
		 &     \\
	     &   \ddots & \\
	     &          &
		\bO_m\bLambda_m\bO_m^T+\tau_m(\bI_{d_m}-\bO_m\bO_m^T)
	\end{bmatrix}
	- \bS
	\psdge \bzero
	.
\end{equation}
%where $\bM \psdge \bzero$ means that a matrix $\bM$ is positive semidefinite. 

Condition \eqref{eqn:certificate} requires finding a first-order critical point. A block relaxation-type algorithm that converges to a first-order point is considered in \citep{won2018orthogonal}.
\textit{A priori} conditions on the data matrix $\bS$ under which $\bL \psdge \bzero$ has remained an open question. %

This work shows that if the noises $\bW_{ij}$ are ``small'', then  all ``not too bad'' %local maxima (second-order critical points) 
%\textcolor{red}{\sout{second-order}} 
critical points (for precise definition, see \Cref{sec:mainresults:local})
of \eqref{eqn:tracemax} satisfy condition \eqref{eqn:certificate}, hence are globally optimal.
The meanings of ``small'' and ``not too bad'' will be made clear in the sequel.



%the pairwise noisy observations $\bTheta_i\bTheta_j^T$, $1\leq i\neq j\leq m$. $\{\bS_{ij}\}_{i\neq j, i,j=1}^m$, where $\bS_{ij}\approx \bTheta_i\bTheta_j^T$.
%In this paper, we consider the orthogonal trace-sum maximization problem proposed in~\citep{won2018orthogonal} . %Given $\bS_{ij}=\bS_{ji}^T\in\reals^{d_i\times d_j}$ for $1\leq i,j\leq m$ and $r<\min_{1, \cdots, m}d_i$, 
%To estimates $\bTheta_i$, we are interested in the following optimization problem:
%\begin{equation}\label{eqn:tracemax}
%    \{\hat{\bO}_i\}_{i=1}^m=\max_{\bO_i\in\reals^{d_i\times r}, i=1,\cdots,m} \sum_{i,j=1, i\neq j}^m\tr(\bO_i^T\bS_{ij}\bO_j),\,\,\,\text{subject to $\bO_i^T\bO_i=\bI$ for all $1\leq i\leq m$}.
%\end{equation}
%This problem was introduced and discussed in \citep{won2018orthogonal}  as the orthogonal trace-sum maximization problem, and it has many applications such as canonical correlation analysis, the little Grothendieck problem over the orthogonal group, and orthogonal least squares. (add cirations). In addition, when $d_1=\cdots=d_m=r$, then it is the synchronization of rotations problem (citations...), which can be considered as a generalization of the angular synchronization(cite...).


\subsection{Notation}

This work sometimes divides a matrix $\bX$ of size $D\times D$ into $m^2$ submatrices, such that the %$ij-$th 
 {$(i,j)$}
block is a $d_i\times d_j$ submatrix. We use $\bX_{ij}$ or $[\bX]_{ij}$ to denote this submatrix. Similarly, sometimes we divide a matrix of $\bY\in\reals^{D\times r}$ or a vector $\by\in\reals^D$ into $m$ submatrices or $m$ vector, where the $i$-th component, denoted by $\bY_i$, $[\bY]_i$ or $\by_i$, $[\by]_i$, is a matrix of size $d_i\times r$ or a vector of length $d_i$.

For any matrix $\bX$, we use $\|\bX\|$ to represent its operator norm and $\|\bX\|_F$ to represent its Frobenius norm. In addition, $\bP_{\bX}$ represents an orthonormal matrix whose column space is the same as $\bX$, $\bP_{\bX^\perp}$ is an orthonormal matrix whose column space is the orthogonal complement of the column space of $\bX$, $\Proj_{\bX}=\bP_{\bX}\bP_{\bX}^T$ is the projector to the column space of $\bX$, and $\Proj_{\bX^\perp}$ is the projection matrix to the orthogonal complement of the column space of $\bX$. If $\bY\in\reals^{n\times n}$ is symmetric, we use $\lambda_1(\bY)\geq \lambda_2(\bY)\geq \cdots\geq \lambda_n(\bY)$ to denote its eigenvalues in descending order.



==> sections/02-mainresult1.tex <==
\section{Main results}\label{sec:mainresults}
In this section, we present our main results. The first main result, Theorem~\ref{thm:main}, shows that if the noises $\bW_{ij}$ are ``small'', then the convex relaxation in \eqref{eq:tracesum_relaxed} provides a tractable algorithm for solving the original problem \eqref{eqn:tracemax} exactly.  The second main result, Theorem~\ref{thm:main2}, shows that if the noises $\bW_{ij}$ are ``small'', then  %all %``not too bad'' local maxima (second-order critical points) 
%\textcolor{red}{\sout{second-order}} 
the critical points obtained by the algorithm in \citep{won2018orthogonal}
of \eqref{eqn:tracemax} is globally optimal
if an additional technical assumption is satisfied.

\subsection{Theoretical guarantees on the SDP approach}
This section provides conditions that if the noises $\bW_{ij}$ are ``small'', then the solution of problem \eqref{eq:tracesum_relaxed} has rank $r$ and is equivalent to the solution of the problem \eqref{eqn:tracemax}, in the sense that
%$\hat{\bU}=\hat{\bO}\hat{\bO}^T$ with $\hat{\bO}$ rank-$r$, 
 {$\hat{\bU}=\tilde{\bV}\tilde{\bV}^T$ with $\tilde{\bV}$ rank-$r$,}
hence the convex relaxation is tight.
% main technical result and show how it can be used to prove Theorem~\ref{thm:main0}. 
 
 We begin with two deterministic conditions on $\bW$ in Theorem~\ref{thm:main} and Corollary~\ref{cor:probablistic}, show that the condition holds with high probability under a Gaussian model in Corollary~\ref{cor:probablistic_gaussian}, and a statement on the consistency of the solution in \Cref{cor:consistency1}. The statement of the first deterministic theorem is as follows:
\begin{theorem}\label{thm:main}
%Assume that there exists $\bW\in\reals^{D\times D}$ such that $\bW_{ii}=\mathbf{0}$, $\bW_{ij}=\bW_{ij}^T$, and $\bS_{ij}=\bTheta_i\bTheta_j^T+\bW_{ij}$ for all $1\leq i\neq j\leq m$, where $\bTheta_i\in\reals^{d_i\times r}$ and $\bTheta_i^T\bTheta_i=\bI_r$ for all $1\leq i\leq m$, then 
If $m\geq 2\|\bW\|(2\sqrt{r}+1)+2$, and $\bW\in\reals^{D\times D}$ is small in the sense that
\begin{eqnarray}\label{eq:condition_deterministic}
m &>& 4m\frac{2\left(\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+4\|\bW\|^2\sqrt{\frac{r}{m}}\right)}{m-2\|\bW\|(2\sqrt{r}+1)-2} \nonumber \\
& & \quad +2\left(\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+4\|\bW\|^2\sqrt{\frac{r}{m}}\right)+8\|\bW\|\sqrt{\frac{r}{m}}+2\|\bW\|,\end{eqnarray}
then the solutions of \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed} are equivalent in the sense that $\hat{\bU}_{ij}=\hat{\bO}_i\hat{\bO}_j^T$ for all $1\leq i,j\leq m$.
\end{theorem}
The proof of Theorem~\ref{thm:main} will be presented in Section~\ref{sec:proof_thm:main}. While the condition \eqref{eq:condition_deterministic} is rather complicated,  we expect that it holds for large $m$ when $\|\bW\|$ and $\max_{i=1,\dotsc,m}\|(\bW\bTheta)_i\|_F$  grow slowly as $m$ increases.  To prove this idea rigorously, we introduce the notion of $\bTheta$-discordant noise, which is inspired by the notion of ``$z$-discordant matrix'' in \cite[Definition 3.1]{Bandeira2017}. 
\begin{definition}[$\bTheta$-discordance]\label{def:discordance}
	Let $\bTheta=(\bTheta_1,\dotsc,\bTheta_m)\in\times_{i=1}^m\mathcal{O}_{d_i,r}$. Recall $D=\sum_{i=1}d_i$. A matrix $\bW$ is said to be $\bTheta$-discordant if it is symmetric and satisfies 
	$$
		\|\bW\| \le 3\sqrt{D}
	$$
	and
	$$
		\max_{i=1,\dotsc,m}\|[\bW\bTheta]_i\|_F 
		\le 3\sqrt{Dr\log m}
		.
	$$
\end{definition}
Based on the definition of $\bTheta$-discordant noise, The next Corollary is a deterministic, non-asymptotic statement that simplifies the condition \eqref{eq:condition_deterministic} in Theorem~\ref{thm:main}. Its proof is deferred to Section~\ref{sec:proof_cor:probablistic}.
%our result in summarized as follows in Corollary~\ref{cor:probablistic}, and its proof is deferred to Section~\ref{sec:proof_cor:probablistic}.
\begin{corollary}\label{cor:probablistic}
Let $d=D/m$. Suppose that $m\geq 8$ and $\sigma^{-1}\bW$ is $\bTheta$-discordant for some 	\begin{equation}\label{eq:cor:discordant}
	\sigma \le \frac{m^{1/4}}{60\sqrt{dr}},
	\end{equation}
then the condition \eqref{eq:condition_deterministic} holds, and the solutions of \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed} are equivalent.
% Under the additive Gaussian noise model in \eqref{eq:noise_model}, assume $d=\sum_{i=1}^md_i/m$, $d$ and $r$ are fixed, and $\sigma<\frac{1}{17r^{\frac{1}{4}}d^{\frac{1}{2}}} m^{1/4}$, then  as $m\rightarrow\infty$, with probability approaching $1$, the condition \eqref{eq:condition_deterministic} holds, and the solutions of \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed} are equivalent.
\end{corollary}
Next, we apply a natural probabilistic model and investigate the $\bTheta$-discordant property. In particular, we follow \cite{Boumal16NonconvexPhaseSynch,Bandeira2017,ZhongBoumal18PhaseSynchNearOptimalBounds} and use an additive Gaussian noise model:
\begin{equation}\label{eq:noise_model}
\text{$\bW\in\mathbb{R}^{D\times D}$ is elementwisely i.i.d. sampled from $N(0,\sigma^2)$.}
\end{equation}
For this model, we have the following Corollary that shows if %$\sigma<O(\frac{m^{1/4}}{60\sqrt{dr}})$, 
 {$\sigma \le O(\frac{m^{1/4}}{\sqrt{dr}})$,}
then \eqref{eq:condition_deterministic} holds with high probability. Its proof is deferred to Section~\ref{sec:proof_cor:probablistic_gaussian}.
\begin{corollary}\label{cor:probablistic_gaussian}
	Assume the additive Gaussian noise model in \eqref{eq:noise_model}, $m\ge 3$ or $m \ge 2$ and $\min_{i=1}^md_i \ge 6$, then with probability at least $1-1/m-2\exp\left(-\frac{(3-2\sqrt{2})^2}{4}D\right)$, $\bW$ satisfies the $\bTheta$-discordant property. 
	
	As a result, if $\sigma \le \frac{m^{1/4}}{60\sqrt{dr}}$ and $m\ge 8$, then with the same probability, the condition \eqref{eq:condition_deterministic} holds, and the solutions of \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed} are equivalent.
\end{corollary}


%\section{Main Result 2}
%This section presents our main result that the local minimizer of the problem \eqref{eqn:tracemax} is also its global minimizer.
%
%
%\subsection{Certificate of global optimality (is this section needed?)}
%
%We define any point in  $\mathcal{O}_{d_1,r}\times\dotsb\times\mathcal{O}_{d_m,r}$ satisfying \eqref{eqn:firstorder2} as a first-order critical point. The set of first-order critical points is denoted by $\Gamma$. The following result was obtained previously.
%\begin{theorem}[\citet{won2018orthogonal}]\label{thm:certificate}
%	Suppose $(\bar{\bO}_1,\dotsc,\bar{\bO}_m)\in\Gamma$ is a local solution to \eqref{eqn:tracemax}.
%	Let $\bar{\bLambda}_i=\sum_{j\neq i}\bar{\bO}_i^T\bS_{ij}\bar{\bO}_j$ and $\tau_i$ be the smallest eigenvalue of $\bar{\bLambda}_i$ for $i=1,\dotsc,m$.
%	Then $(\bar{\bO}_1,\dotsc,\bar{\bO}_m)$ is a global optimum of \eqref{eqn:tracemax} if
%\begin{equation}\label{eqn:certificate}
%	\bL^\star =
%	\begin{bmatrix} 
%	\bar{\bO}_1\bar{\bLambda}_1\bar{\bO}_1^T+\tau_1(\bI_{d_1}-\bar{\bO}_1\bar{\bO}_1^T)
%		 &     \\
%	     &   \ddots & \\
%	     &          &
%		\bar{\bO}_m\bar{\bLambda}_m\bar{\bO}_m^T+\tau_m(\bI_{d_m}-\bar{\bO}_m\bar{\bO}_m^T)
%	\end{bmatrix}
%	- \bS
%	\succeq \bzero
%	,
%\end{equation}
%where $\bS$ is as defined in \eqref{eqn:blockS}.
%\end{theorem}
%\begin{remark}\label{rem:smallercertificate}
%Let $\bar{\bO} = {m}^{-1/2}[\bar{\bO}_1^T, \cdots, \bar{\bO}_m^T]^T$. It can be easily seen that $\bar{\bO}\in\mathcal{O}_{D,r}$ and $\bL^\star\bar{\bO}=\bzero$
%using the first-order optimality condition \eqref{eqn:firstorder}.
%Therefore it suffices to test $(\bar{\bO}^\perp)^T\bL^\star\bar{\bO}^\perp \succeq \bzero$, 
%where $\bar{\bO}^\perp\in \mathcal{O}_{D,D-r}$ fills out $\bar{\bO}$ to a full orthogonal matrix.
%%This matrix is $(D-r)\times(D-r)$ and may be easier to handle than the $D\times D$ matrix $\bL^\star$.
%\end{remark}
\begin{remark}
The assumption $m\geq 8$ in Corollary~\ref{cor:probablistic} can be relaxed, but with a different constant factor in the upper bound of $\sigma$ in \eqref{eq:cor:discordant}. For example, if $m\geq 3$ is assumed, then we need 	$\sigma \le \frac{m^{1/4}}{124\sqrt{dr}}$; see Section~\ref{sec:proof_cor:probablistic}. 
\end{remark}
\begin{remark}
The result in this section can be naturally adapted to the %MAXBET 
MAXDIFF
model. The main intermediate results for the proof of Theorem~\ref{thm:main} 
 {given in \Cref{sec:proof_thm:main}},
including Lemma~\ref{lemma:noisy} and  Lemma~\ref{lemma:noisy2}, still hold with $\bW_{ii}=0$. While the estimations in Lemma~\ref{lemma:pertubation} do not hold, following the steps %in Section~\ref{sec:MAXBET}, 
 {given at the end of \Cref{sec:MAXBET}},
we are still able to obtain similar bounds on the difference between $\tilde{\bV}$ and %$\tilde{\bTheta}$.
 {$\bTheta$.}
In summary, we are able to obtain parallel results to Theorem~\ref{thm:main} and Corollary~\ref{cor:probablistic} for the %MAXBET 
MAXDIFF
setting. In particular, if $\bW$ is generated using the model in Corollary~\ref{cor:probablistic}, then the solutions of \eqref{eqn:tracemax} and the %MAXBET 
MAXDIFF
problem are equivalent with probability at least  $1-1/m-2\exp\left(-\frac{(3-2\sqrt{2})^2}{4}D\right)$, if $\sigma\leq \frac{m^{1/4}}{120\sqrt{dr}}$ and $m\geq 10$. 
 {%
    This, more restrictive, bound under the MAXDIFF model is expected since MAXDIFF utilizes \emph{less} information on the clean signal $\bTheta$ for the same number of measurements.%
}
\end{remark}

%As a corollary of  theoretical question is whether the solution to \eqref{eqn:tracemax} recovers the true signal $\bTheta$ if $m$ is sufficiently large. The following result is a byproduct of 
Following the proof of \Cref{thm:main}, we have 
 {a consistency result, i.e.,}
that the solution of \eqref{eq:tracesum_relaxed} recovers the true signal $\bTheta$ if $m$ is sufficiently large:
\begin{corollary}\label{cor:consistency1}
Assuming the conditions in Corollary~\ref{cor:probablistic}, then the solution of \eqref{eq:tracesum_relaxed}, $\tilde{\bU}$, admits a decomposition $\tilde{\bU}=\tilde{\bV}\tilde{\bV}^T$ with $\tilde{\bV}\in\reals^{D\times r}$, such that% $\tilde{\bV}$ is close to $\bV$ in the sense that 
\begin{align}\label{eq:consistency1}
&\max_{i=1,\cdots m}\|\tilde{\bV}_i-\bTheta_i\|_F\leq \frac{2\left(3\sigma\sqrt{dmr\log m}+36\sigma^2d\sqrt{rm}\right)}%{m-2\|\bW\|(2\sqrt{r}+1)-2}.
{m-3\sigma\sqrt{dm}(4\sqrt{r}+1)-1}.
\end{align}
Thus, if $\sigma = o\left(\frac{m^{1/4}}{\sqrt{dr}}\right)$, then  $\max_{i=1,\cdots m}\|\tilde{\bV}_i-\bTheta_i\|_F \to 0$ as $m\to\infty$.
\end{corollary}
\begin{remark}
For the MAXDIFF model, \eqref{eq:consistency1} is replaced with
\[
\max_{i=1,\cdots m}\|\tilde{\bV}_i-\bTheta_i\|_F\leq\frac{6\sigma\sqrt{dmr\log m}+\frac{72\sigma^2dm\sqrt{rm}}{m-2}}{m-\frac{12\sigma\sqrt{dm^3r}}{m-2}}.
\]
The bound follows from the discussion of Lemma~\ref{lemma:pertubation} in the MAXDIFF setting. If $\sigma = o\left(\frac{m^{1/4}}{\sqrt{dr}}\right)$, then  $\max_{i=1,\cdots m}\|\tilde{\bV}_i-\bTheta_i\|_F \to 0$ as $m\to\infty$. 
\end{remark}

==> sections/03-mainresult2.tex <==
\subsection{Theoretical guarantees on local optimal solutions}\label{sec:mainresults:local}
This section presents the condition on the size of the noise $\bW$ that ensures locally optimal points of problem  \eqref{eqn:tracemax} are in fact globally optimal.  We begin with two deterministic conditions on $\bW$ in Theorem~\ref{thm:main2} and Corollary~\ref{cor:discordant},  show that the condition in Corollary~\ref{cor:discordant} holds with high probability under the additive Gaussian model~\eqref{eq:noise_model} in Corollary~\ref{cor:gaussian}, and establish the consistency in \Cref{prop:consistencylocal}. %without finding such a point.

Recall that the first-order necessary condition for local optimality of \eqref{eqn:tracemax} is given in equation \eqref{eqn:firstorder}. 
The associated Lagrange multiplier is symmetric:
\begin{equation}\label{eqn:lagrange0}
	\bLambda_i = \bO_i^T\big(\sum_{j=1}^m\bS_{ij}\bO_j\big) 
	= \big(\sum_{j=1}^m\bS_{ij}\bO_j\big)^T\bO_i
	.
\end{equation}
%Substituting this quantity in equation \eqref{eqn:firstorder}, we obtain
%\begin{align}\label{eqn:firstorder2}
%	\bO_i\big(\sum_{j\neq i}\bS_{ij}\bO_j\big)^T\bO_i = \sum_{j\neq i} \bS_{ij}\bO_i, 
%	\quad i=1,\dotsc,m.
%\end{align}
%
\iffalse
The second-order necessary condition for local optimality of \eqref{eqn:tracemax} is 
\begin{equation}\label{eqn:second}
\sum_{i=1}^m \tr(\bLambda_i\bW_i^T\bW_i) - \tr(\bT^T\bS\bT) \ge 0
\end{equation}
for all $\bW_i$ such that
\begin{equation}\label{eqn:tangent}
\bT_i^T\bO_i + \bO_i^T\bT_i = \mathbf{0}, \quad i=1,\dotsc,m,
\end{equation}
and $\bT=[\bT_1^T, \dotsc, \bT_m^T]$, 
where the block matrix $\bS$ is defined in equation \eqref{eqn:blockS}.
%The $\bLambda_i$ is defined in equation \eqref{eqn:lagrange}.
In the sequel, we call a point $\bO=(\bO_1,\dotsc,\bO_m)$ that satisfies both the first- and second-order local optimality conditions a \emph{second-order critical point}. 
%
The subsequent results concern second-order critical points.
\fi
%
{%\color{red}%
We call a point $\bO=(\bO_1,\dotsc,\bO_m)$ that satisfies the first-order local optimality condition a \emph{critical point}.
It has been shown that a necessary condition for global optimality of a critical point is that \emph{the $\bLambda_i$ in equation \eqref{eqn:lagrange0} is symmetric and positive semidefinite for all $i$} \citep{won2018orthogonal}.
(An algorithm for finding such a point is also provided in \citep{won2018orthogonal}.)
In the sequel, we call a critical point $\bO=(\bO_1,\dotsc,\bO_m)$ satisfying this necessary condition a \emph{candidate critical point}.
The subsequent results concern candidate critical points.%
}

%In order to satisfy condition \eqref{eqn:lowerbound3}, let us make an additional assumption on $\bO$:
We further assume the following qualification on $\bO$:
\begin{assumption}\label{assumption}
Point $\bO=(\bO_1, \dotsc, \bO_m)\in\times_{i=1}^m\mathcal{O}_{d_i,r}$ is a %second-order 
{candidate}
critical point such that
	\[
		\tr(\bTheta^T\bS\bTheta) \le \tr(\bO^T\bS\bO)
		.
	\]
\end{assumption}
%\noindent \textcolor{red}{\sout{This assumption is satisfied, e.g., if $\bO$ is a global optimum of \eqref{eqn:tracemax}.}}
Note this assumption rules out ``bad'' local maxima. 
The clean signal $\bTheta$ solves problem \eqref{eqn:tracemax} in the noiseless setting (see Proposition \ref{prop:noiseless}). ``Not too bad'' local maximizer $\bO$ should perform at least as good as $\bTheta$ in the presence of noise.
%Indeed, it can be shown that \emph{all} the second-order critical point makes $\tr(\bO^T\bS\bO) \ge 0$ (Proposition \ref{prop:qualification}).
Indeed, at \emph{all} the %second-order 
{candidate}
critical points the objective function of \eqref{eqn:tracemax} is uniformly bounded below by zero. To see this, since $\bO$ is a %second-order 
{candidate} critical point, 
%$\bLambda_i$ is symmetric and positive definite for $i=1, \dots, m$. (see \Cref{prop:positivity}). 
%Therefore $\sum_{i=1}^m\bLambda_i \psdge \bzero$.
$\sum_{i=1}^m\bLambda_i$ is symmetric and positive definite.
Then it follows
	$$
		0 \le \tr(\sum_{i=1}^m\bLambda_i)
		= \sum_{i=1}^m\sum_{j=1}^m\tr(\bO_i^T\bS_{ij}\bO_j) = \tr(\bO^T\bS\bO)
		.
	$$

The main theorem in this section is stated as follows, with the proof deferred to \Cref{sec:proofmain2:thm}:
\begin{theorem}\label{thm:main2}
If noise $\bW$ is small in the sense that
	\begin{align}\label{eqn:noiselevel}
	m &\ge
    \|\bW\|(4\sqrt{r}+1)
    + \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\sqrt{\frac{r}{m}}
    \nonumber\\
    & \quad
    + \frac{2{m}(\max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\sqrt{\frac{r}{m}})}{m - 4\|\bW\|\sqrt{r}}
    + 16\|\bW\|^2\frac{r}{m}
	,
	\end{align}
	then all the points $\bO=(\bO_1,\dotsc,\bO_m)$ satisfying Assumption \ref{assumption} are \emph{global optima} of \eqref{eqn:tracemax}.
\end{theorem}

Similar to \eqref{eq:condition_deterministic}, the left-hand side of the sufficient condition \eqref{eqn:noiselevel} for global optimality of a second-order local solution dominates its right-hand side as $m\to\infty$, if $\|\bW\|$ and $\max_{i=1,\dotsc,m}\|(\bW\bTheta)_i\|_F$ are bounded or increase slowly as $m$ increases.
Thus, we can expect that a %second-order local solution
{candidate critical point}
is a global optimum with high probability under the additive Gaussian model \eqref{eq:noise_model}, if $\sigma$ is small and the number of observation $m$ is large.

To prove this idea rigorously, we apply the notion of $\bTheta$-discordant noise  {(\Cref{def:discordance}) again}, and present a deterministic, non-asymptotic statement that simplifies the condition \eqref{eqn:noiselevel} in Theorem~\ref{thm:main2}. with the proof deferred to \Cref{sec:proof_discordant}:
\begin{corollary}\label{cor:discordant}
Let $d=D/m$. Suppose that $m\geq 2$, 	\begin{equation}\label{eq:cor:discordant}
	\sigma \le \frac{m^{1/4}}{31\sqrt{dr}},
	\end{equation}
	and $\sigma^{-1}\bW$ is $\bTheta$-discordant, then \eqref{eqn:noiselevel} holds, and all the points $\bO=(\bO_1,\dotsc,\bO_m)$ satisfying Assumption \ref{assumption} are global optima of \eqref{eqn:tracemax}.
\end{corollary}

Finally, since Corollary~\ref{cor:probablistic_gaussian} shows that $\bW$ in the additive Gaussian noise model \eqref{eq:noise_model} is $\bTheta$-discordant,  Corollary~\ref{cor:discordant} implies following result on the probabilistic model:
\begin{corollary}\label{cor:gaussian}
	Suppose the additive Gaussian noise model in \eqref{eq:noise_model}.
	If $\sigma \le \frac{m^{1/4}}{31\sqrt{rd}}$ and $m\ge 3$ or $m \ge 2$ and $\min_{i=1,\dotsc, m}d_i \ge 6$, then with probability at least $1-1/m-2\exp\left(-\frac{(3-2\sqrt{2})^2}{4}D\right)$, all the points $\bO=(\bO_1,\dotsc,\bO_m)$ satisfying Assumption \ref{assumption} are global optima of \eqref{eqn:tracemax}.
\end{corollary}
\begin{remark}\label{rem:maxdifflocal0}
    The upper bound of $\sigma$ in the RHS of \eqref{eq:cor:discordant} can be made smaller if $m$ increases. For example, if we have $m \ge 4$, the \eqref{eq:cor:discordant} can be relaxed to $\sigma \le \frac{m^{1/4}}{29\sqrt{dr}}$; if $m \ge 9$, $\sigma \le \frac{m^{1/4}}{26\sqrt{dr}}$ suffices.
\end{remark}

\begin{remark}\label{rem:maxdifflocal}
    If instead the MAXDIFF model is assumed, the present analysis holds for $m \ge 4$ and \eqref{eq:cor:discordant} replaced with $\sigma \le \frac{m^{1/4}}{64\sqrt{dr}}$.
    This is a worse bound as opposed to $\frac{m^{1/4}}{29\sqrt{dr}}$ for MAXBET (See Remark~\ref{rem:maxdifflocal0}).
    To obtain the same bound as \eqref{eq:cor:discordant}, we need $m \ge 9$; see \Cref{sec:proof:maxdiff}.
    Similar to the SDP relaxation, the more restrictive bound in the MAXDIFF model is expected since MAXDIFF utilizes less information on the clean signal $\bTheta$ for the same number of measurements.
\end{remark}

{ %
%\subsubsection*{Consistency of estimation}
    %Another important theoretical question is whether the solution to \eqref{eqn:tracemax} recovers the true signal $\bTheta$ if $m$ is sufficiently large. 
    The following consistency result is a by-product of the proof of \Cref{thm:main2}. 
    Recall that problem \eqref{eqn:tracemax} is invariant to ``simultaneous rotation,'' i.e., post-multiplying a fully orthogonal matrix $\bQ\in\mathcal{O}_{r,r}$ to $\bO_i$'s (see, e.g., \cite[Eq. (8.2)]{wang2013orientation}):
    %and answers this question affirmatively:
    \begin{corollary}\label{prop:consistencylocal}
            Let $(\bO_1, \dotsc, \bO_m)\in\times_{i=1}^m\mathcal{O}_{d,r}$ be a %second-order critical point of problem \eqref{eqn:tracemax} 
            point
            satisfying Assumption \ref{assumption}. If the noise $\sigma^{-1}\bW$ is $\bTheta$-discordant and  
            $m > 144\sigma^2dr$, we have an estimation error
\[      	   \min_{\bQ\in\mathcal{O}_{r,r}}  \max_{1\le i\le m}\|\bO_i\bQ - \bTheta_i\|_F \le
	        \frac{2\left(3\sigma\sqrt{\frac{dr\log m}{m}} + 36\sigma^2d\sqrt{\frac{r}{m}}\right)}{1 - 12\sigma\sqrt{\frac{dr}{m}}}
	        .
\]	   
          
    \end{corollary}
%The fully orthogonal matrix $\bQ\in\mathcal{O}_{r,r}$ appears since problem \eqref{eqn:tracemax} is invariant to ``simultaneous rotation of all $\bO_i$'s.''    
Thus if $\sigma = o\left(\frac{m^{1/4}}{\sqrt{dr}}\right)$ then we have $\min_{\bQ\in\mathcal{O}_{r,r}} \max_{1\le i\le m}\|\bO_i\bQ - \bTheta_i\|_F \to 0$
as $m\to\infty$, as desired.
\begin{remark}
            If the MAXDIFF model is assumed,  $m > 2$, and $m^{3/2} - 2m^{1/2} - 12\sigma\sqrt{dr}m - 3 > 0$, then 
\[            
	   \min_{\bQ\in\mathcal{O}_{r,r}} \max_{1\le i\le m}\|\bO_i\bQ - \bTheta_i\|_F \le
        \frac{2\left(3\sigma\sqrt{\frac{dr\log m}{m}} + 36\sigma^2\frac{d\sqrt{r}}{\sqrt{m}-2/\sqrt{m}}\right)}{1 - 12\sigma\frac{\sqrt{dr}}{\sqrt{m}-2/\sqrt{m}}-\frac{3}{m}}
        .
\]	     
\end{remark}
}
% \begin{remark}\label{rem:maxdifflocal2}
%     Under the MAXDIFF model, 
% %     inequality \eqref{eqn:concentrationlocal} is replaced by
% % \[
% % 	\Pr{\left(\max_{i=1,\dotsc,m}\|(\bW\bTheta)_i\|_{\rm F} \le \sigma(\sqrt{\underline{d}r(m-1)} + r\sqrt{m-1} + 2\sqrt{r\log m})\right)} > 1 - \frac{1}{m}
% % 	,
% % \]
% % and inequality \eqref{eqn:concentration_discordance} holds for $m \ge 2$ for all $\underline{d}$, since $m - 1 \le m\log m$ for all $m \ge 2$.
% %     Thus 
%     the conclusion of \Cref{cor:gaussian} holds without modification, provided that $m \ge 4$ and $\sigma \le \frac{m^{1/4}}{64\sqrt{dr}}$;
%     also see \Cref{sec:proof:maxdiff}.
% \end{remark}

% \subsection*{Noiseless case}
% In the extreme case of $\bW=\bzero$, the condition \eqref{eqn:noiselevel} in Theorem \ref{thm:main} reduces to
% $$
% 	m > \max\left\{\sqrt{2mr} + 2r + \frac{2\sqrt{r}}{1-\sqrt{2r/m}}, 2r\right\}
% 	.
% $$
% %The solution of this inequality is given as
% %\begin{align*}
% 	%m > \max\{&2r^2, 
% 			%\\
% 			%&
% 			%\text{largest root of }
% 			%x^8 - 16x^7 + 96r^4x^6 - 272r^6x^5
% 			%+ (384r^8 - 2r)x^4 
% 			%\\
% 			%&\quad\quad\quad
% 			%- (256r^{10} + 16r^3)x^3
% 			%+ (64r^{12} + 32r^4)x^2 - 16r^7x + r^2
% 		%\}
% 	%.
% %\end{align*}
% For example, if $r=2$, this leads to $m \ge 18$; for $r=3$, we have $m \ge 21$.

% However, given the fact that $\bTheta$ is a global optimum if $\bW=\bzero$ (Proposition \ref{prop:noiseless}), Theorem \ref{thm:main} is a bit pessimistic.
% %\subsection{Noisy case}

\subsection{Comparison with existing works}
Our results generalize the work \cite{Bandeira2017} on angular synchronization, which analyzes the setting $d=r=1$ with complex values. In particular, Theorem~\ref{thm:main}, Corollary~\ref{cor:probablistic}, Corollary~\ref{cor:probablistic_gaussian}, and Corollary~\ref{cor:gaussian} are generalizations of Lemma 3.2, Theorem 2.1, and Proposition 4.5 in \cite{Bandeira2017} respectively. Corollary~\ref{cor:probablistic} is similar to Lemma 3.2 in \cite{Bandeira2017}, in the sense that both results establish deterministic conditions such that the original problem and the relaxed problem have the same solutions, under a ``discordant'' condition. In addition, Corollary~\ref{cor:probablistic_gaussian} is a generalization of~\cite[Theorem 2.1]{Bandeira2017}, in the sense that both results establish upper bounds on the size of noise $\sigma$ under an additive Gaussian model. At last, both Corollary~\ref{cor:gaussian} and Proposition 4.5 in \cite{Bandeira2017} show that local solutions satisfying an assumption are global optima.

Theorem 2.1 and Proposition 4.5 in \citep{Bandeira2017} require $\sigma\leq \frac{1}{18}m^{\frac{1}{4}}$. In comparison, Corollary~\ref{cor:probablistic_gaussian} and Corollary~\ref{cor:gaussian} require $\sigma\leq \frac{1}{60}m^{\frac{1}{4}}$ and $\sigma\leq \frac{1}{31}m^{\frac{1}{4}}$ under the setting $d=r=1$, so our result is only worse by a constant factor.  

The upper bound $\sigma\leq \frac{1}{18}m^{\frac{1}{4}}$ in~\cite[Theorem 2.1]{Bandeira2017} is later improved to  $\sigma\leq O(\sqrt{\frac{m}{\log m}})$ in \cite{ZhongBoumal18PhaseSynchNearOptimalBounds}, based on a much more complicated argument and an  algorithmic implementation. {  After finishing this work, we became aware of a recent manuscript \cite{ling2021improved}, which investigates the synchronization-of-rotations problem using the method in \cite{ZhongBoumal18PhaseSynchNearOptimalBounds}, and proves that the original problem and the relaxed problem   have the same solution when $\sigma\leq O(\frac{\sqrt{m}}{d+\sqrt{d}\log m})$. While it is better than our rate $\sigma\leq O(\frac{m^{1/2}}{d})$ when $r=d$, our analysis investigates a more generic problem where $r$ could be smaller than $d$, and \sout{our analysis} establishes deterministic conditions that can be verified for a variety of probabilistic models. In comparison, the method in \cite{ling2021improved} is specifically designed for the additive Gaussian noise model. } %We conjecture that by using a similar argument, we might also be able to improve the upper bound of $\sigma$ in  Corollary~\ref{cor:probablistic} to $\sigma\leq O(\sqrt{\frac{m}{\log m}})$, but it would be a much more involved argument and we leave it as a possible future project.

While the results in this section are generalizations of the results in \cite{Bandeira2017}, we remark that the generalization is not trivial. In particular, their proof cannot be extended to our setting directly due to the non-commutability of matrix products. To address this issue, we introduce a novel optimality certificate in Lemma~\ref{lemma:equavalency}, which is very different from the corresponding result in \cite[Lemma 4.4]{Bandeira2017}. 


==> sections/04-proofresult1.tex <==
\section{Proof of main results}\label{sec:proof}
\subsection{Proof of Theorem~\ref{thm:main}}\label{sec:proof_thm:main}
The proof of Theorem \ref{thm:main} can be divided into several components as follows. 


1. Lemma~\ref{lemma:stationary} shows that for each solution to OTSM, there exist two corresponding ``certificate'' variables of $\bT^{(1)}$ and $\bT^{(2)}\in\reals^{D\times D}$. In addition, Lemma~\ref{lemma:equavalency} establishes the conditions of $\bT^{(1)}$ and $\bT^{(2)}$, such that the solution to OTSM is also the solution to \eqref{eq:tracesum_relaxed}.

2. Lemma~\ref{lemma:clean} finds the ``clean'' values of $\bT^{(1)}$ and $\bT^{(2)}$ in the noiseless setting $\bW=0$, denoted by $\bT^{(1)*}$ and $\bT^{(2)*}$, and they satisfy the conditions in Lemma~\ref{lemma:equavalency}.

3. Lemmas~\ref{lemma:noisy}, ~\ref{lemma:noisy2} and~\ref{lemma:pertubation} show that when the noise $\bW$ is small, $\bT^{(1)}$ and $\bT^{(2)}$ do not deviate much from $\bT^{(1)*}$ and $\bT^{(2)*}$. As a result, the condition in Lemma~\ref{lemma:equavalency} holds for small $\bW$, and the solution to OTSM is also the solution to \eqref{eq:tracesum_relaxed}.
%
%First, Lemma~\ref{lemma:equivalent} establishes an equivalent formulation of \eqref{eqn:tracemax}, given in  \eqref{eq:tracesum_problem1}. 
%

% Based on this equivalent formulation, Lemma~\ref{lemma:stationary} shows the property that $\bS$ can be decomposed into {a sum of} two matrices, each with a certain property. Then, based on this decomposition, Lemma~\ref{lemma:equavalency} gives a condition such that the minimizer of \eqref{eq:tracesum_problem1} is also the unique solution to \eqref{eq:tracesum_relaxed}. It remains to verify this condition. Lemma~\ref{lemma:clean} analyzes the decomposition for the clean case that $\bW=\mathbf{0}$. Then using a perturbation argument, Lemmas~\ref{lemma:noisy}, ~\ref{lemma:noisy2}, and~\ref{lemma:pertubation} shows that when $\|\bW\|$ is small, the decomposition does not change much and the condition would still be satisfied. 


We first present our lemmas and a short proof of Theorem~\ref{thm:main} based on these lemmas, and leave the technical proofs of lemmas to Section~\ref{sec:proof_lemma}. 
%\begin{lemma}\label{lemma:equivalent}
%The optimization problem \eqref{eqn:tracemax} is equivalent to the problem 
%\begin{equation}\label{eq:tracesum_problem1}
%\tilde{\bU}=\max_{\bU\in\reals^{D\times D}, \bU=\bU^T}\tr(\bS\bU), \text{subject to $\bU\psdge \mathbf{0}, \bU_{ii}\psdle\bI, \tr(\bU_{ii})=r, \rank(\bU)=r$.}
%\end{equation}
%\end{lemma}


\begin{lemma}[Certificate variables of the \eqref{eqn:tracemax} problem]\label{lemma:stationary}
The solution to \eqref{eq:tracesum_problem1} satisfies the following property: let $\tilde{\bU}=\tilde{\bV}\tilde{\bV}^T$ with $\tilde{\bV}\in\reals^{D\times r}$, 
%\[
%\tilde{\bV}=\left[ \begin{array}{c}
%\tilde{\bV}_1\\
%\vdots\\
%\tilde{\bV}_m\\
% \end{array} \right],
%\]
then $\bS$ can be written as $\bS=\bT^{(1)}+\bT^{(2)}$, where $\bT^{(1)}$ is defined as follows: 
\begin{equation}\label{eq:tildeT1}
[\bT^{(1)}]_{ij}=\bS_{ij},\,\,\text{for $1\leq i\neq j\leq m$},\,\,[\bT^{(1)}]_{ii}=\bS_{ii}-\sum_{j=1}^m\bS_{ij}\tilde{\bV}_j\tilde{\bV}_i^T\,\,\text{for $1\leq i\leq m$}.
\end{equation}
$\bT^{(2)}$ has the property $\Proj_{\tilde{\bV}_i}\bT^{(2)}_{ii} \Proj_{\tilde{\bV}_i}=\bT^{(2)}_{ii}$, and is defined by 
\begin{equation}\label{eq:tildeT2}[\bT^{(2)}]_{ij}=\mathbf{0}\,\,\text{for $1\leq i\neq j\leq m$}, \,\,[\bT^{(2)}]_{ii}=\sum_{j=1}^m\bS_{ij}\tilde{\bV}_j\tilde{\bV}_i^T\,\,\text{for $1\leq i\leq m$}.\end{equation}

\end{lemma}

{%
\begin{remark}
That $\Proj_{\tilde{\bV}_i}\bT^{(2)}_{ii} \Proj_{\tilde{\bV}_i}=\bT^{(2)}_{ii}$ implies 
$\bT^{(2)}_{ii} = \tilde{\bV}_i\bLambda_i\tilde{\bV}_i^T$
for some symmetric matrix $\bLambda_i\in\mathbb{R}^{r\times r}$. In the proof of Lemma \ref{lemma:stationary}, it is shown
\[
    \sum_{j=1}^m\bS_{ij}\tilde{\bV}_j 
    = \bT^{(2)}_{ii}\tilde{\bV}_i
    = \tilde{\bV}_i\bLambda_i
    .
\]
This matrix $\bLambda_i = \sum_{j=1}^m\tilde{\bV}_i^T\bS_{ij}\tilde{\bV}_j$ is the Lagrange multiplier for the orthogonality constraint $\bO_i^T\bO_i=\bI_r$ in the original problem \eqref{eqn:tracemax} \citep{won2018orthogonal}.
%It can be shown that, at the solution, $\bLambda_i$ is positive semidefinite. 
{Recall that, at the solution, $\bLambda_i$ is positive semidefinite.}
\end{remark}
}

\begin{lemma}[Conditions of the certificate variables for the equivalence between \eqref{eqn:tracemax} and \eqref{eq:tracesum_relaxed}]\label{lemma:equavalency}
If there exists a decomposition $\bS=\hat{\bT}^{(1)}+\hat{\bT}^{(2)}+c\bI$ such that $\Proj_{\tilde{\bV}^\perp}\hat{\bT}^{(1)}\Proj_{\tilde{\bV}^\perp}=\hat{\bT}^{(1)}$,  $\hat{\bT}^{(2)}_{ii}=\Proj_{\tilde{\bV}_i}\hat{\bT}^{(2)}_{ii} \Proj_{\tilde{\bV}_i}$ for all $1\leq i\leq m$,  $\{P_{\tilde{\bV}_i}^T\hat{\bT}^{(2)}_{ii} P_{\tilde{\bV}_i}\}_{i=1}^m$, and $-P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ are  positive definite matrices. %The 
{Then,}
$\tilde{\bU}$, the solution to \eqref{eq:tracesum_relaxed}, is also the unique solution to \eqref{eq:tracesum_problem1}.
\end{lemma}

\begin{lemma}[Certificate variables in the noiseless setting]\label{lemma:clean}
Denote $\bT^{(1)}$ generated by \eqref{eq:tildeT1} and \eqref{eq:tildeT2} under the case $\bW=\mathbf{0}$ as $\bT^{(1)*}$. Let $L_1=\Sp(\bTheta)$ and $L_2=\{\bx\in\reals^D: \bx_i\in\Sp(\bTheta_i)\}$, then  $\bT^{(1)*}=-m\Proj_{L_2\cap L_1^\perp}$. That is, \begin{equation}\label{eq:tildeTstar10}
[\bT^{(1)*}]_{ij}=\bTheta_i\bTheta_j^T\,\,\text{for $i\neq j$}, [\bT^{(1)*}]_{ii}=-(m-1){\bTheta}_i{\bTheta}_i^T.
\end{equation} 

\end{lemma}
\begin{lemma}[Certificate variables in the noisy setting]\label{lemma:noisy2}
If $m$ satisfies the following inequality
\begin{equation}\label{eq:noisy2_0}\frac{m}{2}
\geq \max_{1\leq i\leq m}\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+2m\max_{1\leq i\leq m}\|\tilde{\bV}_i-\bTheta_i\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|+\|\bW\|
,
\end{equation} then there exists  $c$, $\hat{\bT}^{(1)}$ and $\hat{\bT}^{(2)}$ such that the conditions in Lemma~\ref{lemma:equavalency} are satisfied, that is, $\bS=\hat{\bT}^{(1)}+\hat{\bT}^{(2)}+c\bI$, $\Proj_{\tilde{\bV}^\perp}\hat{\bT}^{(1)}\Proj_{\tilde{\bV}^\perp}=\hat{\bT}^{(1)}$, $\hat{\bT}^{(2)}_{ii}=\Proj_{\tilde{\bV}_i}\hat{\bT}^{(2)}_{ii} \Proj_{\tilde{\bV}_i}$ for all $1\leq i\leq m$, and $\{P_{\tilde{\bV}_i}^T\hat{\bT}^{(2)}_{ii} P_{\tilde{\bV}_i}\}_{i=1}^m$ and $-P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ are  positive definite matrices.
\end{lemma}
\begin{lemma}[Perturbation of the certificate variables]\label{lemma:noisy}
\begin{align}
&\|\bT^{(1)*}-\bT^{(1)}\|\leq m\max_{1\leq i\leq m}\|\tilde{\bV}_i-\bTheta_i\|+\max_{1\leq i\leq m}\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|+\|\bTheta^T\tilde{\bV}-m\bI\|
+ \|\bW\|
,\label{eq:noisy1}\\
&\text{$\|\tilde{\bV}_i^T[\bT^{(2)}]_{ii}\tilde{\bV}_i-m
\bI\|<\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+m\|\tilde{\bV}_i^T\bTheta_i-\bI\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|$ for all $1\leq i\leq m$\label{eq:noisy2}.}
\end{align}
\end{lemma}
\begin{lemma}[Perturbation of the solutions of OTSM]\label{lemma:pertubation}
%{If $m > 2\|\bW\|(2\sqrt{r}+1)+2$},
 {If $m > \|\bW\|(4\sqrt{r}+1)+1$},
then
the solution of \eqref{eq:tracesum_problem1}, $\tilde{\bU}$, admits a decomposition $\tilde{\bU}=\tilde{\bV}\tilde{\bV}^T$ with $\tilde{\bV}\in\reals^{D\times r}$, such that% $\tilde{\bV}$ is close to $\bV$ in the sense that 
\begin{align}\label{eq:lemma_pertubation1}
&\|\tilde{\bV}-\bTheta\|_F\leq 4\|\bW\|\sqrt{\frac{r}{m}},  \,\,\,\max_{1\leq i\leq m}\|[\bW\tilde{\bV}]_i\|_F\leq \max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+4\|\bW\|^2\sqrt{\frac{r}{m}}, \\ &\max_{i=1,\cdots m}\|\tilde{\bV}_i-\bTheta_i\|_F\leq \frac{2\left(\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+4\|\bW\|^2\sqrt{\frac{r}{m}}\right)}%{m-2\|\bW\|(2\sqrt{r}+1)-2}.
{ m-\|\bW\|(4\sqrt{r}+1)-1}
\label{eq:lemma_pertubation2}
\end{align}
\end{lemma}


\begin{proof}[Proof of Theorem~\ref{thm:main}]
Lemma~\ref{lemma:equavalency}  and Lemma~\ref{lemma:noisy2} implies that to prove Theorem~\ref{thm:main}, it is sufficient to prove \eqref{eq:noisy2_0}, which can be verified by applying  Lemma~\ref{lemma:pertubation}.
\end{proof}
\subsection{Proof of Corollary~\ref{cor:probablistic}}\label{sec:proof_cor:probablistic}
\begin{proof}[Proof of Corollary~\ref{cor:probablistic}]
% Under this setting, %$\bW$ can be generated by $\bW=\bW^{(1)}+\bW^{(2)}$, where $\bW^{(1)}\in\reals^{D\times D}$ is i.i.d. generated from $N(0,\sigma^2/2)$, and $\bW^{(2)}$ is generated as follows: $[\bW^{(2)}]_{ii}$ is i.i.d. from $N(0,\sigma^2/2)$ and is independent of $\bW^{(1)}$, and $[\bW^{(2)}]_{ij}=[\bW^{(1)}]_{ji}^T$ for $i\neq j$. As a result, both $\bW^{(1)}$ and $\bW^{(2)}$ are i.i.d. sampled from $N(0,\sigma^2/2)$, and
% ~\cite[Theorem II.13]{Szarek:survey} implies that 
% % \[
% % \Pr\left(\frac{\sqrt{2}}{\sigma}\|\bW^{(1)}\|\geq 2\sqrt{D}+t\right)=\Pr\left(\frac{\sqrt{2}}{\sigma}\|\bW^{(2)}\|\geq 2\sqrt{D}+t\right)<e^{-t^2/2}.
% % \] 
% % Combining the estimation for $\bW^{(1)}$ and $\bW^{(2)}$ and use $t=\sqrt{D}$,
% \begin{equation}\label{eq:proba1}
% \Pr\left(\|\bW\|\geq 3\sqrt{D}\sigma\right)\leq 2e^{-D/2}.
% \end{equation} 


% It remains to estimate $\|[\bW{\bTheta}]_i\|_F$. %we note that $\|[\bW{\bTheta}]_i\|_F\leq \|[\bW^{(1)}{\bTheta}]_i\|_F+\|[\bW^{(2)}{\bTheta}]_i\|_F$. To estimate $\|[\bW^{(1)}{\bTheta}]_i\|_F$, 
% Since $\bW$ is i.i.d. Gaussian, without loss of generality we may assume that $\bTheta_i=[\bI_{r\times r};\mathbf{0}_{(d_i-r)\times r}]$, that is, $\bTheta_i$ consists of an $r\times r$ identity matrix and an $(d_i-r)\times r$ zero matrix. \st{Then calculation shows that $[\bW\bTheta]_i$ is a matrix of size $d_i\times r$ that can be written as $[\bG_{r\times r}; \mathbf{0}_{(d_i-r)\times r}]$, and $\bG$ is i.i.d. sampled from $N(0,\sigma^2m)$} ({\color{red} Here $[\bW\bTheta]_i$ should be a matrix of size $d_i\times r$ that is i.i.d. from $N(0,m\sigma^2)$, so \eqref{eq:condition_deterministic1} should be replaced with \eqref{eqn:concentrationlocal}}). As a result, applying~\cite[Proposition 2.2]{measure2005} we have 
% \[
% \Pr\left(\frac{1}{\sigma^2m}\|[\bW\bTheta]_i\|_F^2>r^2+\delta\right)\leq \left(\frac{r^2}{r^2+\delta}\right)^{-r^2/2} e^{-\delta/2}
% \]
% and a union bound over $1\leq i\leq m$ implies\[
% \Pr\left(\frac{1}{\sigma^2m}\max_{1\leq i\leq m}\|[\bW\bTheta]_i\|_F^2>r^2+\delta\right)\leq m\left(\frac{r^2}{r^2+\delta}\right)^{-r^2/2} e^{-\delta/2}.
% \]
% %Combining it with the estimation for $\|[\bW^{(2)}\bTheta]_i\|_F$ (which is the same as $\|[\bW^{(1)}\bTheta]_i\|_F$), and 
% Let $\delta=2\log m$ we have
% \begin{equation}\label{eq:proba2}
% \Pr\left(\frac{1}{\sigma^2m}\max_{1\leq i\leq m}\|[\bW\bTheta]_i\|_F^2>r^2+2\log m\right)\leq 2\left(\frac{r^2}{r^2+2\log m}\right)^{-r^2/2}.
% \end{equation}
% Combining the estimations \eqref{eq:proba1} and \eqref{eq:proba2},  \eqref{eq:condition_deterministic} holds with probability at least $1-2\left(\frac{r^2}{r^2+2\log m}\right)^{-r^2/2}-2e^{-D/2}$, if
% \begin{equation}\label{eq:condition_deterministic1}
% m>4m\frac{2\left((\sigma\sqrt{m}(r^2+2\log m))+36D\sigma^2\sqrt{\frac{r}{m}}\right)}{m-6\sigma\sqrt{D}(2\sqrt{r}+1)-2}+2\left((\sigma\sqrt{m}(r^2+2\log m))+36D\sigma^2\sqrt{\frac{r}{m}}\right)+24\sigma\sqrt{\frac{Dr}{m}}+6\sigma\sqrt{D}.\end{equation}
% %which can be verified to hold 
% %Let $d_1, \cdots, d_m, r$ be fixed and $m$ goes to infinity, the Corollary is proved.

% Plug in $d=\sum_{i=1}^md_i/m$, $D=dm$, and $\sigma<\frac{1}{17r^{\frac{1}{4}}d^{\frac{1}{2}}} m^{1/4}$, as $d, r$ be fixed and $m\rightarrow\infty$, the dominant term in the RHS of \eqref{eq:condition_deterministic1} is the term with order $O(\sqrt{m}\sigma^2)$: 
% \begin{align*}
% &4m\frac{72D\sigma^2\sqrt{\frac{r}{m}}}{m-6\sigma\sqrt{D}(2\sqrt{r}+1)-2}\leq 4m\frac{72m \frac{1}{289} }{m-6\frac{1}{17r^{\frac{1}{4}}d^{\frac{1}{2}}} m^{1/4}\sqrt{dm}(2\sqrt{r}+1)-2}\\=& \frac{288}{289} \frac{m^2}{m-6\frac{1}{17r^{\frac{1}{4}}d^{\frac{1}{2}}} m^{1/4}\sqrt{dm}(2\sqrt{r}+1)-2},
% \end{align*}
% and since the denominator is approximately $m$ as $m\rightarrow\infty$, \eqref{eq:condition_deterministic1} holds and the Corollary~\ref{cor:probablistic} is proved.
% \end{proof}


Under the $\bTheta$-discordant property, inequality \eqref{eq:condition_deterministic} is satisfied if
\[
m > \frac{8m[3\sigma\sqrt{drm\log m} + 36\sigma^2d\sqrt{rm}]}{m - 2 - 6\sigma\sqrt{dm}(2\sqrt{r}+1)}
+ 2[3\sigma\sqrt{drm\log m} + 36\sigma^2d\sqrt{rm}]
+ 24\sigma\sqrt{dr}
+ 6\sigma\sqrt{dm}
.
\]
Dividing both sides of the above inequality by $m$, we have
\begin{align*}
    1 > \left( 2 + \frac{8}{1 - 2 / m - 6\sigma\sqrt{d/m}(2\sqrt{r}+1)}\right)
    \left[3\sigma\sqrt{dr}\sqrt{\frac{\log m}{m}} + 36\sigma^2\frac{d\sqrt{r}}{\sqrt{m}}\right]
    + 24\sigma\frac{\sqrt{dr}}{m}
    + 6\sigma\frac{\sqrt{d}}{\sqrt{m}}
    .
\end{align*}
If 
\[
    \sigma \le \frac{m^{1/4}}{\alpha\sqrt{dr}}
    ,
\]
then the RHS of the above inequality is upper-bounded by
\begin{align*}
    &\left( 2 + \frac{8}{1 - \frac{2}{m} - \frac{6}{\alpha}\frac{2\sqrt{r}+1}{\sqrt{r}}\frac{1}{m^{1/4}}}\right)
    \left[\frac{3}{\alpha}\frac{\sqrt{\log m}}{m^{1/4}} + \frac{36}{\alpha^2}\frac{1}{\sqrt{r}}\right]
    + \frac{24}{\alpha}\frac{1}{m^{3/4}}
    + \frac{6}{\alpha}\frac{1}{\sqrt{r}}\frac{1}{m^{1/4}}
    \\
    &\le
    \left( 2 + \frac{8}{1 - \frac{2}{m} - \frac{18}{\alpha}\frac{1}{m^{1/4}}}\right)
     \left[\frac{3}{\alpha}\frac{\sqrt{\log m}}{m^{1/4}} + \frac{36}{\alpha^2}\right]
    + \frac{24}{\alpha}\frac{1}{m^{3/4}}
    + \frac{6}{\alpha}\frac{1}{m^{1/4}}     
\end{align*}
since $r \ge 1$ and $\frac{2\sqrt{r}+1}{\sqrt{r}} \le 3$.
The last line is decreasing in $m$ if $m \ge 8$. Hence if
\[
    \left( 2 + \frac{8}{1 - \frac{2}{8} - \frac{18}{\alpha}\frac{1}{8^{1/4}}}\right)
     \left[\frac{3}{\alpha}\frac{\sqrt{\log 8}}{8^{1/4}} + \frac{36}{\alpha^2}\right]
    + \frac{24}{\alpha}\frac{1}{8^{3/4}}
    + \frac{6}{\alpha}\frac{1}{8^{1/4}}     
    < 1
\]
and
\[
    1 - \frac{2}{8} - \frac{18}{\alpha}\frac{1}{8^{1/4}} > 0
\]
for some $\alpha > 0$, we are done. Indeed, for $\alpha=60$, we have 
\[
    \left( 2 + \frac{8}{1 - \frac{2}{8} - \frac{18}{\alpha}\frac{1}{8^{1/4}}}\right)
     \left[\frac{3}{\alpha}\frac{\sqrt{\log 8}}{8^{1/4}} + \frac{36}{\alpha^2}\right]
    + \frac{24}{\alpha}\frac{1}{8^{3/4}}
    + \frac{6}{\alpha}\frac{1}{8^{1/4}}     
    \approx 0.98925
\]
and
\[
    1 - \frac{2}{8} - \frac{18}{\alpha}\frac{1}{8^{1/4}} \approx 0.57162
    .
\]
\end{proof}
\begin{remark}If $m < 8$, the $\frac{\sqrt{\log m}}{m^{1/4}}$ has the maximum value of $\sqrt{2/e}$ at $m=e^2\approx7.39$. Thus we require
\[
    \left( 2 + \frac{8}{1 - \frac{2}{m_0} - \frac{18}{\alpha}\frac{1}{m_0^{1/4}}}\right)
     \left[\frac{3}{\alpha}\sqrt{\frac{2}{e}} + \frac{36}{\alpha^2}\right]
    + \frac{24}{\alpha}\frac{1}{m_0^{3/4}}
    + \frac{6}{\alpha}\frac{1}{m_0^{1/4}}     
    < 1
\]
for the smallest allowed value $m_0$ of $m$. Brute-force computation gives the following.
\\
\begin{center}
\begin{tabular}{rr}
$m_0$ & $\alpha$ \\
\midrule
3   & 124 \\
4   & 87  \\
5   & 74  \\
6   & 67  \\
7   & 63  \\
8   & 60
\end{tabular}
\end{center}
The last row is duplicated for ease of reference.
\end{remark}

\subsection{Proof of Corollary~\ref{cor:probablistic_gaussian}}\label{sec:proof_cor:probablistic_gaussian}
\begin{proof}[Proof of Corollary~\ref{cor:probablistic_gaussian}]
Considering \Cref{cor:probablistic}, it is sufficient to show that Gaussian noise $\bW$ satisfies the $\bTheta$-discordance with high probability under the MAXBET model.
Assume $\sigma^{-1}\bW_{ij}$ has i.i.d. standard normal entries. Then from $[\bW\bTheta]_i=\sum_{j=1}^m\bW_{ij}\bTheta_j\in\mathbb{R}^{d_i\times r}$, it is obvious that this matrix has zero-mean normal entries. To see the variance, note
$$
	\vec(\bW_{ij}\bTheta_j) = \vec(\bI_{d_i}\bW_{ij}\bTheta_j) 
	= (\bTheta_j^T\otimes\bI_{d_i})\vec(\bW_{ij})
	.
$$
Then $\Cov(\vec(\bW_{ij}))=\sigma^2\bI_{d_id_j}$ and
\begin{align*}
	\Cov(\vec(\bW_{ij}\bTheta_j))
	&= \sigma^2(\bTheta_j^T\otimes\bI_{d_i})(\bTheta_j^T\otimes\bI_{d_i})^T
	\\
	&= \sigma^2(\bTheta_j^T\otimes\bI_{d_i})(\bTheta_j\otimes\bI_{d_i})
	\\
	&= \sigma^2(\bTheta_j^T\bTheta_j\otimes\bI_{d_i}\bI_{d_i})
	\\
	&= \sigma^2(\bI_r\otimes\bI_{d_i})
	= \sigma^2\bI_{rd_i}
	,
\end{align*}
i.e., $\bW_{ij}\bTheta_j$ has i.i.d. normal entries with variance $\sigma^2$.
Then $[\bW\bTheta]_i$ is the sum of $m$ i.i.d. copies of $\bW_{ij}\bTheta_j$, hence entries have variance $m\sigma^2$.
Now from Theorem 9.26 of \cite{Foucart2013},
$$
	\Pr{\left(\frac{1}{\sigma\sqrt{m}}\|[\bW\bTheta]_i\| \ge \sqrt{d_i} + \sqrt{r} + t\right)} \le e^{-t^2/2}
$$
for $t \ge 0$.
Applying the union bound and noting that $\frac{1}{\sqrt{r}}\|[\bW\bTheta]_i\|_F \le \|(\bW\bTheta)_i\|_2$, we obtain
$$
	\Pr{\left(\max_{i=1,\dotsc,m}\|[\bW\bTheta]_i\|_F \le \sigma(\sqrt{\underline{d}rm} + r\sqrt{m} + t\sqrt{r})\right)} > 1 - me^{-t^2/2}
	,
$$
where $\underline{d}=\min_{i=1,\dotsc,m} d_i$.
Now choose $t$ such that $e^{-t^2/2}=1/m^2$, i.e., $t=2\sqrt{\log m}$. Then, 
\begin{equation}\label{eqn:concentrationlocal}
	\Pr{\left(\max_{i=1,\dotsc,m}\|[\bW\bTheta]_i\|_F \le \sigma(\sqrt{\underline{d}rm} + r\sqrt{m} + 2\sqrt{r\log m})\right)} > 1 - \frac{1}{m}
	.
\end{equation}
%Since $\underline{d}\ge \sqrt{\underline{d}r} \ge r \ge 2$, $m \ge 2$, and $m-1 \le m\log m$, we have
Since $\underline{d}\ge \max\{r, 2\}$ and $m \ge 2$, we have $r \le \sqrt{\underline{d}r}$ and $\sqrt{\underline{d}m} \ge 2$. 
Furthermore, if $m \ge 3$, then $m \le m\log m$.
Thus
\begin{align}\label{eqn:concentration_concordance}
 &\sqrt{\underline{d}rm} + r\sqrt{m} + 2\sqrt{r\log m}
 \nonumber\\
 &\le 
 \sqrt{\underline{d}rm\log m} + \sqrt{\underline{d}r}\sqrt{m\log m} + \sqrt{\underline{d}m}\sqrt{r\log m}
 \le
 3\sqrt{\underline{d}rm\log m}
 \le
 3\sqrt{Dr\log m}
 .
\end{align}
If $m=2$,  
\begin{align*}
\sqrt{\underline{d}rm} + r\sqrt{m} + 2\sqrt{r\log m}
= 
\sqrt{2\underline{d}r} + \sqrt{2r^2} + 2\sqrt{r\log 2}
&\leq
\sqrt{2\underline{d}r} + \sqrt{2\underline{d}r} + 2\sqrt{r\log 2}
\\
&\leq
3\sqrt{2\underline{d}r\log 2}
\leq
3\sqrt{Dr\log 2}
\end{align*}
if $\underline{d} \ge 6$.
Thus if  $m\ge 3$ or $m \ge 2$ and $\underline{d} \ge 6$, then
$$
	\max_{i=1,\dotsc,m}\|[\textstyle\frac{1}{\sigma}\bW\bTheta]_i\|_F \le 3\sqrt{Dr\log m}
$$
with probability at least $1 - 1/m$.

To bound $\|\bW\|$, using the same argument as in Corollary \ref{cor:probablistic}, we have
%\citet{Zhang2019}, we have
$$
	\Pr{\left(\|\bW\| \le \sigma\sqrt{2}(2\sqrt{D}+t)\right)} > 1 - 2e^{-t^2/2}
$$
for $t \ge 0$. Choose $t=(\frac{3}{\sqrt{2}}-2)\sqrt{D}$ to have
$$
	\Pr{\left(\|\bW\| \le 3\sigma\sqrt{D}\right)} > 1 - 2e^{-\frac{(3-2\sqrt{2})^2}{4}D}
	.
$$
\end{proof}
\subsection{Proof of \Cref{cor:consistency1}}
The proof follows from \eqref{eq:lemma_pertubation2} in \Cref{lemma:pertubation} and \Cref{cor:probablistic}.

==> sections/05-proofresult2.tex <==
%\section{Proof of main result 2}\label{sec:proofmain2}
\subsection{Proof of \Cref{thm:main2}}\label{sec:proofmain2:thm}
%We present the main result, Theorem~\ref{thm:main}, in the last part of this section. It shows that any local solution of \eqref{eqn:tracemax} are also its global solution. 
As a preparation, we provide intermediate results first. Proofs of these results are provided in Section \ref{sec:proofs}.  
\iffalse
It was shown that positive semidefiniteness of the Lagrange multipliers $\bLambda_i$ is a necessary condition for second-order local optimality: %\citep{won2018orthogonal}: 
%We begin with that this is also a necessary condition for second-order local optimality:
\begin{proposition}[\citep{won2018orthogonal}]\label{prop:positivity}
% 	If $\bO=(\bO_1,\dotsc,\bO_m)$ is a second-order critical point,
% 	then $\bLambda_i$ as defined in equation \eqref{eqn:lagrange0} is positive semidefinite, for all $i=1,\dotsc,m$.
{\color{red}%
	If $\bO=(\bO_1,\dotsc,\bO_m)\in\mathcal{O}_{d_1,r}\times \cdots \times\mathcal{O}_{d_m,r}$ is a 	local maximizer of
	\eqref{eqn:tracemax},
		then $\bLambda_i$ as defined in equation \eqref{eqn:lagrange0} is positive semidefinite, for 		$i \in \{1, \dotsc, m\}$ such that $d_i > r$.
	If $\bO$ is a stationary point but $\bLambda_i$ is not positive semidefinite for some $i$, then one can find another stationary point $\tilde{\bO}=(\tilde{\bO}_1, \dotsc, \tilde{\bO}_m)$ such that $\frac{1}{2}\sum_{i,j}\tr(\bO_i\bS_{ij}\bO_j) < \frac{1}{2}\sum_{i,j}\tr(\tilde{\bO}_i\bS_{ij}\tilde{\bO}_j)$ and $\tilde{\bLambda}_i=\tilde{\bO_i}^T\sum_{j=1}^m\bS_{ij}\tilde{\bO}_j$ is positive semidefinite for all $i=1,\dotsc,m$.
	Furthermore, if $\bO$ is a global maximizer of \eqref{eqn:tracemax}, then $\bLambda_i$ is positive semidefinite for all $i$. %
}
\end{proposition}
\fi
\iffalse
The following result is not directly used in the proof, but qualifies a critical point:
\begin{proposition}\label{prop:qualification}
	If $(\bO_1,\dotsc,\bO_m)\in\Gamma$ is a second-order critical point,
	then for block matrix $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$,
	$\tr(\bO^T\bS\bO) \ge 0$.
\end{proposition}
\fi

Results similar to \Cref{lemma:noisy} are obtained as follows.
\begin{lemma}\label{lem:weyllocal}
    Let $\bLambda_i$ be the Lagrange multiplier of a %\textcolor{red}{\sout{first-order}}
    critical point $(\bO_1, \dotsc, \bO_m)$ of problem \eqref{eqn:tracemax}. That is, it is a symmetric $r\times r$ matrix satisfying $\bO_i\bLambda_i=\sum_{j=1}^m\bS_{ij}\bO_j$.
    Then,
    for block matrices $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$ and 
    $\bTheta=[\bTheta_1^T, \dotsc, \bTheta_m^T]^T$,
    the following holds.
    \begin{align*}
    \|\bLambda_i - m\bI\| &\le
    \|\sum_{j=1}^m\bW_{ij}\bO_j\|
    + m\|\bO_i^T\bTheta_i - \bI_r\|
    + \|\bTheta^T\bO - m\bI_r\|
    \quad
    \text{(under MAXBET model)}
    ,
    \\
    \|\bLambda_i - (m-1)\bI\| &\le
    \|\sum_{j\neq i}\bW_{ij}\bO_j\|
    + m\|\bO_i^T\bTheta_i - \bI_r\|
    + \|\bTheta^T\bO - m\bI_r\|
    \quad
    \text{(under MAXDIFF model)}
    .
    \end{align*}
\end{lemma}

Results parallel to \Cref{lemma:pertubation} are also obtained: %as follows.
\iffalse
\begin{proposition}\label{prop:upperbound1}
	Let $(\bO_1, \dotsc, \bO_m)\in\times_{i=1}^m\mathcal{O}_{d,r}$ be a second-order critical point of problem \eqref{eqn:tracemax}
	satisfying Assumption \ref{assumption}. 
	If we build a block matrix $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$, then
	we have
	$$
	\|\bO - \bTheta\| \le
	\|\bO - \bTheta\|_F \le
	\sqrt{\frac{r}{m}}(2\|\bW\| + \sqrt{4\|\bW\|^2 + 2m})
	.
	$$
	%where $\|\cdot\|_F$ is the Frobenius norm.
\end{proposition}

\begin{proposition}\label{prop:upperbound2}
	For any block matrix $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$, then such that $\bO_i\in\mathcal{O}_{d_i,r}$,
	we have
	$$
	\|(\bW\bO)_i\| 
	\le
	\|(\bW\bO)_i\|_F
	\le
	\|\bW\|\|\bO-\bTheta\|_F
	+ \|(\bW\bTheta)_i\|_F
	.
	$$
	%where $\|\cdot\|_F$ is the Frobenius norm.
\end{proposition}

\begin{proposition}\label{prop:upperbound3}
	Let $(\bO_1, \dotsc, \bO_m)\in\times_{i=1}^m\mathcal{O}_{d_i,r}$ be a second-order critical point of problem \eqref{eqn:tracemax}
	satisfying Assumption \ref{assumption},  
	and $\bO$ be a block matrix $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$.
	If 
	$$
		m > \sqrt{r}(2\|\bW\| + \sqrt{4\|\bW\| + 2m}),
	$$
	then
	$$
	\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|
	\le
	\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|_F
	\le
	\frac{2(\max_{i=1,\dotsc,m}\|(\bW\bO)_i\|_F + \sqrt{r})}{m - \sqrt{r}(2\|\bW\| + \sqrt{4\|\bW\| + 2m})}
	.
	$$
\end{proposition}
\fi 
\begin{lemma}\label{lem:upperboundlocal}
    Let $(\bO_1, \dotsc, \bO_m)\in\times_{i=1}^m\mathcal{O}_{d,r}$ be a
    %second-order
    {candidate}
    critical point of problem \eqref{eqn:tracemax},
    {i.e., a point}
	satisfying Assumption \ref{assumption}. 
	If we build a block matrix $\bO=[\bO_1^T, \dotsc, \bO_m^T]^T$, then the following error estimates hold.
	\begin{align}
	    \|\bO - \bTheta\|_F &\le
	    \begin{cases}
	        4\|\bW\|\frac{\sqrt{r}}{\sqrt{m}},
	        & \text{under MAXBET model}, 
	        \\
	        4\|\bW\|\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}},
	        & \text{under MAXDIFF model},
	    \end{cases}
	    \label{eqn:localupperbound1}
	    \\
	    \|\bTheta^T\bO - m\bI_r\| &\le
	    \begin{cases}
	        4\|\bW\|\sqrt{r},
	        & \text{under MAXBET model}, 
	        \\
	        4\|\bW\|\frac{\sqrt{r}}{1-2/m},
	        & \text{under MAXDIFF model},
	    \end{cases}
	    \label{eqn:localupperbound1_1}
	    \\	    
	    \max_{1\le i\le m}\|[\bW\bO]_i]\|_F &\le
	    \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F 
	    +
	    \begin{cases}
	        4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}}, 
	        & \text{under MAXBET model}, 
	        \\
	        4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}},
	        & \text{under MAXDIFF model},
	    \end{cases}
	    \label{eqn:localupperbound2}
	    \\
	    \max_{1\le i\le m}\|\bO_i - \bTheta_i\|_F &\le
	    \begin{cases}
	        \frac{2\left(\max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}}\right)}{m - 4\|\bW\|\sqrt{r}},
	        & \text{under MAXBET model},
	        \\
	        \frac{2\left(\max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}}\right)}{m - 4\|\bW\|\frac{\sqrt{r}}{1-2/m}-3},
	        & \text{under MAXDIFF model}
	   \end{cases}
	   \label{eqn:localupperbound3}
	\end{align}
	where
	\begin{align*}
	    m > 
	    \begin{cases}
	        4\|\bW\|\sqrt{r},
	        & \text{under MAXBET model},
	        \\
	        \frac{5+4\|\bW\|\sqrt{r} + \sqrt{16\|\bW\|^2 r + 40 \|\bW\|\sqrt{r} + 1}}{2},
	        & \text{under MAXDIFF model.}
	    \end{cases}
	\end{align*}
\end{lemma}

We now assume %$d_1=\dotsb=d_m=d$ and 
the data model \eqref{eq:model}.
%\begin{equation}\label{eqn:model}
%	\bS_{ij} = \bTheta_i\bTheta_j^T + \bW_{ij},
%	\quad \bTheta_i, \bTheta_j \in \mathcal{O}_{d_i,r}, ~ \bW_{ji} = \bW_{ij}^T.
%\end{equation}
%for $j \neq i$. 
%Recall $\bS_{ii}=\bzero$.
We want a condition on the noise matrices $\bW_{ij}$ that guarantees the certificate \eqref{eqn:certificate} to hold.
Since $\bL\bO=\bzero$ if $\bO=(\bO_1,\dotsc,\bO_m)$ is a first-order critical point, it suffices to find a condition that
$$
	\bx^T\bL\bx \ge 0 \quad \text{for all $\bx=(\bx_1,\dotsc,\bx_m), \bx_i \in \mathbb{R}^{d}$ such that $\bO^T\bx =\bzero$}.
$$
Then for $\bO$ being a %second-order 
\textcolor{red}{candidate}
critical point and $\bx$ satisfying $\bO^T\bx=\bzero$,
\begin{align*}
	\bx^T\bL\bx &=
	\sum_{i=1}^m\left(
		\bx_i^T\bO_i\bLambda_i\bO_i^T\bx_i + \tau_i\bx_i^T\bO_i^{\perp}\bO_i^{\perp T}\bx
	\right)
	- \bx^T\bS\bx
	\\
	&\ge
	\sum_{i=1}^m\left(
		\tau_i\bx_i^T\bO_i\bO_i^T\bx_i + \tau_i\bx_i^T\bO_i^{\perp}\bO_i^{\perp T}\bx_i
	\right)
	- \bx^T\bS\bx
	\\
	&=
	\sum_{i=1}^m\tau_i\|\bx_i\|^2 - \bx^T\bS\bx
	.
\end{align*}

The block matrix \eqref{eqn:blockS} can be written 
\begin{equation}\label{eqn:Sexpansion}
	\bS = \bTheta\bTheta^T 
	%- \diag(\bTheta_i\bTheta_i^T) 
	+ \bW,
\end{equation}
where %$\bTheta=(\bTheta_1^T, \dotsc, \bTheta_m^T)^T$ and 
$\bW$ is a block matrix constructed from $\bW_{ij}$ in a similar fashion to \eqref{eqn:blockS}.
Then
\begin{align}\label{eqn:quadraticform}
	\bx^T\bS\bx &= \bx^T\bTheta\bTheta^T\bx %- \sum_{i=1}^m\bx_i^T\bTheta_i\bTheta_i^T\bx_i 
	+ \bx^T\bW\bx
	\nonumber\\
	&=
	\bx^T(\bTheta-\bO)(\bTheta-\bO)^T\bx 
	%- \sum_{i=1}^m\bx_i^T\bTheta_i\bTheta_i^T\bx_i 
	+ \bx^T\bW\bx
	\nonumber\\
	&= \|(\bTheta-\bO)^T\bx\|^2 
	%- \sum_{i=1}^m\bx_i^T\bTheta_i\bTheta_i^T\bx_i 
	+ \bx^T\bW\bx
	\nonumber\\
	&\le
	\|\bTheta-\bO\|^2\|\bx\|^2 
	%- \sum_{i=1}^m\|\bTheta_i\bTheta_i^T\bx_i\|^2 
	+ \|\bW\|\|\bx\|^2
	.
\end{align}
%for the induced matrix 2-norm $\|\bM\| = \sup_{\|\bx\|\le 1}\|\bM\bx\|$.
The second equality is due to
$\bO^T\bx=\bzero$.
% $$
% 	\bTheta^T\bx = (\bTheta-\bO)^T\bx
% $$
% since 
%$\bO^T\bx=\bzero$.

Hence we have
\begin{equation}\label{eqn:lowerbound1}
	\bx^T\bL\bx \ge
	\sum_{i=1}^m\tau_i\|\bx_i\|^2 - \|\bTheta-\bO\|^2\|\bx\|^2 - \|\bW\|\|\bx\|^2
	.
\end{equation}
% Combining Weyl's inequality
% $$
% 	|\tau_i - (m-1) | = |\lambda_{\min}(\bLambda_i) - \lambda_{\min}((m-1)\bI)|
% 	\le
% 	\|\bLambda_i - (m-1)\bI\|
% $$
% with Lemma \ref{lemma:noisy}:
% $$
% 	\|\bLambda_i - (m-1)\bI\| 
% 	\le
% 	\|(\bW\bO)_i\| + m\|\bO_i^T\bTheta_i - \bI\| + \|\bTheta^T\bO - m\bI\|
% 	,
% $$
Combining Weyl's inequality and \Cref{lem:weyllocal},
we obtain a lower bound on $\tau_i$:
$$
	\tau_i \ge 
	m
	%m - 1 
	- \|[\bW\bO]_i\| - m\|\bO_i^T\bTheta_i-\bI\| - \|\bTheta^T\bO - m\bI\|
	.
$$
Substituting this with inequality \eqref{eqn:lowerbound2}, we see
\begin{align}\label{eqn:lowerbound2}
	\bx^T\bL\bx &\ge
	(%m-1 
	m - \|\bTheta^T\bO - m\bI\|)\|\bx\|^2
	%\nonumber\\
	%& \quad 
	- \sum_{i=1}^m\left(
		\|[\bW\bO]_i\|\|\bx_i\|^2 + m\|\bO_i^T\bTheta_i-\bI\|\|\bx_i\|^2
	\right)
	\nonumber\\
	& \quad\quad - \|\bTheta - \bO\|^2\|\bx\|^2 
	- \|\bW\|\|\bx\|^2
	\nonumber
	\\
	&\ge
	\left(
	%m - 1 
	m - \|\bTheta^T\bO - m\bI\| - \max_{i=1,\dotsc,m}\|[\bW\bO]_i\| 
	\right.
	\nonumber\\
	& \quad\quad
	\left.
	- m\max_{i=1,\dotsc,m}\|\bO_i^T\bTheta_i - \bI\| - \|\bTheta - \bO\|^2 - \|\bW\|
	\right)
	\|\bx\|^2
	.
\end{align}
Thus if
\begin{equation}\label{eqn:lowerbound3}
	%\begin{split}
	m %& >
	\ge
	\|\bTheta^T\bO - m\bI\| + \max_{i=1,\dotsc,m}\|[\bW\bO]_i\| 
	%\\
	%&\quad
	+ m\max_{i=1,\dotsc,m}\|\bO_i^T\bTheta_i - \bI\| 
	+ \|\bTheta - \bO\|^2 
	+ \|\bW\|
	,
	%\end{split}
\end{equation}
then we have $\bL \psdge \bzero$.

Also, since post-multiplying a fully orthogonal matrix in $\mathcal{O}_{r,r}$ to $\bO_1, \dotsc, \bO_m$ does not change the objective of \eqref{eqn:tracemax}, 
% we can assume without loss of generality
% \begin{equation}\label{eqn:wlog}
% 	\bTheta^T\bO \text{ is symmetric, positive semidefinite}.
% \end{equation}
we may choose $\bO$ such that $\bTheta^T\bO$ is symmetric, positive semidefinite.

% Since $\bTheta^T\bTheta=m\bI_r$, we see $\|\bTheta^T\bO-m\bI_r\| \le \sqrt{m}\|\bTheta-\bO\|$. 
% Thus both the first and fourth terms of the right-hand side of \eqref{eqn:lowerbound3} can be upper bounded provided that an upper bound of $\|\bO-\bTheta\|$. The latter is obtained by Proposition \ref{prop:upperbound1}.
% %Upper bounds of the first and fourth terms of the right-hand side of \eqref{eqn:lowerbound3} can be found:
% %\begin{proposition}\label{prop:upperbound1}
% %	Under Assumption \ref{assumption}, we have
% %	$$
% %	\|\bO - \bTheta\| \le
% %	\|\bO - \bTheta\|_F \le
% %	\sqrt{\frac{r}{m}}(2\|\bW\| + \sqrt{4\|\bW\|^2 + 2mr})
% %	.
% %	$$
% %	where $\|\cdot\|_F$ is the Frobenius norm.
% %\end{proposition}

% An upper bound of the second term of the right-hand side of \eqref{eqn:lowerbound3} can be found by combining Proposition \ref{prop:upperbound2} and \ref{prop:upperbound1}, since $\max_{i=1,\dotsc,m}\|(\bW\bO)_i\| \le \max_{i=1,\dotsc,m}\|(\bW\bO)_i\|_F$.  %and the following:
% %\begin{proposition}\label{prop:upperbound2}
% %	Under Assumption \ref{assumption}, we have
% %	$$
% %	\|(\bW\bO)_i\| 
% %	\le
% %	\|(\bW\bO)_i\|_F
% %	\le
% %	\|\bW\|\|\bO-\bTheta\|_F
% %	+ \|(\bW\bTheta)_i\|_F
% %	.
% %	$$
% %	%where $\|\cdot\|_F$ is the Frobenius norm.
% %\end{proposition}

% Finally, an upper bound of the third term of the right-hand side of \eqref{eqn:lowerbound3} follows from combining Propositions \ref{prop:upperbound3}, \ref{prop:upperbound2}, and \ref{prop:upperbound1}, because $\max_{i=1,\dotsc,m}\|\bO_i\bTheta_i-\bI\| \le \max_{i=1,\dotsc,m}\|\bTheta_i\|\|\bO_i-\bTheta_i\| = \max_{i=1,\dotsc,m}\|\bO_i-\bTheta_i\|$. %and the following result:
% %\begin{proposition}\label{prop:upperbound3}
% %	Suppose Assumption \ref{assumption} holds.
% %	If 
% %	$$
% %		m > \sqrt{r}(2\|\bW\| + \sqrt{4\|\bW\| + 2mr}),
% %	$$
% %	then
% %	$$
% %	\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|
% %	\le
% %	\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|_F
% %	\le
% %	\frac{2(\max_{i=1,\dotsc,m}\|(\bW\bO)_i\|_F + \sqrt{r})}{m - \sqrt{r}(2\|\bW\| + \sqrt{4\|\bW\| + 2mr})}
% %	.
% %	$$
% %\end{proposition}

Thus we apply \Cref{lem:upperboundlocal}  to the right-hand side of inequality \eqref{eqn:lowerbound3} to get:
\begin{align*}
	&\|\bTheta^T\bO - m\bI\| + \max_{i=1,\dotsc,m}\|(\bW\bO)_i\| 
	\quad
	+ m\max_{i=1,\dotsc,m}\|\bO_i^T\bTheta_i - \bI\| 
	+ \|\bTheta - \bO\|^2 
	+ \|\bW\|
	\\
	&\le
    4\|\bW\|\sqrt{r}
    + \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\sqrt{\frac{r}{m}}
    + \frac{2m(\max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\sqrt{\frac{r}{m}})}{m - 4\|\bW\|\sqrt{r}}
    \\
    &\quad
    + 16\|\bW\|^2\frac{r}{m}
    + \|\bW\|
	.
\end{align*}
%This final upper bound is independent of $\bO$. 
If this bound is less than or equal to $m$, then condition \eqref{eqn:lowerbound3} is satisfied. Thus we have proved Theorem \ref{thm:main2}.

\subsection{Proof of \Cref{cor:discordant}}\label{sec:proof_discordant}
Under the $\bTheta$-concordance of $\frac{1}{\sigma}\bW$,
the right-hand side of inequality  \eqref{eqn:noiselevel} in \Cref{thm:main2} is upper bounded by
\begin{equation}\label{eqn:concordanceupperbound1}
12\sigma\sqrt{Dr} 
+ 3\sigma\sqrt{Dr\log m}
+ 36\sigma^2 D \sqrt{\frac{r}{m}}
+ \frac{2m(3\sigma\sqrt{Dr\log m} + 36\sigma^2 D \sqrt{\frac{r}{m}})}{m - 12\sigma\sqrt{Dr}}
+ 144\sigma^2\frac{Dr}{m}
+ 3\sigma\sqrt{D}
\end{equation}
if $\sigma < \frac{m}{12\sqrt{Dr}}$.
If \eqref{eqn:concordanceupperbound1} is less than or equal to $m$, or equivalently
\begin{equation}\label{eqn:concordanceupperbound2}
    1 \geq
    12\sigma\sqrt{\frac{dr}{m}}
    + 3\sigma\sqrt{\frac{dr\log m}{m}}
    + 36\sigma^2 d\sqrt{\frac{r}{m}}
    + \frac{2(3\sigma\sqrt{drm\log m} + 36\sigma^2 d\sqrt{rm})}{m - 12\sigma\sqrt{drm}}
    + 144\sigma^2\frac{dr}{m}
    + 3\sigma\sqrt{\frac{d}{m}}
\end{equation}
for 
\[
    \sigma < \frac{m^{1/2}}{12\sqrt{dr}}
    ,
\]
then from the proof of \Cref{thm:main2}, we see that condition \eqref{eqn:lowerbound3} is satisfied and thus the claim is proved.

The fourth term in the right-hand side of inequality \eqref{eqn:concordanceupperbound2} is 
\begin{align*}
    \frac{2(3\sigma\sqrt{drm\log m} + 36\sigma^2 d\sqrt{rm})}{m - 12\sigma\sqrt{drm}}
    &=
    \frac{2\left(3\sigma\sqrt{\frac{dr\log m}{m}} + 36\sigma^2 d\sqrt{\frac{r}{m}}\right)}{1 - 12\sigma\sqrt{\frac{dr}{m}}}
    \\
    &\leq
    %\frac{20}{7}
    %2.625\left(3\sigma\frac{\sqrt{dr\log m}}{m^{1/2}} + 36\sigma^2 \frac{d\sqrt{r}}{m^{1/2}}\right)
    \frac{2}{1 - \frac{12}{31}\frac{1}{m^{1/4}}}
    \left(3\sigma\sqrt{\frac{dr\log m}{m}} + 36\sigma^2 d\sqrt{\frac{r}{m}}\right)
\end{align*}
if $\sigma \le \frac{m^{1/4}}{31\sqrt{dr}}$.
%, since $m \ge 2$ and
% \[
% 1 - 12 \sigma\frac{\sqrt{dr}}{m}
% \ge 1 - \frac{12}{30}\frac{m^{1/4}}{\sqrt{dr}}\frac{\sqrt{dr}}{m}
% = 
% 1 - \frac{12}{30}\frac{1}{m^{3/4}}
% \geq
% 1 - \frac{12}{30}\frac{1}{2^{3/4}}
% \ge %\frac{7}{10}
% 0.763
% .
% \]
Thus,
\begin{align*}
    \text{(RHS of \eqref{eqn:concordanceupperbound2})}
    & \leq
    \frac{12}{31}\frac{m^{1/4}}{\sqrt{dr}}\frac{\sqrt{dr}}{m^{1/2}}
    + 
    \left(1 + \frac{2}{1 - \frac{12}{31}\frac{1}{m^{1/4}}}\right)
    \left(\frac{3}{31}\frac{m^{1/4}}{\sqrt{dr}}\frac{\sqrt{dr\log m}}{m^{1/2}}
    + \frac{36}{961}\frac{m^{1/2}}{dr}\frac{d\sqrt{r}}{m^{1/2}}
    \right)
    \\
    &\quad
    % + %\frac{20}{7}
    % 2.625\left(
    %     \frac{3}{30}\frac{m^{1/4}}{\sqrt{dr}}\frac{\sqrt{dr\log m}}{m^{1/2}} 
    %     + \frac{36}{900}\frac{m^{1/2}}{dr}\frac{d\sqrt{r}}{m^{1/2}}
    %     \right)
    + \frac{144}{961}\frac{m^{1/2}}{dr}\frac{dr}{m}
    + \frac{3}{31}\frac{m^{1/4}}{\sqrt{dr}}\frac{\sqrt{d}}{m^{1/2}}
    \\
    & =
    \frac{12}{31}\frac{1}{m^{1/4}}
    + 
    \left(1 +
    \frac{2}{1 - \frac{12}{31}\frac{1}{m^{1/4}}}\right)
    \left(
    \frac{3}{31}\frac{\sqrt{\log m}}{m^{1/4}}
    + \frac{36}{961}\frac{1}{\sqrt{r}}
    \right)
    % + %\frac{20}{7}
    % 2.625\frac{3}{30}\frac{\sqrt{\log m}}{m^{1/4}} 
    % + %\frac{20}{7}
    % 2.625\frac{36}{900}\frac{1}{\sqrt{r}}
    + \frac{144}{961}\frac{1}{m^{1/2}}
    + \frac{3}{31}\frac{1}{\sqrt{r}m^{1/4}}
    \\
    & \leq
    \frac{12}{31}\frac{1}{2^{1/4}}
    + 
    \left(1 + \frac{2}{1 - \frac{12}{31}\frac{1}{2^{1/4}}}\right)
    \left(
    \frac{3}{31}\sqrt{\frac{2}{e}}
    + \frac{36}{961}
    \right)
    % + 2.625\frac{3}{30}\sqrt{\frac{2}{e}}
    % + 2.625\frac{36}{900}%\frac{1}{2}
    + \frac{144}{961}\frac{1}{2^{1/2}}
    + \frac{3}{31}\frac{1}{2^{1/4}}
    \approx 0.9905
    < 1
\end{align*}
as desired,
since $r \ge 1$ and $\frac{\sqrt{\log m}}{m^{1/4}} \le \sqrt{\frac{2}{e}}$. %, and $\frac{\sqrt{\log m}}{m^{5/4}} \le \sqrt{\frac{2}{5e}}$.



\subsection{\Cref{thm:main2}, \Cref{cor:discordant}, and \Cref{cor:gaussian} under the MAXDIFF setting}\label{sec:proof:maxdiff}
Under the MAXDIFF model, inequality \eqref{eqn:quadraticform} is replaced by
\begin{align*}
	\bx^T\bS\bx 
	&\leq
	\|\bTheta-\bO\|^2\|\bx\|^2 
	- \sum_{i=1}^m\|\bTheta_i\bTheta_i^T\bx_i\|^2 
	+ \|\bW\|\|\bx\|^2
	\\
	&\leq
	\left(\|\bTheta-\bO\|^2
	- \min_{1\le i \le m}\|\bTheta_i\|^2
	+ \|\bW\|\right)
	\|\bx\|^2	
	,
\end{align*}
and \eqref{eqn:lowerbound2} by
\begin{align*}
	\bx^T\bL\bx &\ge
	\left(
	m - 1 
	- \|\bTheta^T\bO - m\bI\| - \max_{i=1,\dotsc,m}\|[\bW\bO]_i\| 
	\right.
	\nonumber\\
	& \quad\quad
	\left.
	- m\max_{i=1,\dotsc,m}\|\bO_i^T\bTheta_i - \bI\| - \|\bTheta - \bO\|^2 - \|\bW\|
	+ \min_{1\le i \le m}\|\bTheta_i\|^2
	\right)
	\|\bx\|^2
	\\
	&=
	\left(
	m 
	- \|\bTheta^T\bO - m\bI\| - \max_{i=1,\dotsc,m}\|[\bW\bO]_i\| 
	\right.
	\nonumber\\
	& \quad\quad
	\left.
	- m\max_{i=1,\dotsc,m}\|\bO_i^T\bTheta_i - \bI\| - \|\bTheta - \bO\|^2 - \|\bW\|
	\right)
	\|\bx\|^2
	.
\end{align*}
since $\|\bTheta_i\|=1$ for all $i$.
Thus condition \eqref{eqn:lowerbound3} for $\bL \psdge \bzero$ to hold remains unchanged.
Applying \Cref{lem:upperboundlocal}, we obtain
\begin{align*}
    m
	&\ge
    4\|\bW\|\frac{\sqrt{r}}{1-2/m}
    + \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}}
    \\
    & \quad
    + \frac{2m(\max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}})}{m - 4\|\bW\|\frac{\sqrt{r}}{1-2/m}-3}
    + 16\|\bW\|^2\frac{r}{(\sqrt{m}-2/\sqrt{m})^2}
    + \|\bW\|
	.
\end{align*}
Proceeding as above for MAXBET, we obtain the bound on $\sigma$ as stated in \Cref{rem:maxdifflocal}.

Furthermore, inequality \eqref{eqn:concentrationlocal} is replaced by
\[
	\Pr{\left(\max_{i=1,\dotsc,m}\|[\bW\bTheta]_i\|_F \le \sigma(\sqrt{\underline{d}r(m-1)} + r\sqrt{m-1} + 2\sqrt{r\log m})\right)} > 1 - \frac{1}{m}
	,
\]
(recall that $\underline{d}=\min_{m=1,\dotsc,m}d_i$)
and inequality \eqref{eqn:concentration_concordance} holds for $m \ge 2$ for all $\underline{d}$, since $m - 1 \le m\log m$ for all $m \ge 2$.
Thus the conclusion of \Cref{cor:gaussian} holds without modification, provided that $m \ge 4$ and $\sigma \le \frac{m^{1/4}}{64\sqrt{dr}}$ as stated in \Cref{rem:maxdifflocal}.


{%
\subsection{Proof of \Cref{prop:consistencylocal}}
The desired results follow immediately from inequality \eqref{eqn:localupperbound3} of \Cref{lem:upperboundlocal} and \Cref{def:discordance}.%
}

==> sections/06-proofothers.tex <==
\section{Proofs of Technical Lemmas and Propositions}\label{sec:proof_lemma}

\subsection{Proof of Proposition \ref{prop:noiseless}}\label{sec:proof_prop:noiseless}
\begin{proof}[Proof of Proposition \ref{prop:noiseless}]
    First consider model \eqref{eq:model}. 
	We have $\bS_{ij}=\bTheta_i\bTheta_j^T$ for all $i, j$. Then the objective of \eqref{eqn:tracemax} is
	$$
		\sum_{i,j}\tr(\bO_i^T\bTheta_i\bTheta_j^T\bO_j)
		= \sum_{i,j}\tr[(\bTheta_i^T\bO_i)^T(\bTheta_j^T\bO_j)]
		.
	$$
	Each term is bounded by the von Neumann-Fan inequality \citep[Example 2.8.7]{lange2016mm}
	\begin{equation}\label{eqn:vonneumann}
		\tr[(\bTheta_i^T\bO_i)^T(\bTheta_j^T\bO_j)]
		\le
		\sum_{k=1}^r\sigma_k(\bTheta_i^T\bO_i)\sigma_k(\bTheta_j^T\bO_j)
		,
	\end{equation}
	where $\sigma_k(\bM)$ is the $k$th largest singular value of matrix $\bM$.
	Since $\bO_i^T\bTheta_i\bTheta_i\bO_i \psdle \bO_i^T\bO_i = \bI_r$, we see $\max_{k=1,\cdots,r}\sigma_k(\bTheta_i^T\bO_i) \le 1$ for all $\bO_i \in \mathcal{O}_{d_i,r}$, $i=1,\dotsc,m$.
	Thus the largest possible value of the right-hand side of inequality \eqref{eqn:vonneumann} is $r$ and \eqref{eqn:tracemax} has maximum $m^2r$.
	%$m(m-1)r$. 
	This is achieved by $\bO_i=\bTheta_i$ for $i=1,\dotsc,m$ since $\bTheta_i^T\bTheta_i=\bI_r$.
	
	It is straightforward to modify the above proof for model \eqref{eq:model2}. The maximum is $m(m-1)r$.
\end{proof}

\subsection{Proofs of Lemmas for Theorem \ref{thm:main}}\label{sec:proof_lemma:local}

%\begin{proof}[Proof of Lemma~\ref{lemma:equivalent}]
%Since $\bU$ is symmetric and has rank $r$, there exists a decomposition such that $\bU=\bO\bO^T$, where $\bO\in\reals^{D\times r}$. Then the condition $\bU_{ii}\psdle\bI$ implies that all singular values of $\bO_i$ are not greater than $1$, $\tr(\bU_{ii})=r$ implies that $\|\bO_i\|_F=\sqrt{r}$. Recall that $\bO_i\in\reals^{m_i\times r}$ has at most $r$ singular values, we have that all singular values of $\bO_i$ are $1$ and $\bO_i^T\bO_i=\bI$. 
%
%On the other hand, for any $\bO$ in the constraint set of \eqref{eqn:tracemax}, $\bU=\bO\bO^T$ lies in the constraint set of \eqref{eq:tracesum_problem1}. 
%
%In addition, with $\bU=\bO\bO^T$ and $\bS_{ii}=\mathbf{0}$, we have $\tr(\bS\bU)=\sum_{i,j=1, i\neq j}^m\tr(\bO_i^T\bS_{ij}\bO_j)$. As a result,  \eqref{eqn:tracemax} and  \eqref{eq:tracesum_problem1} are equivalent. 
%\end{proof}
	
\begin{proof}[Proof of Lemma~\ref{lemma:stationary}]
% First recall that 
% the OTSM problem \eqref{eqn:tracemax} is equivalent to the problem 
% \begin{equation}\label{eq:tracesum_problem1}
% \tilde{\bU}= {\arg}\max_{\bU\in\reals^{D\times D}, \bU=\bU^T}\tr(\bS\bU), \text{subject to $\bU\psdge \mathbf{0}, \bU_{ii}\psdle\bI, \tr(\bU_{ii})=r, \rank(\bU)=r$.}
% \end{equation}


Let us consider the tangent space of the constraint set in \eqref{eq:tracesum_problem1} at $\bU=\tilde{\bU}$. In particular, the condition $\bU\psdge \mathbf{0}$ and $\rank(\bU)=r$ give a tangent cone of $\{\bX: P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}=\mathbf{0}\}.$
The condition $\bU_{ii}\psdle \bI$ and $\tr(\bU_{ii})=r$ give the tangent cone of $
\{\bX: P_{\bTheta_i}^T\bX_{ii}P_{\bTheta_i}\psdle \mathbf{0}, \tr(\bX_{ii})=0,\,\,\text{for all $1\leq i\leq m$}\}.$

In combination, the tangent cone of \eqref{eq:tracesum_problem1} at $\bU=\tilde{\bU}$ is
\begin{equation}\label{eq:tangent}
\calT_1=\{\bX\in\reals^{D\times D}: P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}=\mathbf{0}, \text{and for all $1\leq i\leq m$,}\,\, P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}\psdle \mathbf{0}, \tr(\bX_{ii})=0\}.
\end{equation}
Next, we will prove that the set in \eqref{eq:tangent} can be simplified to
\begin{equation}\label{eq:tangent1}
\calT_2=\{\bX\in\reals^{D\times D}: P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}=\mathbf{0}, \text{and for all $1\leq i\leq m$,}\,\, P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}= \mathbf{0}\}.
\end{equation}
Clearly, $\calT_2\subseteq\calT_1$. Next, we will prove $\calT_1\subseteq\calT_2$ by showing that all $\bX\in \calT_1$ satisfies $P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}= \mathbf{0}$.

For any $\bX\in \calT_1$, since $P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}=\mathbf{0}$, there exists $\bY\in\reals^{D\times r}$ such that $\bX=\tilde{\bV}\bY^T+\bY\tilde{\bV}^T$, and we have $\bX_{ii}=\tilde{\bV}_i\bY_i^T+\bY_i\tilde{\bV}_i^T$. This implies that \[
P_{\tilde{\bV}_i^\perp}^T\bX_{ii}P_{\tilde{\bV}_i^\perp}=\mathbf{0},
\]
and then
\[
0=\tr(\bX_{ii})=\tr(P_{\tilde{\bV}_i^\perp}^T\bX_{ii}P_{\tilde{\bV}_i^\perp})+\tr(P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i})=\tr(P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}).
\]
Combining it with the assumption that $P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}\psdge \mathbf{0}$, we have $\tr(P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i})= \mathbf{0}$. This implies that $\bX\in \calT_2$. As a result, $\calT_1=\calT_2$.

Since $\tilde{\bU}$ is the optimal solution for the problem \eqref{eq:tracesum_problem1}, we have $0=\tr(\bX\bS)=\langle\bX, \bS\rangle$ for all $\bX\in\calT_2$. Notice that $\calT_2$ is a subspace in $\reals^{D\times D}$, this implies that $\bS$ lies in the orthogonal complement of $\calT_2$,
which is
\begin{equation}\label{eq:tangent3}
\{\bX: \Proj_{\tilde{\bV}^\perp}\bX \Proj_{\tilde{\bV}^\perp}=\bX\}\oplus\{\bX:\bX_{ij}=\mathbf{0} \,\,\text{if $i\neq j$, and $\Proj_{\tilde{\bV}_i}\bX_{ii} \Proj_{\tilde{\bV}_i}=\bX_{ii}$.}\}
\end{equation}
This proves the decomposition of $\bS=\bT^{(1)}+\bT^{(2)}$, such that 
\[
\text{$\Proj_{\tilde{\bV}^\perp}\bT^{(1)} \Proj_{\tilde{\bV}^\perp}=\bT^{(1)}$, $\bT^{(2)}_{ij}=\mathbf{0}$ for $i\neq j$, and $\Proj_{\tilde{\bV}_i}\bT^{(2)}_{ii} \Proj_{\tilde{\bV}_i}=\bT^{(2)}_{ii}$.}
\]
%The formula in \eqref{eq:tildeT1} and \eqref{eq:tildeT2} follow from the properties of $\bT^{(1)}, \bT^{(2)}$ and in particular, the last equation in \eqref{eq:tildeT2} follows from the fact that $\bT^{(1)}\tilde{\bV}=\mathbf{0}$.
{%
The formula in \eqref{eq:tildeT1} and \eqref{eq:tildeT2} follow from the properties of $\bT^{(1)}$ and $\bT^{(2)}$. 
In particular, 
$\Proj_{\tilde{\bV}^\perp}\bT^{(1)} \Proj_{\tilde{\bV}^\perp}=\bT^{(1)}$
implies that $\bT^{(1)}\tilde{\bV}=\mathbf{0}$,
which in turn implies $\bS\tilde{\bV} = \bT^{(2)}\tilde{\bV}$ or equivalently
\[
    \sum_{j=1}^m\bS_{ij}\tilde{\bV}_j 
    = \bT^{(2)}_{ii}\tilde{\bV}_i
    .
\]
Then $\Proj_{\tilde{\bV}_i}\bT^{(2)}_{ii} \Proj_{\tilde{\bV}_i}=\bT^{(2)}_{ii}$ implies that
$\bT^{(2)}_{ii} = \tilde{\bV}_i\bLambda_i\tilde{\bV}_i^T$
for some symmetric matrix $\bLambda_i\in\mathbb{R}^{r\times r}$. Thus,
\[
    \sum_{j=1}^m\bS_{ij}\tilde{\bV}_j 
    = \bT^{(2)}_{ii}\tilde{\bV}_i
    = \tilde{\bV}_i\bLambda_i
    ,
\]
which yields
\[
    \sum_{j=1}^m\bS_{ij}\tilde{\bV}_j\tilde{\bV}_i^T = \tilde{\bV}_i\bLambda_i\tilde{\bV}_i^T 
    = \bT^{(2)}_{ii}
    ,
\]
that is, equation \eqref{eq:tildeT2}.
}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:equavalency}]
For any $\bU$ in the constraint set of  \eqref{eq:tracesum_relaxed} such that $\bU\neq \tilde{\bU}$, and $\bX=\bU-\tilde{\bU}$, we have $P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}=P_{\tilde{\bV}^\perp}^T\bU P_{\tilde{\bV}^\perp}-P_{\tilde{\bV}^\perp}^T\tilde{\bU} P_{\tilde{\bV}^\perp}= P_{\tilde{\bV}^\perp}^T\bU P_{\tilde{\bV}^\perp}\psdge \mathbf{0}$, and $P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}=P_{\tilde{\bV}_i}^T\bU_{ii}P_{\tilde{\bV}_i}-P_{\tilde{\bV}_i}^T\tilde{\bU}_{ii}P_{\tilde{\bV}_i}=P_{\tilde{\bV}_i}^T\bU_{ii}P_{\tilde{\bV}_i}-\bI\psdle \mathbf{0}$. In summary, $\bX$ has the properties of
\begin{equation}\label{eq:tangent4}
P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}\psdge \mathbf{0}, \text{$\tr(\bX_{ii})=0$ and  $P_{\tilde{\bV}_i}^T\bX_{ii}P_{\tilde{\bV}_i}\psdle \mathbf{0}$ for all $1\leq i\leq m$.} 
\end{equation}

In addition, either $P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}$ is nonzero or  $P_{\tilde{\bV}_i}^T\bX_{ii} P_{\tilde{\bV}_i}$ is nonzero {for some $i$}. If they are all zero matrices, then we have
\begin{equation}\label{eq:tangent5}
P_{\tilde{\bV}^\perp}^T\bU P_{\tilde{\bV}^\perp}=P_{\tilde{\bV}^\perp}^T\tilde{\bU} P_{\tilde{\bV}^\perp}=\mathbf{0},
\end{equation}
and
\begin{equation}\label{eq:tangent6}
P_{\tilde{\bV}_i}^T\bU_{ii} P_{\tilde{\bV}_i}=P_{\tilde{\bV}_i}^T\tilde{\bU}_{ii} P_{\tilde{\bV}_i}=\bI.
\end{equation}
Since  $\bU_{ii}\psdge 0$, we have {$\tilde{\bV}_i^T\bU_{ii}\tilde{\bV}_i\psdge \mathbf{0}$}. Combining it with $\tr(P_{\tilde{\bV}_i}^T\bU_{ii} P_{\tilde{\bV}_i})=r$ {(due to equation \eqref{eq:tangent6})} and $r=\tr(\bU_{ii})=\tr(P_{\tilde{\bV}_i}^T\bU_{ii} P_{\tilde{\bV}_i})+\tr(\tilde{\bV}_i\bU_{ii}\tilde{\bV}_i)$, we have {$\tilde{\bV}_i^T\bU_{ii}\tilde{\bV}_i= \mathbf{0}$}. Combining it with $\bU_{ii}\psdge \mathbf{0}$, we have {$\tilde{\bV}_i^T\bU_{ii}=\mathbf{0}$ and $\bU_{ii}^T\tilde{\bV}_i=\mathbf{0}$}. It implies that 
\begin{equation}\label{eq:tangent7}
\bU_{ii}=\Proj_{\tilde{\bV}_i}^T\bU_{ii} \Proj_{\tilde{\bV}_i}=\tilde{\bV}_i\tilde{\bV}_i^T.
\end{equation}
In addition, \eqref{eq:tangent5} and $\bU\psdge \mathbf{0}$ means that the $\bU=\Proj_{\tilde{\bV}}\bU \Proj_{\tilde{\bV}}$, that is, there exists a matrix $\bZ\in\mathbb{R}^{r\times r}$ such that $\bU=\tilde{\bV}\bZ\tilde{\bV}^T$ and as a result, $\bU_{ii}=\tilde{\bV}_i\bZ\tilde{\bV}_i^T$. Combining it with \eqref{eq:tangent7}, we have $\bZ=\bI$ and $\bU=\tilde{\bV}\tilde{\bV}^T=\tilde{\bU}$, which is a contradiction to {assumption} $\bU\neq \tilde{\bU}$.

Combining the property of $\bX$ in \eqref{eq:tangent4} with the assumption that $\{P_{\tilde{\bV}_i}^T\hat{\bT}^{(2)}_{ii} P_{\tilde{\bV}_i}\}_{i=1}^m$ and $-P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ are  positive definite matrices, we have
\begin{align}
&\tr(\bX\bS)=\tr(\bX\hat{\bT}^{(1)})+\tr(\bX\hat{\bT}^{(2)})+c\tr(\bX)= \tr\left((P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp})( P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp})\right)+\sum_{i=1}^m\tr(\bX_{ii} \hat{\bT}^{(2)}_{ii})\\= &\tr\left((P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp})( P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp})\right) + \sum_{i=1}^m\tr\left((P_{\tilde{\bV}_i}^T\bX_{ii} P_{\tilde{\bV}_i})(P_{\tilde{\bV}_i}^T\hat{\bT}^{(2)}_{ii} P_{\tilde{\bV}_i})\right)< 0.\label{eq:tangent8}
\end{align}
The last inequality is strict because either $P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}$ is nonzero or  $P_{\tilde{\bV}_i}^T\bX_{ii} P_{\tilde{\bV}_i}$ is nonzero for some $1\leq i\leq m$. {Then equation \eqref{eq:tangent}} implies that $\trace(\bS\bU)< \trace(\bS\tilde{\bU})$ for all $\bU\neq\tilde{\bU}$, and as a result, $\tilde{\bU}$ is the unique solution to  \eqref{eq:tracesum_relaxed}.


%for any $\bX$ . If  $P_{\tilde{\bV}^\perp}^T\bX P_{\tilde{\bV}^\perp}$ and $P_{\tilde{\bV}_i}^T\bX_{ii} P_{\tilde{\bV}_i}$ are zero for all $1\leq i\leq m$, then  $\bX$ is in the set \eqref{eq:tangent} and by the definition of \eqref{eq:tracesum_problem1}, we know that $\tr(\bX\bS)=0$. In summary, $\tr(\bX\bS)$ is not positive $\tilde{\bU}$ is also the minimizer of \eqref{eq:tracesum_relaxed}.
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma:clean}]
Since {$L_1\subset L_2$}, we have $\Proj_{L_2\cap L_1^\perp}=\Proj_{L_2}-\Proj_{L_1}$. Applying the definitions of $L_1$ and $L_2$, we have
\[
[\Proj_{L_1}]_{ij}=\frac{1}{m}\bTheta_i\bTheta_j^T
\]
and
\[
[\Proj_{L_2}]_{ii}=\bTheta_i\bTheta_i^T, \,\,[\Proj_{L_2}]_{ij}=\mathbf{0}\,\,\text{for $i\neq j$}.
\]
Combining it with the definition of $\bT^{(1)*}$ in \eqref{eq:tildeT1} and \eqref{eq:tildeT2}, 
and recalling Proposition \ref{prop:noiseless},
we have
\begin{equation}\label{eq:tildeTstar1}
[\bT^{(1)*}]_{ij}=\bTheta_i\bTheta_j^T\,\,\text{for $i\neq j$}, %\,\,P_{\tilde{\bV}_i^\perp}^T[\bT^{(1)*}]_{ii}=0,\,\,[\bT^{(1)*}]_{ii}=-(m-1){\bV}_i{\bV}_i^T=-[\bT^{(2)*}]_{ii},
{\bT^{(2)*}_{ij} = 0\,\,\text{for $i\neq j$},\,\,\bT^{(2)*}_{ii}=m\bTheta_i\bTheta_i^T}.
\end{equation} 
{Hence $\bT^{(1)*}_{ii}=\bS_{ii} - \bT^{(2)*}_{ii} = -(m-1)\bTheta_i\bTheta_i^T$}
and Lemma~\ref{lemma:clean} is proved.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:noisy}]
(i)
Applying \eqref{eq:tildeT1}, \eqref{eq:tildeT2}, and \eqref{eq:tildeTstar1}, we have
% \begin{equation}\text{$[{\bT}^{(1)}-{\bT}^{(1)*}]_{ij}=\bS_{ij}-\bTheta_i\bTheta_j^T=\bW_{ij}$ for $i\neq j$, $[\hat{\bT}^{(1)}-\hat{\bT}^{(1)*}]_{ii}
% =-(\sum_{j=1,j\neq i}^{m}\bS_{ij}\tilde{\bV}_j)\tilde{\bV}_i^T+(m-1)\bTheta_i\bTheta_i^T$.}\label{eq:tildeTstar2}\end{equation}
\begin{equation}\label{eq:tildeTstar2}
\begin{split}
[{\bT}^{(1)}-{\bT}^{(1)*}]_{ij} &= \bS_{ij}-\bTheta_i\bTheta_j^T=\bW_{ij} \text{~for~} i\neq j, \\ 
[{\bT^{(1)}-\bT^{(1)*}}]_{ii}
&= {\bW_{ii}}
-({\sum_{j=1}^{m}}\bS_{ij}\tilde{\bV}_j)\tilde{\bV}_i^T+{m}\bTheta_i\bTheta_i^T.
\end{split}
\end{equation}
As a result, 
% \begin{align}\label{eq:pertubation_1}
% \|\bT^{(1)}-\bT^{(1)*}\|\leq \|\bW\|+\max_{1\leq i\leq m}\left\|\left(\sum_{j=1,j\neq i}^{m}\bS_{ij}\tilde{\bV}_j\right)\tilde{\bV}_i^T-(m-1)\bTheta_i\bTheta_i^T\right\|.
% \end{align}
\begin{align}\label{eq:pertubation_1}
\|\bT^{(1)}-\bT^{(1)*}\|\leq \|\bW\|+\max_{1\leq i\leq m}\left\|\left({\sum_{j=1}^{m}}\bS_{ij}\tilde{\bV}_j\right)\tilde{\bV}_i^T-{m}\bTheta_i\bTheta_i^T\right\|.
\end{align}


% Applying 
% \begin{equation}\label{eq:j_exclude_i}
% \|(\sum_{j=1,j\neq i}^{m}\bTheta_j^T\tilde{\bV}_j)-(m-1)\bI\|\leq \|(\sum_{j=1}^{m}\bTheta_j^T\tilde{\bV}_j)-m\bI\|+\|\bTheta_i^T\tilde{\bV}_i-\bI\|\leq \|\bTheta^T\tilde{\bV}-m\bI\|+\|\bTheta_i-\tilde{\bV}_i\|,
% \end{equation}
{
Noting
\begin{equation}\label{eq:j_exclude_i}
\sum_{j=1}^{m}\bTheta_j^T\tilde{\bV}_j
= 
\bTheta^T\tilde{\bV}
,
\end{equation}
}
we have 
% \begin{align}\label{eq:j_exclude_i2}
% &\|(\sum_{j=1,j\neq i}^{m}\bTheta_i\bTheta_j^T\tilde{\bV}_j)\tilde{\bV}_i^T-(m-1)\bTheta_i\bTheta_i^T\|
% = \|(\sum_{j=1,j\neq i}^{m}\bTheta_j^T\tilde{\bV}_j)\tilde{\bV}_i^T-(m-1)\bTheta_i^T\|
% \\\leq &\|(\sum_{j=1,j\neq i}^{m}\bTheta_j^T\tilde{\bV}_j)-(m-1)\bI\|+(m-1)\|\tilde{\bV}_i-\bTheta_i\|\leq \|\bTheta^T\tilde{\bV}-m\bI\|+m\|\tilde{\bV}_i-\bTheta_i\|.\nonumber
% \end{align}
\begin{align}\label{eq:j_exclude_i2}
&\|({\sum_{j=1}^{m}}\bTheta_i\bTheta_j^T\tilde{\bV}_j)\tilde{\bV}_i^T-{m}\bTheta_i\bTheta_i^T\|
= \|({\sum_{j=1}^{m}}\bTheta_j^T\tilde{\bV}_j)\tilde{\bV}_i^T-{m}\bTheta_i^T\|
\\\leq &\|({\sum_{j=1}^{m}}\bTheta_j^T\tilde{\bV}_j)-{m}\bI\|+{m}\|\tilde{\bV}_i-\bTheta_i\|
{=} 
\|\bTheta^T\tilde{\bV}-m\bI\|+m\|\tilde{\bV}_i-\bTheta_i\|.\nonumber
\end{align}
Applying \eqref{eq:j_exclude_i2} and $\bS_{ij}=\bW_{ij}+\bTheta_i\bTheta_j^T$ when $i\neq j$, the RHS of \eqref{eq:pertubation_1} is bounded by 
\[
m\max_{1\leq i\leq m}\|\tilde{\bV}_i-\bTheta_i\|+\max_{1\leq i\leq m}\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|+\|\bTheta^T\tilde{\bV}-m\bI\| {+\|\bW\|}
.
\]

(ii)  
% Applying \eqref{eq:tildeTstar2} and \eqref{eq:tildeT2}, we have \[
% [\hat{\bT}^{(2)}]_{ii}=(\sum_{j=1,j\neq i}^{m}\bS_{ij}\tilde{\bV}_j)\tilde{\bV}_i^T.
% \]
{%
Combining %it 
equation \eqref{eq:tildeT2}
with \eqref{eq:j_exclude_i}}, 
% \begin{align*}
% &\|\tilde{\bV}_i^T[\bT^{(2)}]_{ii}\tilde{\bV}_i-(m-1)\bI\|=\left\|\tilde{\bV}_i^T\Big(\sum_{j=1,j\neq i}^m\bS_{ij}\tilde{\bV}_j\Big)-(m-1)\bI\right\|\\\leq& \|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|+\left\|\tilde{\bV}_i^T\bTheta_i \Big(\sum_{j=1,j\neq i}^m{\bTheta}_j^T\tilde{\bV}_j\Big)-(m-1)\bI\right\|\\\leq &\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+\|\tilde{\bV}_i^T\bTheta_i-\bI\|\Big\|\sum_{j=1,j\neq i}^m{\bTheta}_j^T\tilde{\bV}_j\Big\|+\left\|\sum_{j=1,j\neq i}^m{\bTheta}_j^T\tilde{\bV}_j-(m-1)\bI\right\|%\\\leq& (m-1)\|\tilde{\bV}_i^T\bTheta_i-\bI\|+\left(\|\sum_{j=1}^m{\bV}_j^T\tilde{\bV}_j-m\bI\|+\|\tilde{\bV}_i^T\bTheta_i-\bI\|\right)+\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|
% \\\leq &
% \Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+(m-1)\|\tilde{\bV}_i^T\bTheta_i-\bI\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|+\|\bTheta_i-\tilde{\bV}_i\|\\
% =&\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+m\|\tilde{\bV}_i^T\bTheta_i-\bI\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|.
% \end{align*}
\begin{align*}
&\|\tilde{\bV}_i^T[\bT^{(2)}]_{ii}\tilde{\bV}_i-{m}\bI\|
=
\left\|\tilde{\bV}_i^T\Big({\sum_{j=1}^m}\bS_{ij}\tilde{\bV}_j\Big)-{m}\bI\right\|\\\leq& \|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|+\left\|\tilde{\bV}_i^T\bTheta_i \Big({\sum_{j=1}^m}{\bTheta}_j^T\tilde{\bV}_j\Big)-{m}\bI\right\|\\\leq &\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+\|\tilde{\bV}_i^T\bTheta_i-\bI\|\Big\|{\sum_{j=1}^m}{\bTheta}_j^T\tilde{\bV}_j\Big\|+\left\|{\sum_{j=1}^m}{\bTheta}_j^T\tilde{\bV}_j-{m}\bI\right\|
\\\leq &
\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+{m}\|\tilde{\bV}_i^T\bTheta_i-\bI\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|
\end{align*}



\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:noisy2}]
Define $\hat{\bT}^{(1)}$ and $\hat{\bT}^{(2)}$ as follows:
\[
\hat{\bT}^{(1)}_{ij}=\bT^{(1)}_{ij}\,\,\text{and $\hat{\bT}^{(2)}_{ij}=\bT^{(2)}_{ij}$ for $i\neq j$, $\hat{\bT}^{(1)}_{ii}=\bT^{(1)}_{ii}-c\Proj_{\tilde{\bV}_i^\perp}$, and $\hat{\bT}^{(2)}_{ii}=\bT^{(2)}_{ii}-c\Proj_{\tilde{\bV}_i}.$}
\]
Clearly, $\bS=\hat{\bT}^{(1)}+\hat{\bT}^{(2)}+c\bI$, $\Proj_{\tilde{\bV}^\perp}\hat{\bT}^{(1)}\Proj_{\tilde{\bV}^\perp}=\hat{\bT}^{(1)}$, and $\hat{\bT}^{(2)}_{ii}=\Proj_{\tilde{\bV}_i}\hat{\bT}^{(2)}_{ii} \Proj_{\tilde{\bV}_i}$. It remains to show that $P_{\tilde{\bV}_i}^T\hat{\bT}^{(2)}_{ii} P_{\tilde{\bV}_i}$ and $-P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ are  positive definite matrices. 

Applying \eqref{eq:noisy2} {and Weyl's inequality,} and noting that $\|\tilde{\bV}_i^T\bTheta_i-\bI\|\leq \|\tilde{\bV}_i-\bTheta_i\|$, $P_{{\tilde{\bV}_i}}^T\hat{\bT}^{(2)}_{ii}P_{{\tilde{\bV}_i}}$ is positive definite for all $1\leq i\leq m$ if
\begin{equation}\label{eq:noisy2_1}
%m-1
{m}
>c+\max_{1\leq i\leq m}\Big\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_i\Big\|+m\max_{1\leq i\leq m}\|\tilde{\bV}_i-\bTheta_i\|+\|{\bTheta}^T\tilde{\bV}-m\bI\|.
\end{equation}


To prove that $-P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ is  positive definite, we first define $\hat{\bT}^{(1)*}$ as follows (similar to the definition of $\hat{\bT}^{(1)}$):
\[
\hat{\bT}^{(1)*}_{ij}=\bT^{(1)*}_{ij},\,\,\hat{\bT}^{(1)*}_{ii}=\bT^{(1)*}_{ii}-c%\Proj_{{\bV}_i^\perp}.
{\Proj_{{\bTheta}_i^\perp}}
.
\] 
If we define the subspace $L_3=L_2^\perp=\{\bx\in\reals^D: \bx_i\in\Sp(\bTheta_i^\perp)\}$, then we have  %$\bT^{(1)*}=-m\Proj_{L_2\cap L_1^\perp}-c\Proj_{L_3}$.
${\hat{\bT}^{(1)*}}=-m\Proj_{L_2\cap L_1^\perp}-c\Proj_{L_3}$.
Considering that $\dim(L_2\cap L_1^\perp)=\dim(L_2)-\dim(L_1)=rm-r$ and $\dim(L_3)=D-\dim(L_2)=D-rm$, we have 
\[
\lambda_{r+1}(\hat{\bT}^{(1)*})=-c.
\]
Applying Weyl's inequality on the perturbation of eigenvalue and $\|\bTheta_i\bTheta_i^T-\tilde{\bV}_i\tilde{\bV}_i^T\|=\|\bTheta_i(\bTheta_i-\tilde{\bV}_i)^T+(\tilde{\bV}_i-\bTheta_i)\tilde{\bV}_i^T\|\leq 2\|\bTheta_i-\tilde{\bV}_i\|$,
\begin{align*}
&|\lambda_{r+1}(\hat{\bT}^{(1)*})-\lambda_{r+1}(\hat{\bT}^{(1)})|\leq \|\hat{\bT}^{(1)*}-\hat{\bT}^{(1)}\|\leq \|{\bT}^{(1)*}-{\bT}^{(1)}\|+c\max_{1\leq i\leq m}%\|\Proj_{{\bV}_i^\perp}-\Proj_{\tilde{\bV}_i^\perp}\|\\
\|{\Proj_{{\bTheta}_i^\perp}}-\Proj_{\tilde{\bV}_i^\perp}\|\\
= &\|{\bT}^{(1)*}-{\bT}^{(1)}\|+c\max_{1\leq i\leq m}\|\bTheta_i\bTheta_i^T-\tilde{\bV}_i\tilde{\bV}_i^T\|\leq \|{\bT}^{(1)*}-{\bT}^{(1)}\|+2c\max_{1\leq i\leq m}\|\bTheta_i-\tilde{\bV}_i\|.
\end{align*}
Combining it with \eqref{eq:noisy1}, when
\begin{equation}\label{eq:noisy2_2}c>(m+2c)\max_{1\leq i\leq m}\|\tilde{\bV}_i-\bTheta_i\|+\max_{1\leq i\leq m}\|\sum_{j=1}^m\bW_{ij}\tilde{\bV}_j\|+\|\bTheta^T\tilde{\bV}-m\bI\|
{+\|\bW\|}
,
\end{equation}
$\lambda_{r+1}(\hat{\bT}^{(1)})$ is negative, which means that $\hat{\bT}^{(1)}$ has at least $D-r$ negative eigenvalues. By definition, $\hat{\bT}^{(1)}$ has $r$ zeros eigenvalues with eigenvectors spanning the column space of $\tilde{\bV}$, so $P_{\tilde{\bV}^\perp}^T\hat{\bT}^{(1)}P_{\tilde{\bV}^\perp}$ is negative definite. 

Let %$c=(m-1)/2$, 
{$c=m/2$}.
then both \eqref{eq:noisy2_1} and \eqref{eq:noisy2_2} would hold under the assumption of \eqref{eq:noisy2_0}, and Lemma~\ref{lemma:noisy2} is proved.  
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma:pertubation}]
First, we remark that the choice of $\tilde{\bV}\in\reals^{D\times r}$ is only unique up to an $r\times r$ orthogonal matrix. That is, for any orthogonal matrix $\bO\in\reals^{r\times r}$, $\tilde{\bV}\bO$ is also a potential choice. In this proof, we choose $\tilde{\bV}$ such that $\bTheta^T\tilde{\bV}\in \reals^{r\times r}$ is a symmetric, positive semidefinite matrix, and as a result, $\tr(\bTheta^T\tilde{\bV})=\|\bTheta^T\tilde{\bV}\|_*$. 


Then we have that
\begin{align}\label{eq:pertubation1}
&\|\tilde{\bV}-\bTheta\|_F^2=\sum_{i=1}^m\|\tilde{\bV}_i-\bTheta_i\|_F^2=\sum_{i=1}^m\|\tilde{\bV}_i\|_F^2+\|\bTheta_i\|_F^2-2\tr(\tilde{\bV}_i\bTheta_i^T)=\sum_{i=1}^m\|\tilde{\bV}_i\|_F^2+\|\bTheta_i\|_F^2-2\tr(\bTheta_i^T\tilde{\bV}_i)\\=&2rm-2\tr(\sum_{i=1}^m\bTheta_i^T\tilde{\bV}_i)=2rm-2\tr(\bTheta^T\tilde{\bV})=2rm-2\|\bTheta^T\tilde{\bV}\|_*,
\end{align}
where $\|\cdot\|_*$ represents the nuclear norm that is the summation of all singular values (and since $\bV^T\tilde{\bV}$ is positive semidefinite, it is also the summation of its eigenvalues).

Using the definition in \eqref{eq:tracesum_problem1}, we have
\begin{align}\label{eq:pertubation2}
\tr(\tilde{\bV}^T\bS\tilde{\bV})\geq 
\tr({\bTheta}^T\bS{\bTheta}).
\end{align}
Applying $\bS=\bTheta\bTheta^T+\bW$, \eqref{eq:pertubation2} implies
\begin{align*}
&\tr(\tilde{\bV}^T\bW\tilde{\bV})+\|\tilde{\bV}^T\bTheta\|_F^2=\tr(\tilde{\bV}^T\bW\tilde{\bV})+\tr(\tilde{\bV}^T\bTheta\bTheta^T\tilde{\bV})\geq \tr(\bTheta^T\bW\bTheta)+\tr(\bTheta^T\bTheta\bTheta^T\bTheta)\\=&\tr(\bTheta^T\bW\bTheta)+\|\bTheta^T\bTheta\|_F^2
\end{align*}
and
\begin{align}\label{eq:pertubation4}
\tr(\tilde{\bV}^T\bW\tilde{\bV})-\tr({\bTheta}^T\bW{\bTheta})\geq \|\bTheta^T\bTheta\|_F^2-\|\tilde{\bV}^T\bTheta\|_F^2=rm^2-\|\tilde{\bV}^T\bTheta\|_F^2.
\end{align}
Since $\|\bX\|_F^2=\sum_{i}\lambda_i(\bX)^2$, we have
\begin{align}\label{eq:pertubation5}
rm^2-\|\tilde{\bV}^T\bTheta\|_F^2=\sum_{i=1}^r(m^2-\lambda_i(\tilde{\bV}^T\bTheta)^2)\geq m \sum_{i=1}^r(m-\lambda_i(\tilde{\bV}^T\bTheta))=m(rm-\|\tilde{\bV}^T\bTheta\|_*).
\end{align}
The combination \eqref{eq:pertubation4}, \eqref{eq:pertubation5}, $\|\tilde{\bV}\|_F=\|\bTheta\|_F=\sqrt{rm}$,  $\tr(\bA\bB)\leq \|\bA\|_F\|\bB\|_F$, and $\|\bA\bB\|_F\leq \|\bA\|\|\bB\|_F$ implies that
\begin{align*}
&m(rm-\|\tilde{\bV}^T\bTheta\|_*)\leq \tr(\tilde{\bV}^T\bW\tilde{\bV})-\tr({\bTheta}^T\bW{\bTheta})
=\tr((\tilde{\bV}-\bTheta)^T\bW\tilde{\bV})+\tr(\bTheta^T\bW(\tilde{\bV}-\bTheta))\\
\leq& \|\bW\|\|\tilde{\bV}-\bTheta\|_F\|\tilde{\bV}\|_F+\|\bW\|\|\tilde{\bV}-\bTheta\|_F\|{\bTheta}\|_F=2\|\bW\|\|\tilde{\bV}-\bTheta\|_F\sqrt{rm}.
\end{align*}
Combining it with \eqref{eq:pertubation1}, we have
\begin{align}\label{eq:pertubation6}
\frac{m}{2}\|\tilde{\bV}-\bTheta\|_F^2\leq 2\|\bW\|\|\tilde{\bV}-\bTheta\|_F\sqrt{rm},
\end{align}
which implies that
\begin{align}\label{eq:pertubation7}
\|\tilde{\bV}-\bTheta\|_F\leq 4\|\bW\|\sqrt{\frac{r}{m}},
\end{align}
which proves the first inequality in \eqref{eq:lemma_pertubation1}. It implies that
\begin{align}\label{eq:pertubation7.5}
\|\tilde{\bV}\bTheta^T-m\bI\|_F=\|(\tilde{\bV}-\bTheta)\bTheta^T\|_F\leq \|\tilde{\bV}-\bTheta\|_F\|\bTheta\|= \|\tilde{\bV}-\bTheta\|_F\sqrt{m}\leq 4\|\bW\|\sqrt{r}.
\end{align}
Applying \eqref{eq:pertubation7}, the second inequality in \eqref{eq:lemma_pertubation1} is proved:
\begin{align}\nonumber&\max_{1\leq i\leq m}\|[\bW\tilde{\bV}]_i\|_F\leq \max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+\max_{1\leq i\leq m}\|[\bW(\tilde{\bV}-\bTheta)]_i\|_F\leq \max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F\\&+\|\bW\|\|\tilde{\bV}-\bTheta\|_F
\leq \max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+4\|\bW\|^2\sqrt{\frac{r}{m}}.\label{eq:pertubation13}
\end{align}

Now let us consider $\bar{\bV}\in\reals^{D\times r}$ defined by $\bar{\bV}_i=\bTheta_i$ and $\bar{\bV}_j=\tilde{\bV}_j$ for all $1\leq j\leq m, j\neq i$. By definition we have
\[
\tr(\tilde{\bV}^T\bS\tilde{\bV})\geq 
\tr(\bar{\bV}^T\bS\bar{\bV}),
\]
and it is equivalent to
\[
\tr((\tilde{\bV}-\bar{\bV})^T\bS\tilde{\bV})+
\tr( {\tilde{\bV}^T}\bS(\tilde{\bV}-\bar{\bV}))-\tr((\tilde{\bV}-\bar{\bV})^T\bS(\tilde{\bV}-\bar{\bV}))\geq 0.
\]
By the definition of $\bar{\bV}$, $\tilde{\bV}$, and $\bS$, we have
\begin{equation}\label{eq:pertubation_10}
%2\tr((\tilde{\bV}_i-\bTheta_i)^T\bTheta_i\bTheta^T\tilde{\bV})+2\tr((\tilde{\bV}_i-\bTheta_i)^T\bW^T\tilde{\bV})-\tr((\tilde{\bV}_i-\bTheta_i)^T\bS_{ii}(\tilde{\bV}_i-\bTheta_i))\geq 0.
2\tr((\tilde{\bV}_i-\bTheta_i)^T\bTheta_i\bTheta^T\tilde{\bV})+2\tr((\tilde{\bV}_i-\bTheta_i)^T[\bW\tilde{\bV}]_i)-\tr((\tilde{\bV}_i-\bTheta_i)^T\bS_{ii}(\tilde{\bV}_i-\bTheta_i))\geq 0.
\end{equation}

% and notice that $\bS_{ii}=\mathbf{0}$, we have
% \[
% 2\tr\left((\bTheta_i-\tilde{\bV}_i)^T[\bS\tilde{\bV}]_i\right)\leq 0.
% \]
% By the definition of $\bS$, it implies that
% \begin{align}\label{eq:pertubation10}
% \tr\left((\bTheta_i-\tilde{\bV}_i)^T\bTheta_i\bV^T\tilde{\bV}- (\bTheta_i-\tilde{\bV}_i)^T\bTheta_i\bTheta_i^T\tilde{\bV}_i+(\bTheta_i-\tilde{\bV}_i)^T[\bW\tilde{\bV}]_i\right)\leq 0
% \end{align}
Recall that $\tilde{\bV}$ is chosen such that $\bTheta^T\tilde{\bV}$ is symmetric, positive semidefinite, and apply the fact that when $\bA$ is positive semidefinite, then $\tr(\bB\bA)=\tr(\bB^T\bA)$ and when both $\bA, \bB$ are p.s.d., $\tr(\bA\bB)\geq \tr(\bA\lambda_{\min}(\bB)\bI)\geq \lambda_{\min}(\bB)\tr(\bA)$ ($\lambda_{\min}$ represents the smallest eigenvalue), we have
\begin{align}\label{eq:pertubation11}
&\tr\left((\bTheta_i-\tilde{\bV}_i)^T\bTheta_i\bTheta^T\tilde{\bV}\right)=
\tr\left((\bI-\tilde{\bV}_i^T\bTheta_i)(\bTheta^T\tilde{\bV})\right)=
\frac{1}{2}\tr\left((2\bI-\tilde{\bV}_i^T\bTheta_i-\bTheta_i^T\tilde{\bV}_i)(\bTheta^T\tilde{\bV})\right)\\=&\frac{1}{2}\tr\left((\tilde{\bV}_i-\bTheta_i)^T(\tilde{\bV}_i-\bTheta_i)(\bTheta^T\tilde{\bV})\right)\geq \frac{1}{2}\tr\left((\tilde{\bV}_i-\bTheta_i)^T(\tilde{\bV}_i-\bTheta_i)\right)\lambda_r(\bTheta^T\tilde{\bV})=\frac{1}{2}\|\tilde{\bV}_i-\bTheta_i\|_F^2\lambda_r(\bTheta^T\tilde{\bV}).\nonumber
\end{align}
In addition, we have
\begin{equation}\label{eq:pertubation_12}
\tr((\tilde{\bV}_i-\bTheta_i)^T\bS_{ii}(\tilde{\bV}_i-\bTheta_i))\geq -\|\bS_{ii}\|\|\tilde{\bV}_i-\bTheta_i\|_F^2\geq -(1+\|\bW_{ii}\|)\|\tilde{\bV}_i-\bTheta_i\|_F^2
\end{equation}
and $\tr(\bA\bB)\leq \|\bA\|_F\|\bB\|_F$ implies
\begin{equation}\label{eq:pertubation_14}
%\tr((\tilde{\bV}_i-\bTheta_i)^T\bW^T\tilde{\bV})\leq \|\tilde{\bV}_i-\bTheta_i\|_F\|\bW^T\tilde{\bV}\|_F. 
\tr((\tilde{\bV}_i-\bTheta_i)^T[\bW\tilde{\bV}]_i)\leq \|\tilde{\bV}_i-\bTheta_i\|_F\|\bW^T\tilde{\bV}\|_F. 
\end{equation}
Combining \eqref{eq:pertubation_10},  \eqref{eq:pertubation11}, \eqref{eq:pertubation_12}, and \eqref{eq:pertubation_14},
\[
\|\tilde{\bV}_i-\bTheta_i\|_F%\|\bW^T\tilde{\bV}\|_F
 {\|[\bW\tilde{\bV}]_i\|_F}
\geq \|\tilde{\bV}_i-\bTheta_i\|_F^2%\left(\frac{\lambda_r(\bTheta^T\tilde{\bV})}{2}-1-\|\bW_{ii}\|\right).
 {(\lambda_r(\bTheta^T\tilde{\bV})-1-\|\bW_{ii}\|)}
.
\]
Combining it with \eqref{eq:pertubation13} and \eqref{eq:pertubation7.5} which implies that $\lambda_r(\bTheta^T\tilde{\bV})\geq m-4\|\bW\|\sqrt{r}$,
 {and noting that $\|\bW\| \ge \|\bW_{ii}\|$,}
\eqref{eq:lemma_pertubation2} is proved.
% Combining \eqref{eq:pertubation10}, \eqref{eq:pertubation11}, and $\tr(\bA\bB)\leq \|\bA\|_F\|\bB\|_F,$ we have
% \[\frac{1}{2}\lambda_r(\bTheta^T\tilde{\bV})\|\bTheta_i-\tilde{\bV}_i\|_F^2\leq \|\bTheta_i-\tilde{\bV}_i\|_F(\|[\bW\tilde{\bV}]_i\|_F+\sqrt{r})\]
% Since it holds for all $1\leq i\leq m$, 
% \begin{align}\label{eq:pertubation12}
% \frac{1}{2}\lambda_r(\bTheta^T\tilde{\bV})\max_{1\leq i\leq m}\|\bTheta_i-\tilde{\bV}_i\|_F\leq \max_{1\leq i\leq m}\|[\bW\tilde{\bV}]_i\|_F+\sqrt{r}.\end{align}
% Combining \eqref{eq:pertubation13} with \eqref{eq:pertubation7.5} (which implies that $\lambda_r(\bTheta^T\tilde{\bV})\geq m-4\|\bW\|\sqrt{r}$), and \eqref{eq:pertubation12}, \eqref{eq:lemma_pertubation2} is proved.
\end{proof}
%\subsection{Lemma~\ref{lemma:pertubation} in the MAXBET setting}\label{sec:MAXBET}
\subsection*{Lemma~\ref{lemma:pertubation} in the MAXDIFF setting}\label{sec:MAXBET}
\begin{proof}[Proof of Lemma~\ref{lemma:pertubation} in the  {MAXDIFF} setting]
Following the proof of  Lemma~\ref{lemma:pertubation}, we have
\begin{align*}
&2\|\bW\|\|\tilde{\bV}-\bTheta\|_F\sqrt{rm}\geq \tr(\tilde{\bV}^T\bW\tilde{\bV})-\tr({\bTheta}^T\bW{\bTheta})\geq (rm^2-\|\tilde{\bV}^T\bTheta\|_F^2)-(rm-\sum_{1\leq i\leq m}\|\tilde{\bV}_i^T\bTheta_i\|_F^2)\\
\geq &\frac{m}{2}\|\tilde{\bV}-\bTheta\|_F^2-\sum_{i=1}^m\|\tilde{\bV}_i-\bTheta_i\|_F^2=(\frac{m}{2}-1)\|\tilde{\bV}-\bTheta\|_F^2
,
\end{align*}
{ %
where the first inequality is \eqref{eq:pertubation5},
the second inequality is from the definition of $\bS$ under the MAXDIFF setting, and the third inequality is from
\[
    r - \|\tilde{\bV}_i^T\bTheta_i\|_F^2
    \le \|\tilde{\bV}_i - \bTheta_i\|_F^2
    = 2r - \tr(\tilde{\bV}_i^T\bTheta_i)
    ,
\]
since $\|\tilde{\bV}_i^T\bTheta\|_F^2 - 2\tr(\tilde{\bV}_i^T\bTheta) + r = \|\tilde{\bV}_i^T\bTheta_i - \bI_r\|_F^2$.}

As a result,  {if $m > 2$},
\[
\|\tilde{\bV}-\bTheta\|_F\leq \frac{4\|\bW\|\sqrt{rm}}{m-2},\,\,
\|\tilde{\bV}^T\bTheta- {m}\bI\|_F\leq \frac{4\|\bW\|m\sqrt{r}}{m-2},\,\,
\max_{1\leq i\leq m}\|[\bW\tilde{\bV}]_i\|_F\leq
\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+\frac{4\|\bW\|^2\sqrt{rm}}{m-2}.
\]
In addition, \eqref{eq:pertubation_10} is replaced with
\begin{equation}
%2\tr((\tilde{\bV}_i-\bTheta_i)^T\bTheta_i\bTheta^T\tilde{\bV})+2\tr((\tilde{\bV}_i-\bTheta_i)^T\bW^T\tilde{\bV})-2\tr((\tilde{\bV}_i-\bTheta_i)^T\bTheta_i\bTheta_i^T\tilde{\bV}_i)\geq 0.
2\tr((\tilde{\bV}_i-\bTheta_i)^T\bTheta_i\bTheta^T\tilde{\bV})+2\tr((\tilde{\bV}_i-\bTheta_i)^T[\bW\tilde{\bV}]_i)
\geq 0.
\end{equation}
Then we have
%\[\frac{1}{2}\lambda_r(\bTheta^T\tilde{\bV})\|\bTheta_i-\tilde{\bV}_i\|_F^2\leq \|\bTheta_i-\tilde{\bV}_i\|_F(\|[\bW\tilde{\bV}]_i\|_F+\sqrt{r})\]
\[
\frac{1}{2}\lambda_r(\bTheta^T\tilde{\bV})\|\bTheta_i-\tilde{\bV}_i\|_F^2\leq \|\bTheta_i-\tilde{\bV}_i\|_F(\|[\bW\tilde{\bV}]_i\|_F)
\]
and
\[
%\|\bTheta_i-\tilde{\bV}_i\|_F\leq \frac{\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+\frac{4\|\bW\|^2\sqrt{rm}}{m-2}+\sqrt{r}}{\frac{1}{2}(m-\frac{4\|\bW\|\sqrt{rm}}{m-2})}.
\max_{1\le i\le m}\|\bTheta_i-\tilde{\bV}_i\|_F\leq \frac{2\max_{1\leq i\leq m}\|[\bW{\bTheta}]_i\|_F+\frac{8\|\bW\|^2\sqrt{rm}}{m-2}}{m-\frac{4\|\bW\|m\sqrt{r}}{m-2}}
\]
 {%
for $m > 4\|\bW\|\sqrt{r}+2$.
}
\end{proof}

\subsection{Proof of  lemmas for \Cref{thm:main2}}\label{sec:proofs}
\iffalse
\begin{proof}[Proof of \Cref{prop:positivity}]
	Let $\tau_i=\lambda_{\min}(\bLambda_i)$ and $\bv_i\in\mathbb{R}^r$ be the associated unit eigenvector, i.e., $\bLambda_i\bv_i = \tau_i\bv_i$.
	If $\bO_i^{\perp}\in\mathcal{O}_{d_i-r,r}$ fills out $\bO_i$ to a full orthogonal matrix,
	then for any $\bx_i \in \mathbb{R}^{d_i-r}$, $\bW_i=\bO_i^{\perp}\bx_i\bv_i^T$ and $\bW_j = \bzero$ for $j\neq i$ satisfy the tangency condition \eqref{eqn:tangent}. Furthermore, $\tr(\bW^T\bS\bW)=0$, 
	\begin{align*}
	\tr(\bLambda_i\bW_i^T\bW_i) &= \tr(\bLambda_i \bv_i\bx_i^T\bO_i^{\perp T}\bO_i^{\perp}\bx_i\bv_i^T)
	\\
	&= \tr(\bLambda_i \bv_i\bx_i^T\bx_i\bv_i^T)
	\\
	&= \|\bx_i\|^2\bv_i^T\bLambda_i\bv_i = \|\bx_i\|^2\tau_i
	\end{align*}
	and $\tr(\bLambda_j\bW_j^T\bW_j) = 0$ for $j\neq i$.
	Then the second-order condition \eqref{eqn:second} entails
	$$
	0 \le \sum_{i=1}^m \tr(\bLambda_i\bW_i^T\bW_i) - \tr(\bW^T\bS\bW) 	= \tau_i\|\bx_i\|^2
	.
	$$
	Thus $\tau_i \ge 0$.
\end{proof}
\fi


\iffalse
\begin{proof}[Proof of Proposition \ref{prop:qualification}]
	Since $\bO$ is a second-order critical point, matrix
	$$
		\bLambda_i = \sum_{j\neq i}\bO_i^T\bS_{ij}\bO_j
	$$
	is symmetric and positive definite for $i=1, \dots, m$. Therefore $\sum_{i=1}^m\bLambda_i \psdge \bzero$.
	Then it follows
	$$
		0 \le \tr(\sum_{i=1}^m\bLambda_i)
		\le \sum_{i=1}^m\sum_{j\neq i}\tr(\bO_i^T\bS_{ij}\bO_j) = \tr(\bO^T\bS\bO)
		.
	$$
\end{proof}
\fi
\iffalse
\begin{proof}[Proof of Proposition \ref{prop:upperbound1}]
	Note $\bO_i^T\bO_i=\bI_r=\bTheta_i^T\bTheta_i$ and $\bO^T\bO=m\bI_r=\bTheta^T\bTheta$.

	From Assumption \eqref{assumption} and expansion \eqref{eqn:Sexpansion},
	\begin{align*}
		m^2r - mr + \tr(\bTheta^T\bW\bTheta)
		&=
		\tr(\bTheta^T\bTheta\bTheta^T\bTheta)
		- \sum_{i=1}^m\tr(\bTheta_i^T\bTheta_i\bTheta_i^T\bTheta_i)
		+ \tr(\bTheta^T\bW\bTheta)
		\\
		&=
		\tr(\bTheta^T\bS\bTheta)
		\\
		&\le
		\tr(\bO^T\bS\bO)
		\\
		&=
		\tr(\bO^T\bTheta\bTheta^T\bO)
		- \sum_{i=1}^m\tr(\bO_i^T\bTheta_i\bTheta_i^T\bO_i)
		+ \tr(\bO^T\bW\bO)
		\\
		&=
		\|\bTheta^T\bO\|_{\rm F}^2 
		- \sum_{i=1}^m\tr(\bO_i^T\bTheta_i\bTheta_i^T\bO_i)
		+ \tr(\bO^T\bW\bO)
	\end{align*}
	Thus
	\begin{align}\label{eqn:upperbound1_1}
		m^2r - \|\bTheta^T\bO\|_{\rm F}^2 - mr  
		&+ \sum_{i=1}^m\tr(\bO_i^T\bTheta_i\bTheta_i^T\bO_i)
		\nonumber\\
		&\le
		\tr(\bO^T\bW\bO) - \tr(\bTheta^T\bW\bTheta)
		\nonumber\\
		&=
		\tr((\bO-\bTheta)^T\bW\bO) 
		+ \tr(\bTheta^T\bW(\bO-\bTheta))
		\nonumber\\
		&\le
		\|(\bO-\bTheta)^T\bW\|_{\rm F}\|\bO\|_{\rm F}
		+
		\|\bTheta\|_{\rm F}\|\bW(\bO-\bTheta)\|_{\rm F}
		\nonumber\\
		&\le
		\|\bO-\bTheta\|_{\rm F}\|\bW\|_2\|\bO\|_{\rm F}
		+
		\|\bTheta\|_{\rm F}\|\bW\|_2\|\bO-\bTheta\|_{\rm F}
		\nonumber\\
		&=
		2\sqrt{mr}\|\bW\|_2\|\bO-\bTheta\|_{\rm F}
	\end{align}
	where the second inequality is Cauchy-Schwarz,
	and the third inequality is from $\|\bA\bB\|_{\rm F} \le \|\bA\|_2\|\bB\|_{\rm F}$.

	Recall
	\begin{align*}
	\|\bO-\bTheta\|_{\rm F}^2 
	&= \|\bO\|_{\rm F}^2 + \|\bTheta\|_{\rm F}^2
		- 2\tr(\bTheta^T\bO)
	\\
	&= 2(mr - \tr(\bTheta^T\bO))
	.
	\end{align*}
	From the condition \eqref{eqn:wlog}, it follows that
	\begin{align*}
	m(mr - \tr(\bTheta^T\bO))
	&=
	m\sum_{j=1}^r[m - \lambda_j(\bTheta^T\bO)]
	\\
	&\le
	\sum_{j=1}^r [m + \lambda_j(\Theta^T\bO)][m - \lambda_j(\Theta^T\bO)]
	\\
	&=
	\sum_{j=1}^r [m^2 - \lambda_j^2(\Theta^T\bO)]
	= m^2r - \|\bTheta^T\bO\|_{\rm F}^2
	.
	\end{align*}
	Combining this with inequality \eqref{eqn:upperbound1_1},
	we obtain
	\begin{align*}
		2\sqrt{mr}\|\bW\|_2\|\bO-\bTheta\|_{\rm F}
		&\ge
		m^2r - \|\bTheta^T\bO\|_{\rm F}^2 - mr + \sum_{i=1}^m\tr(\bO_i^T\bTheta_i\bTheta_i^T\bO_i)
		\\
		&\ge
		\frac{m}{2}\|\bO-\bTheta\|_{\rm F}^2 - mr + \sum_{i=1}^m\tr(\bO_i\bO_i^T\bTheta_i\bTheta_i^T)
		\\
		&\ge
		\frac{m}{2}\|\bO-\bTheta\|_{\rm F}^2 - mr 
		.
	\end{align*}
	The last inequality holds because both $\bO_i\bO_i^T$ and $\bTheta_i\bTheta_i^T$ are positive semidefinite.
	
	Solving the quadratic inequality for $\|\bO-\bTheta\|_{\rm F} \ge 0$, we have
	$$
		\|\bO-\bTheta\|_{\rm F} \le \sqrt{\frac{r}{m}}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})
		.
	$$
	The desire result follows since $\|\bO-\bTheta\|_2 \le \|\bO - \bTheta\|_{\rm F}$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:upperbound2}]
	\begin{align*}
	\|(\bW\bO)_i\|_2
	\le 
	\|(\bW\bO)_i\|_{\rm F}
	&\le
	\|[\bW(\bO-\bTheta)]_i\|_{\rm F} + \|(\bW\bTheta)_i\|_{\rm F}
	\\
	&\le
	\|\bW_{i\cdot}(\bO-\bTheta)\|_{\rm F} + \|(\bW\bTheta)_i\|_{\rm F}
	\\
	&\le
	\|\bW_{i\cdot}\|_2\|\bO-\bTheta\|_{\rm F} + \|(\bW\bTheta)_i\|_{\rm F}
	\\
	&\le
	\|\bW\|_2\|\bO-\bTheta\|_{\rm F} + \|(\bW\bTheta)_i\|_{\rm F}
	,
	\end{align*}
	where $\bW_{i\cdot}=[\bW_{i1}, \bW_{i2}, \dotsc, \bW_{im}]=[\bzero, \cdots, \bzero, \bI_{d_i}, \bzero, \dotsc, \bzero]\bW$.
	The third inequality is from $\|\bA\bB\|_{\rm F} \le \|\bA\|_2\|\bB\|_{\rm F}$.
\end{proof}

To prove Proposition \ref{prop:upperbound3}, we need the following lemma:
\fi

\begin{proof}[Proof of \Cref{lem:weyllocal}]
    From $\bO_i\bLambda_i = \sum_{j=1}^m\bS_{ij}\bO_j$, we have $\bLambda_i = \sum_{j=1}^m\bO_i^T\bS_{ij}\bO_j$. 
    Hence, under the MAXBET model,
    \begin{align*}
        \|\bLambda_i - m\bI_r\|
        &= \|\sum_{j=1}^m\bO_i^T\bS_{ij}\bO_j- m\bI_r\|
        \\
        &\leq
        \|\bO_i^T\sum_{j=1}^m\bW_{ij}\bO_j\|
        + \|\bO_i^T\bTheta_i\sum_{j=1}^m\bTheta_j^T\bO_j - m\bI_r\|
        \\
        &\leq
        \|\sum_{j=1}^m\bW_{ij}\bO_j\|
        + \|(\bO_i^T\bTheta_i - \bI_r)\sum_{j=1}^m\bTheta_j^T\bO_j + \sum_{j=1}^m\bTheta_j^T\bO_j - m\bI_r \|
        \\
        &\leq
        \|\sum_{j=1}^m\bW_{ij}\bO_j\|
        + \|(\bO_i^T\bTheta_i - \bI_r)\sum_{j=1}^m\bTheta_j^T\bO_j\| + \|\sum_{j=1}^m\bTheta_j^T\bO_j - m\bI_r \|
        \\        
        &\leq
        \|\sum_{j=1}^m\bW_{ij}\bO_j\|
        + \|\bO_i^T\bTheta_i - \bI_r\|\|\sum_{j=1}^m\bTheta_j^T\bO_j\| + \|\bTheta^T\bO - m\bI_r \|
        \\
        &\leq
        \|\sum_{j=1}^m\bW_{ij}\bO_j\|
        + m\|\bO_i^T\bTheta_i - \bI_r\| + \|\bTheta^T\bO - m\bI_r \|
    \end{align*}
    since $\|\bTheta_j^T\bO_j\| \le 1$.
    Under the MAXDIFF model,
    \begin{align*}
        \|\bLambda_i - (m-1)\bI_r\|
        &= \|\sum_{j\neq i}\bO_i^T\bS_{ij}\bO_j- (m-1)\bI_r\|
        \\
        &\leq
        \|\bO_i^T\sum_{j\neq i}\bW_{ij}\bO_j\|
        + \|\bO_i^T\bTheta_i\sum_{j \neq i}\bTheta_j^T\bO_j - (m-1)\bI_r\|
        \\
        &\leq
        \|\sum_{j \neq i}\bW_{ij}\bO_j\|
        + \|(\bO_i^T\bTheta_i - \bI_r)\sum_{j=1}^m\bTheta_j^T\bO_j + \sum_{j\neq i}\bTheta_j^T\bO_j - (m-1)\bI_r \|
        \\
        &\leq
        \|\sum_{j \neq i}\bW_{ij}\bO_j\|
        + \|(\bO_i^T\bTheta_i - \bI_r)\sum_{j \neq i}\bTheta_j^T\bO_j\| + \|\sum_{j \neq i}\bTheta_j^T\bO_j - (m-1)\bI_r \|
        \\        
        &\leq
        \|\sum_{j\neq i}\bW_{ij}\bO_j\|
        + \|\bO_i^T\bTheta_i - \bI_r\|\|\sum_{j \neq i}\bTheta_j^T\bO_j\| + \|\bTheta^T\bO - m\bI_r - \bTheta_i^T\bO_i + \bI_r \|
        \\
        &\leq
        \|\sum_{j \neq i}\bW_{ij}\bO_j\|
        + (m-1)\|\bO_i^T\bTheta_i - \bI_r\| + \|\bTheta^T\bO - m\bI_r \|
        + \|\bO_i^T\bTheta_i - \bI_r\|
        \\
        &=
        \|\sum_{j\neq i}\bW_{ij}\bO_j\|
        + m\|\bO_i^T\bTheta_i - \bI_r\| + \|\bTheta^T\bO - m\bI_r \|
        .
    \end{align*}    
\end{proof}

The following technical lemma is needed to prove \Cref{lem:upperboundlocal}.
\begin{lemma}\label{lem:normalcone}
	Suppose $\bX, \bY \in \mathcal{O}_{d,r}$ and $\bLambda \in \mathbb{R}^{d\times d}$ is symmetric and positive semidefinite.
	Then, there holds
	$$
	\langle \bX\bLambda, \bY - \bX \rangle \le 0
	.
	$$
\end{lemma}
\begin{proof}%[Proof of Lemma \ref{lem:normalcone}]
	\begin{align*}
		\langle \bX\bLambda, \bY - \bX \rangle 
		&\le
		\tr(\bLambda^T\bX^T(\bY-\bX))
		\\
		&=
		\tr(\bLambda(\bX^T\bY - \bI_r))
		\\
		&= 
		\tr(\bLambda\bX^T\bY) - \tr(\bLambda)
		\\
		&= 
		\tr(\bY^T\bX\bLambda) - \tr(\bLambda)
		\\
		&=
		\tr(\bLambda\bY^T\bX) - \tr(\bLambda)
		\\
		&=
		\tr\left[\bLambda\left(\frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX - \bI_r\right)\right]
		\\
		&=
		\left\langle \bLambda, \frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX - \bI_r \right\rangle
	\end{align*}
	Since $\bX\bX^T \psdle \bI_d$,
	$$
		(\bX^T\bY)^T(\bX^T\bY) = \bY^T\bX\bX^T\bY
		\psdle \bY^T\bY = \bI_r
		.
	$$
	Thus $\|\bX^T\bY\|_2 \le 1$.
	%Likewise, since $\bY\bY^T \psdle \bI_d$,
	%$$
		%(\bY^T\bX)^T(\bY^T\bX) = \bX^T\bY\bY^T\bX
		%\psdle \bX^T\bX = \bI_r
		%.
	%$$
	Likewise $\|\bY^T\bX\|_2 \le 1$. Then,
	because
	$\frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX$
	is symmetric,
	$$
	\lambda_{\max}\left(
		\frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX
	\right)
	\le
	\left\| \frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX \right\|_2 
	\le
	\frac{1}{2}\|\bX^T\bY\|_2 + \frac{1}{2}\|\bY^T\bX\|_2 \le 1
	$$
	and
	$$
		\frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX - \bI_r \psdle \bzero
		.
	$$
	Since $\bLambda \psdge \bzero$, it follows that
	$$
		\left\langle \bLambda, \frac{1}{2}\bX^T\bY + \frac{1}{2}\bY^T\bX - \bI_r \right\rangle
		\le 0
		.
	$$
\end{proof}
\iffalse
\begin{proof}[Proof of Proposition \ref{prop:upperbound3}]
	Since $\bO=(\bO_1,\dotsc,\bO_m)$ is a second-order critical point, the associated Lagrange multiplier $\bLambda_i$ of $\bO_i$ satisfies
	\begin{equation}\tag{\ref{eqn:firstorder}}
	\bO_i\bLambda_i = \sum_{j\neq i}\bS_{ij}\bO_j 
	\end{equation}
	and is symmetric, positive semidefinite by \Cref{prop:positivity}.
	Since $\bS_{ij} = \bTheta_i\bTheta_j^T + \bW_{ij}$ for $j\neq i$, 
	\begin{align*}
		\sum_{j\neq i}\bS_{ij}\bO_j 
		&=
		\sum_{j\neq i}\bTheta_i\bTheta_j^T\bO_j + \sum_{j\neq i}\bW_{ij}\bO_j
		\\
		&=
		\bTheta_i(\sum_{j\neq i}\bTheta_j^T\bO_j-\bTheta_i^T\bO_i) + (\bW\bO)_i
		\\
		&=
		\bTheta_i\bTheta^T\bO + (\bW\bO)_i
		.
	\end{align*}
	Thus from Lemma \ref{lem:normalcone}, we have
	\begin{align*}%\label{eqn:normalbound}
	0 &\ge \tr[(\bTheta_i-\bO_i)^T\sum_{j\neq i}\bS_{ij}\bO_j] 
	\\
	&= \tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO]
	- \tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta_i^T\bO_i]
	+ \tr[(\bTheta_i-\bO_i)^T(\bW\bO)_i]
	.
	\end{align*}
	The first term of the right-hand side of the above inequality can be further bounded:
	\begin{align*}
		\tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO]
		&=
		\tr[(\bI_r-\bO_i^T\bTheta_i)(\bTheta^T\bO)]
		\\
		&=
		\tr\left[\left(\bI_r-\frac{1}{2}\bO_i\bTheta_i^T-\frac{1}{2}\bTheta_i\bO_i^T)(\bTheta^T\bO)\right)\right]
		\\
		&\ge
		\tr\left(\bI_r-\frac{1}{2}\bO_i\bTheta_i^T-\frac{1}{2}\bTheta_i\bO_i^T\right)\lambda_{\min}(\bTheta^T\bO)
		\\
		&=
		\frac{1}{2}\|\bTheta_i-\bO_i\|_F^2\cdot\lambda_{\min}(\bTheta^T\bO)
	\end{align*}
	because of assumption \eqref{eqn:wlog}.
	Therefore
	\begin{align*}
		\lambda_{\min}(\bTheta^T\bO)\frac{1}{2}\|\bTheta_i-\bO_i\|_F^2
		&\le
		\tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO_i]
		- \tr[(\bTheta_i-\bO_i)^T(\bW\bO)_i]
		\\
		&\le
		\|\bTheta_i-\bO_i\|_{\rm F}\|\bTheta_i\bTheta_i^T\bO_i\|_{\rm F}
		+ \|\bTheta_i-\bO_i\|_{\rm F}\|(\bW\bO)_i\|_{\rm F}
		\\
		&\le
		\|\bTheta_i-\bO_i\|_{\rm F}\|\bTheta_i\bTheta_i^T\|_2\bO_i\|_{\rm F}
		+ \|\bTheta_i-\bO_i\|_{\rm F}\|(\bW\bO)_i\|_{\rm F}
		\\
		&\le
		\|\bTheta_i-\bO_i\|_{\rm F}\|\bO_i\|_{\rm F}
		+ \|\bTheta_i-\bO_i\|_{\rm F}\|(\bW\bO)_i\|_{\rm F}
		\\
		&=
		\|\bTheta_i-\bO_i\|_{\rm F}\sqrt{r}
		+ \|\bTheta_i-\bO_i\|_{\rm F}\|(\bW\bO)_i\|_{\rm F}
		.
	\end{align*}
	The second inequality is Cauchy-Schwarz;
	the third uses $\|\bA\bB\|_{\rm F}\le\|\bA\|_2\|\bB\|_{\rm F}$; the fourth is due to $\bTheta_i\bTheta_i^2 \psdle \bI_r$.
	Then we have
	\begin{equation}\label{eqn:intermediatebound}
		\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|_{\rm F}
		\le
		\frac{2(\max_{i=1,\dotsc,m}\|(\bW\bO)_i\|_{\rm F} + \sqrt{r})}{\lambda_{\min}(\bTheta^T\bO)}
		.
	\end{equation}
	Now we need a positive lower bound for $\lambda_{\min}(\bTheta^T\bO)$. From Proposition \ref{prop:upperbound1},
	$$
		\|\bTheta^T\bO-m\bI\|_2
		\le \sqrt{m}\|\bO-\bTheta\|_2
		\le \sqrt{r}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})
		.
	$$
	Weyl's inequality entails
	$$
		|\lambda_{\min}(\bTheta^T\bO) - m|
		\le
		\|\bTheta^T\bO-m\bI\|_2
		\le \sqrt{r}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})
	$$
	or
	$$
		\lambda_{\min}(\bTheta^T\bO) 
		\ge
		m - \sqrt{r}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})
		.
	$$
	Thus if $m > \sqrt{r}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})$, then
	$$
		\max_{i=1,\dotsc,m}\|\bTheta_i-\bO_i\|_{\rm F}
		\le
		\frac{2(\max_{i=1,\dotsc,m}\|(\bW\bO)_i\|_{\rm F} + \sqrt{r})}{m - \sqrt{r}(2\|\bW\|_2 + \sqrt{4\|\bW\|_2^2 + 2m})}
	$$
	as desired.
\end{proof}
\fi 

\begin{proof}[Proof of \Cref{lem:upperboundlocal}]
    Recall that $\bO$ is chosen without loss of generality such that $\bTheta^T\bO$ is symmetric and positive semidefinite. %by, if necessary, post-multiplying  an appropriate $r\times r$ orthogonal matrix to it.
    
    Assumption \ref{assumption} plays a similar role to inequality \eqref{eq:pertubation2} in the proof of \Cref{lemma:pertubation}. It immediately follows that
    \[
    2\sqrt{mr}\|\bW\|\|\bO-\bTheta\|_F
    \ge
    \tr(\bO^T\bW\bO) - \tr(\bTheta^T\bW\bTheta)
    \ge
    \frac{m}{2}\|\bO-\bTheta\|_F^2
    \quad
    \text{(under MAXBET model)}
    \]
    and
    \[
    2\sqrt{mr}\|\bW\|\|\bO-\bTheta\|_F
    \ge
    \tr(\bO^T\bW\bO) - \tr(\bTheta^T\bW\bTheta)
    \ge
    \left(\frac{m}{2}-1\right)\|\bO-\bTheta\|_F^2
    \quad
    \text{(under MAXDIFF model)}
    ,
    \]
    from which inequality \eqref{eqn:localupperbound1} holds.
    Inequality \eqref{eqn:localupperbound2} follows from inequality \eqref{eqn:localupperbound1} and
    \begin{align*}
    \|[\bW\bO]_i\|_F &\le
    \|[\bW(\bO - \bTheta)]_i\|_F + \|[\bW\bTheta]_i\|_F
    =
    \|\bW_{i\cdot}(\bO-\bTheta)\|_F + \|[\bW\bTheta]_i\|_F
    \\
    &\le
    \|\bW_{i\cdot}\|\|\bO - \bTheta\|_F + \|[\bW\bTheta]_i\|_F
    \le 
    \|\bW\|\|\bO - \bTheta\|_F + \|[\bW\bTheta]_i\|_F
    ,
    \end{align*}
    where $\bW_{i\cdot}=[\bW_{i1}, \dotsc, \bW_{im}]$ is the $i$th row block of $\bW$.
    
    Inequality \eqref{eqn:localupperbound1} also implies
    \begin{equation}\label{eqn:weyl}
    \|\bTheta^T\bO - m\bI_r\| \le
    \begin{cases}
    4\|\bW\|\sqrt{r}, &\text{under MAXBET model},
    \\
    4\|\bW\|\frac{\sqrt{r}}{1-2/m}, &\text{under MAXDIFF model}.
    \end{cases}
    \end{equation}
    
    We first consider the MAXBET model.
    Since $\bO=[\bO_1^T,\dotsc,\bO_m^T]^T$ is a
    %second-order 
    {candidate}
    critical point, the associated Lagrange multiplier $\bLambda_i$ of $\bO_i$ satisfies $\bO_i\bLambda_i = \sum_{j=1}^m\bS_{ij}\bO_j$
	(see equation \eqref{eqn:firstorder})
	and is symmetric, positive semidefinite. 
	%by  \Cref{prop:positivity}.
	Since $\bS_{ij} = \bTheta_i\bTheta_j^T + \bW_{ij}$, 
	\begin{equation}\label{eqn:lagrange2}
		\sum_{j=1}^m\bS_{ij}\bO_j 
		=
		\sum_{j=1}^m\bTheta_i\bTheta_j^T\bO_j + \sum_{j=1}^m\bW_{ij}\bO_j
		=
		\bTheta_i\bTheta^T\bO + [\bW\bO]_i
		.
	\end{equation}
	Thus from Lemma \ref{lem:normalcone}, we have
	\begin{align}\label{eqn:normalbound}
	0 &\ge \tr[(\bTheta_i-\bO_i)^T\sum_{j\neq i}\bS_{ij}\bO_j] 
	\nonumber\\
	&= \tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO]
	+ \tr[(\bTheta_i-\bO_i)^T[\bW\bO]_i]
	.
	\end{align}
	From Assumption \ref{assumption} and the choice of $\bO$, we have, similar to inequality \eqref{eq:pertubation11},
	\begin{equation}\label{eqn:eigenbound}
		\tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO]
		\ge
		\frac{1}{2}\lambda_r(\bTheta^T\bO)\|\bTheta_i-\bO_i\|_F^2
		.
	\end{equation}
	Then the Cauchy-Schwarz inequality and inequality \eqref{eqn:localupperbound2} entail
	\[
	\frac{1}{2}\lambda_r(\bTheta^T\bO)\max_{1\le i\le m}\|\bTheta_i-\bO_i\|_F
	\le \max_{1\le i\le m}\|[\bW\bO]_i\|_F
	\le \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}}
	.
	\]
	Combining inequality \eqref{eqn:weyl} and Weyl's inequalty,
	\[
	\lambda_r(\bTheta^T\bO) \ge m - 4\|\bW\|\sqrt{r}
	\]
	and inequality \eqref{eqn:localupperbound3} is obtained.
	
	Under the MAXDIFF model, equation \eqref{eqn:lagrange2} becomes
	\begin{align*}
		\bO_i\bLambda_i = \sum_{j\neq i}\bS_{ij}\bO_j 
		=
		\bTheta_i\bTheta^T\bO - \bTheta_i\bTheta_i^T\bO_i + [\bW\bO]_i
	\end{align*}
	and inequality \eqref{eqn:normalbound} is replaced by
	\begin{align*}
	0 \ge
	\tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta^T\bO]
	- \tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta_i^T\bO_i]
	+ \tr[(\bTheta_i-\bO_i)^T[\bW\bO]_i]
	.
	\end{align*}
	Inequality \eqref{eqn:eigenbound} remains intact, and
	\begin{align*}
	    - \tr[(\bTheta_i-\bO_i)^T\bTheta_i\bTheta_i^T\bO_i]
	    &= 
	    \tr[(\bO_i-\bTheta_i)^T\bTheta_i\bTheta_i^T(\bO_i-\bTheta_i)] - \tr[(\bTheta_i - \bO_i)^T\bTheta_i\bTheta_i^T\bTheta_i]
	    \\
	    &\ge
	    -\|\bTheta_i\bTheta_i^T\|\|\bO_i - \bTheta_i\|_F^2
	    - \tr[(\bTheta_i - \bO_i)^T\bTheta_i]
	    \\
	    &\ge
	    - \|\bO_i - \bTheta_i\|_F^2
	    - \tr(\bI_r - \bO_i^T\bTheta_i)
	    \\
	    &\ge
	    - \|\bO_i - \bTheta_i\|_F^2
	    - [r - \tr(\bO_i^T\bTheta_i)]
	    \\
	    &\ge
	    - \|\bO_i - \bTheta_i\|_F^2
	    -\frac{1}{2}[\|\bO_i\|_F^2 + \|\bTheta_i\|_F^2 - 2\tr(\bO_i^T\bTheta_i)]
	    \\
	    &=
	    -\frac{3}{2}\|\bO_i - \bTheta_i\|_F^2
	    ,
	\end{align*}
	where the third line is due to $\|\bTheta_i\bTheta_i^T\|\le 1$.
	Hence the Cauchy-Schwarz inequality and inequality \eqref{eqn:localupperbound2} now give
	\[
	\frac{1}{2}(\lambda_r(\bTheta^T\bO)-3)\max_{1\le i\le m}\|\bTheta_i-\bO_i\|_F
	\le \max_{1\le i\le m}\|[\bW\bO]_i\|_F
	\le \max_{1\le i\le m}\|[\bW\bTheta]_i\|_F + 4\|\bW\|^2\frac{\sqrt{r}}{\sqrt{m}-2/\sqrt{m}}
	.
	\]	
	Inequality \eqref{eqn:weyl} and Weyl's inequality now result in
	\[
	\lambda_r(\bTheta^T\bO) \ge m - 4\|\bW\|\frac{\sqrt{r}}{1-2/m}
	\]
	and inequality \eqref{eqn:localupperbound3} is obtained.
	For a valid bound we need
	\[
	m > 4\|\bW\|\frac{\sqrt{r}}{1-2/m} + 3
	.
	\]
	Solving the involved quadratic inequality provides the desired lower bound for $m$.
\end{proof}



==> sections/07-conclusion.tex <==
\section{Conclusion}
This paper studies the orthogonal trace-sum maximization \citep{won2018orthogonal} . It shows two results  when the noise is small: first, that while the problem is nonconvex, its solution can be achieved by solving its convex relaxation; second, any local minimizer with Assumption~\ref{assumption} is also its global minimizer. 

A future direction is to improve the estimation on maximum noise that this method can handle. While this paper shows that the method succeeds when $\sigma=O(m^{1/4})$, we expect that it would also hold for noise as large as $\sigma=O(m^{1/2})$, which has been proved in \cite{ZhongBoumal18PhaseSynchNearOptimalBounds} for phase synchronization and in \cite{ling2021improved} for synchronization of rotations. Another future direction is to use a more generic model than the additive Gaussian noise model, which would have a larger range of real-life applications.



==> sections2/00-abstract.tex <==
This paper studies an optimization problem on the sum of traces of matrix quadratic forms in $m$  {semi-}orthogonal matrices, which can be considered as a generalization of the synchronization of rotations. While the problem is nonconvex, the paper shows that its semidefinite programming relaxation solves the original nonconvex problems exactly  {with high probability}, under an additive noise model with small noise in the order of $O(m^{1/4})$. In addition, it shows that a local solution of the nonconvex problem is also its global solution  {with high probability under similar conditions}. These results can be considered as a generalization of existing results on phase synchronization.

